Camera Fingerprint Extraction via Spatial Domain Averaged Frames

Photo Response Non-Uniformity (PRNU) based camera attribution is an effective method to determine the source camera of visual media (an image or a video). To apply this method, images or videos need to be obtained from a camera to create a "camera fingerprint" which then can be compared against the PRNU of the query media whose origin is under question. The fingerprint extraction process can be time-consuming when a large number of video frames or images have to be denoised. This may need to be done when the individual images have been subjected to high compression or other geometric processing such as video stabilization. This paper investigates a simple, yet effective and efficient technique to create a camera fingerprint when so many still images need to be denoised. The technique utilizes Spatial Domain Averaged (SDA) frames. An SDA-frame is the arithmetic mean of multiple still images. When it is used for fingerprint extraction, the number of denoising operations can be significantly decreased with little or no performance loss. Experimental results show that the proposed method can work more than 50 times faster than conventional methods while providing similar matching results.

==> sections/old/3_background_bkp.tex <==
\section{Background and Related Work}
\label{sec:background}

In this section, we discuss PRNU-based source camera attribution and video stabilization. 

% 1) talk about prnu
% 2) talk about denoising
% 3) fingerprint extraction
% 4) Stabilization

\subsection{PRNU-based Source Camera Attribution}
\label{sec:background:PRNU}
PRNU-based camera attribution is established on the fact that the output of the camera sensor, $I$, can be modeled as 
\begin{equation}
    I = I_0 + I_0K + \psi
\label{Eq:im_noise}
\end{equation}
where $I_0$ is the noise-free still image, $K$ is the PRNU noise, and $\psi$ is the combination of additional noise, such as readout noise, dark current, shot noise, content-related noise, and quantization noise which are of random nature. The multiplicative PRNU noise pattern, $K$, is unique for each camera and can be used as a camera fingerprint which allows to attribute visual media to its source camera.
Using a denoising filter $F$ (such as a Wavelet filter) on a set of images of a camera,
we can estimate the camera fingerprint by first getting the
noise residual (i.e., the estimated PRNU) of $i^{th}$ image as $F_i = I_i - F(I_i)$, and then combining the noise residuals of all the images.
For determining if a specific camera has taken
a given query image, we can first obtain the noise residual of the query image using $F$, and then correlate the noise residual with the camera fingerprint.



% Denoising is typically done in each color component separately which results in three PRNU noise patterns of the same resolution: $X_R$, $X_G$, and $X_B$ \cite{fridrich2009digital}. These three noise components  are then converted to a final  noise component $X$ as follows:
% \begin{equation}
% \label{eqn:noise_weights}
%     X=0.3\times X_R + 0.6\times X_G + 0.1\times X_B.
% \end{equation}

%o estimate the PRNU noise $K$ from $I$, a denoising filter (such as Wavelet Denoising\cite{mihcak1999low}, BM3D\cite{dabov2009bm3d}) is used to estimate the noise free signal $I^0$. Using the denoising filter, the noise residual, $W = I^{(0)}K + \psi_1 + \psi_2$, where $\psi_2$ is the post-denoising noise, is obtained. Then, the PRNU noise $K$ is estinated from $n$ given images using Minimum Likelihood Estimation (MLE) as
% \begin{equation}
%     K = \frac{\sum_{i=1}^{n} W_i . I_i}{\sum_{i=1}^{n} I_i^2}
% \end{equation}
% where $W_i$ is noise pattern extracted from $I_n$ and all the operations are element-wise. %Jessica et al suggests when $N$ is more than 20, a reliable camera fingerprint estimate can be extracted from images, [citation].  Talk more about images.

%A given query image can then be attributed to a camera by matching the PRNU noise extracted from the query image with $K$ using the Pearson correlation coefficient or Peak-to-Correlation Energy (PCE). However, for this to work, the PRNU of the query image has to be aligned with the camera fingerprint. If the image or fingerprint is resized, the correct resizing parameter must be found, and the resizing operation must be reversed. A brute force method can be used to find the resizing parameters~\cite{jessica:crop}. When a still image is cropped, Normalized Cross Correlation (NCC)~\cite{lewis1995fast} can be used to find the cropping location~\cite{jessica:crop}.

Over the years, PRNU-based source camera attribution for images has taken enough attention that various research has been done to improve PRNU based attribution~\cite{jessica:camera, Sutcu:2007:Improve, Li:2012:Color, Chierchia:2010:IDP, Li:2010:Enhance},
as well as using the scheme for purposes other than attribution~\cite{Caldelli:201:WIFS, lukavs2006detecting, Chierchia:2014:Fing}. 


Although some initial work has been done for extending image-centric methods towards video ~\cite{Chen:2007:Vid, McCloskey:2008:Confidence, chuang2011exploring, Simone:VideoOv:2012, Chen:2013:Video, Houten:2009:YVid, hyun2012camcorder}, applying the same schema for videos poses some other challenges. First challenge is a video typically goes through severe compression. Therefore, the PRNU signals extracted from video frames are quite weak. To overcome this, several frames are required to be denoised to extract a reliable camera fingerprint. This makes fingerprint extraction process to be time-consuming. Chuang et al. investigated the effect of the video compression on the video frames and their results have shown I-frames contain stronger PRNU signal compared to other frames. Moreover, using all frames tends to create a better fingerprint estimate than only I- or P-frames \cite{chuang2011exploring}. 

Secondly, as [mixed media and \cite{jin2012analysis}] present, video frames typically undergo different processes (such as binning or line-skipping) to resize the sensor output than images. Moreover, the parameters of these processes are unknown to investigators; therefore, their attribution in the case of mixed media setting is not straightforward. 

Third problem is the usage of video stabilization which causes desynchronization between the fingerprint estimate obtained from a video and the camera sensor. This issue has been addressed by \cite{taspinar2016prnu, iuliani2017hybrid} both of which used brute-force approach to do attribution and had limited success. Another issue for both of them was they used the first frame as reference (i.e., non-stabilized) frames as they typically are not geometrically transformed. However, this approach is not practical because the first frame may not be available or different stabilization techniques may geometrically transform it.
Later, Luisa et al has proposed a technique [luisa2019facing] which chooses a reference frame which matches with has the largest number of frames. In this problem, they assume the video may have enough frames that are transformed with similar resizing and scaling factors. However, videos with high shakes may not have enough frames that are goes through a similar transformation. 
[READ MORE, EXPLAIN BETTER]. Moreover, XXX has proposed that when a stabilized video is long enough (i.e. more than 4 mins), it can be matched against other fingerprints obtained from the same camera. However, all these techniques have very high time-complexity. For example, obtaining a fingerprint from a 4-min full HD video (\textit{i.e.} approx. $7200$ frames) might take up to 4-5 hours from a single-threaded implementation. Similarly, exhaustively trying many possible transformation parameters (i.e., resizing, rotation, and translation) might take hours to extract a single fingerprint. Therefore, these techniques may not be usable when immense amount of data is available. 

\subsection{Video Stabilization}
\label{sec:VidCap}

\begin{figure}[ht!]
\centering
  \includegraphics[height=56mm, width=85mm]{images/background/StabilizationProcess}
  \caption{Video Stabilization Pipeline. This figure is a modified version of a figure that appeared in~\cite{Ejaz:2012:Video}.}
 \label{Fig:VidStab}
\end{figure}

\textbf{WE CAN PUT AFFINE HERE AND EXPLAIN IT. AND TELL IN NON-STABILIZED, ROTATION WRT SENSOR IS ZERO. ONLY SCALE (BINNING, LINE-SKIPPING) AND CROP.}

Video stabilization removes the effect of shakes, jitters, etc. from a video, that results when the camera is subject to unintentional motion (e.g., due to shaking of hand). A video can be stabilized either using an optical or digital stabilization.
Optical stabilization has limited effect on PRNU-based source camera attribution, as it doesn't cause any geometric transformation instead it uses an extra physical device to compensate unintentional shake~\cite{Hoglund:2011:VideoStab}. On the other hand, digital stabilization (also called electronic stabilization) geometrically transforms (e.g., rotates, resizes and/or translates) a frame with respect to a reference frame such that the unintentional motion between the frames is removed. In practice, digital stabilization is used more often, as  optical stabilization is expensive. Unlike optical stabilization, digital stabilization can have significant impact on PRNU-based source camera attribution. Hence, we refer digital stabilization when we use the term \emph{stabilization}.


A video can be digitally stabilized either internally when it is being captured, or externally after it has been captured. In the case of the former, stabilization software provided by the camera manufacturer is integrated into the video capturing software. In the case of the latter, stabilization is done by a standard  third-party software (e.g., FFMPEG \textit{deshaker}) that is not part of the video capturing pipeline. In this paper, we focus on the latter.

An out-of-camera video stabilization process contains three major stages: camera motion estimation, motion smoothing, and motion correction (Figure~\ref{Fig:VidStab})~\cite{Matsushita:VideoStab:2006}~\cite{Ejaz:2012:Video}. In the motion estimation step, the global inter-frame motion between adjacent frames of a non-stabilized video is modeled from the optical flow vectors of the frames using an affine transformation. 
In the motion smoothing step, unintentional translations and/or rotations are filtered out from the global motion vectors using a low pass filter. Finally, in the motion correction step,  stabilized video is created by shifting and/or rotating frames according to the parameters in the filtered motion vector. Since different frames can shift and/or rotate using different parameters, pixels across frames can be misaligned with each other with respect to the underlying sensor array.



==> sections/old/3b_related_work.tex <==
\section{Related Work}
\label{sec:related}

1) denoising algorithms


\subsection{Fingerprint extraction from images}
% TALK ABOUT CONVENTIONAL WAY, CT.LI PAPER MAYBE?

\subsection{Fingerprint extraction from videos}
When a video is captured, they have undergone a compression process which aims to decrease the storage usage in disk. One of the most used algorithm to date is H264 in which there are three types of frames: intra-coded (I-frame), predicted (P-frame), and bidirectional predicted picture (B-frame). I-frames can be considered as starting point frames. The compression algorithm needs to know it to compress the other two types of frames. P-frames depends on previous frames, therefore, to decode a P-frame, previous frames must be decoded and B-frames requires both previous and the next frame to be decoded. Hence, I-frames have the lowest compression whereas B-frames have the highest compression, therefore, the PRNU noise of the P- and B-frames tend to contain more random noise than I-frames. (i.e. $\psi$ in Eqn. ~\ref{Eqn:im_noise}).

\textbf{TALK ABOUT PREVIOUS WORK?}

\textbf{MAKE IT BETTER, DON'T JUST TALK ABOUT 30-FRAMES ETC. MAKE IT MORE GENERAL}
This paper proposes the notion of average-frame (\textit{avg-frame}) to compute fingerprint. An average frames is the arithmetic mean of all frames from an i-frame to the next one (Group of Pictures, \textit{GoP}). We divide the set into $30$-framed subgroups and obtained an avg-frame from each of them. \textbf{The intuition behind this notion is when a fingerprint is created each of i-, p-, and b- frames contribute to improve its quality. If only one type of frame (e.g. i-frames) is used, the other types will not contribute. However, when the average of $30$ frames is taken to create an avg-frame, the avg-frame may have a better quality than individual frames}

\subsection{Time issue}
One of the issues related to PRNU based source attribution is the time complexity of the technique. This issue can be evaluated into two main parts: creation of database and identification.

\subsection{stabilization}


==> sections/old/4_our_approach_10jun.tex <==
\section{Spatial Domain Averaging}
\label{sec:approach}
As mentioned in the introduction, this paper proposes spatial domain averaging to reduce the number of expensive denoising operations performed  when computing camera fingerprints from a large number of media objects taken from the camera.  Efficient computation of a fingerprint is  achieved by  first creating  averaged objects from a large collection, and using these averaged objects  for computing the fingerprint. For example, given a video with $m$ frames, $g$ non-intersecting equal-sized subgroups (i.e., each subgroup has $d = \frac{m}{g}$ frames) are formed and a \textit{Spatial Domain Averaged frame (SDA-frame)} is created from each subgroup. Then, in the second step each SDA-frame is denoised, and an averaging of the estimated PRNU noise is done to  arrive at the final camera fingerprint estimate. In this manner, the number of frames that are denoised gets reduced by a factor of $d$ {\color{blue}which we call the depth of the sda-frame}. As another example, an sda-frame obtained from three different images is shown in Figure~\ref{fig:avgframe}.  

\begin{figure}[!ht]
\centering
\subfloat [1st] {\includegraphics[height=15mm]{images/avg_frame/im1.jpg}}~
\subfloat [2nd] {\includegraphics[height=15mm]{images/avg_frame/im2.jpg}}~
\subfloat [3rd] {\includegraphics[height=15mm]{images/avg_frame/im3.jpg}}~~
\subfloat [SDA-frame] {\includegraphics[height=15mm]{images/avg_frame/avg.jpg}}
\caption{SDA-frame is the average of 1st, 2nd, and 3rd frames.}
\label{fig:avgframe}
\end{figure}

% The difference between the proposed method and the conventional fingerprint extraction method is shown in Figure TODO. As shown in the figure, the proposed method introduces an extra pre-processing step of frame averaging. Other fingerprint computation steps are similar to the conventional method.  

When using the above approach, there are many questions that arise. First, does averaging lead to a drop in the accuracy of the fingerprint computed as compared to the conventional method, assuming the same number of images are used for both? If so, what is the trade-off between decrease in computation and the loss in accuracy? What is the optimal combination of averaging and denoising that leads to the least computation while yielding the best performance? In the next two subsections, we first investigate these questions analytically using a simple framework. We then validate our analysis in the next section by providing experimental results. The results show that spatial domain averaging strategy can indeed result in significant saving in computation while maintaining performance. 






%Given $m$ pictures to compute the camera fingerprint, the proposed method divides the pictures are divided into $d$ disjoint sets of equal number of pictures. An sda-frame is then computed from each set using the arithmetic mean on member pictures. Each picture $F$ of a set can be considered as a matrix of $3 \times r$ color components (i.e., R, G, and B), where $r$ is the dimension of the pictures. Thus, the sda-frame $F_{sda}$ of the set can be computed as $F_{sda} = \frac{F_1 + F_2 + \dots + F_{m/d}}{m/d}$ (each set has $m/d$ elements).% Figure~\ref{Fig:avgframe} shows an example of an sda-frame computed from three images.
%Similar to how conventional method works (discussed in Section~\ref{sec:background:PRNU}), the $k$ sda-frames are then denoised, and the $k$ noise are used to obtain the camera fingerprint. 

%The frame averaging method uses all $n$ frames of a video (i.e., all $n$ I-frames p-frames and b-frames) to compute the camera fingerprint. The $n$ frames are divided into $k$ disjoint sets of equal number of frames. An average frame (called as \textit{avg-frame}) is computed from each set using the arithmetic mean on member frames. Each frame $F$ of a set can be considered as a matrix of $3 \times r$ color components (i.e., R, G, and B), where $r$ is the dimension of the fame. The avg-frame $F_{avg}$ of the set can be computed as $F_{avg} = \frac{F_1 + F_2 + \dots + F_{n/k}}{n/k}$ (each set has $n/k$ elements). Figure~\ref{Fig:avgframe} shows an example of an avg-frame computed from three frames. The $k$ avg-frames are then denoised, and the $k$ noise are further averaged to obtain the camera fingerprint. In this paper, the value of $k$ is fixed to $30$, as a GoP (Group of Pictures) of the video in most cases contains $30$ frames. 

%the random noise $\psi$ (Equation~\ref{Eqn:im_noise}) contains both pre-denoising random noise $\psi_1$ (such as quantization noise, compression noise) and post-denoising random noise $\psi_2$. While the picture averaging can reduce $\psi_1$, the PRNU noise averaging can reduce both $\psi_1$ and $\psi_2$. In the case of the proposed picture averaging method, all the frames are used to reduce $\psi_1$ and PRNU noise of only $k$ sda-frames are used to reduce $\psi_2$.

% \label{sec:math}
The proposed frame averaging approach is inspired by the fact that the averaging operation can be used as a filter for reducing some random noise from an image. In the PRNU-based method, random noise can be either a pre-denoising random noise such as quantization noise, compression noise or post-denoising random noise which {\color{blue}is the noise introduced by the sub-optimal denoising filter}. The averaging of frames can reduce the pre-denoising random noise and make a stronger PRNU noise.

This section provides an analysis of the proposed sda-frames scheme. To this end, we
first provide an analysis of the conventional (non-sda-based) PRNU-based method, and then analyse the sda-based method.

\subsection{Conventional method}
As discussed in Section~\ref{sec:background}, in the conventional method, the camera fingerprint is estimated from $n$ given images. Each image $I$ can be modeled as $I = I_0 + I_0K + \psi_1$, where $\psi_1$ is the pre-denoising random noise (Equation~\ref{Eq:im_noise}). 

To estimate the PRNU noise $K$, a denoising filter (such as Wavelet Denoising\cite{mihcak1999low}, BM3D\cite{dabov2009bm3d}) is used to estimate the noise free signal $I^0$. Using the denoising filter, the noise residual, $W = I^{(0)}K + \psi_1 + \psi_2$, where $\psi_2$ is the post-denoising noise. Then, the estimated PRNU noise $\hat{K}$ can be estimated  using Maximum Likelihood Estimation (MLE) as
\begin{equation}
    \hat{K} = \frac{\sum_{i=1}^{n} W_i . I_i}{\sum_{i=1}^{n} I_i^2}
\end{equation}
where $W_i$ is noise pattern extracted from $I_i$.%, and all the operations are element-wise. %Jessica et al suggests when $N$ is more than 20, a reliable camera fingerprint estimate can be extracted from images, [citation].  Talk more about images.

Note that in the estimated PRNU noise $\hat{K}$, the PRNU noise is the signal of interest whereas  $\psi_1$ and $\psi_2$ are the unwanted noise. The quality of $\hat{K}$ can be assessed from its variance $Var(\hat{K})$. The lower the variance, the higher the quality (and vice-versa). Assuming that $\psi_1$ and $\psi_2$ are White Gaussian noise with variances $\sigma_1^2$ and $\sigma_2^2$ respectively,  $Var(\hat{K})$ can be found as (using Cramer-Rao Lower Bound as shown by Fridrich et al.\cite{Jessica:Sensor:2013})
\begin{align} \label{eq:conv1}
    Var(\hat{K}) \ge \frac{\sigma_1^2 + \sigma_2^2}{\sum_{i=1}^n I_i^2}.
\end{align}
Thus a better PRNU is obtained from lower $\sigma_1^2$  and $\sigma_2^2$ (smoother image), and high luminance.

\subsection{Proposed Sda-based method}
In this subsection we derive the variance of the estimated PRNU noise obtained using frame averaging. We then compare this variance with the variance obtained by the conventional approach (in Equation~\ref{eq:conv1}).    

Suppose $I_1, I_2, \dots, I_m$ are $m$  images used to compute the camera fingerprint. With frame averaging, these $m$ images are divided into $d = \frac{m}{g}$ disjoint sets of equal size with $g$ pictures in each set. From each set, an average image is computed. Thereafter, the process is similar to the conventional approach. Each average picture is denoised, and the PRNU noise is estimated from $d$ noise residuals using the MLE.

Suppose, $I_i^{avg}$ is the average picture obtained from the $i^{th}$ image-set. Then 
\begin{equation}
\begin{aligned}
I_i^{avg} &= \frac{\sum_{j=(i-1)g+1}^{ig} I_j}{g} \nonumber \\
          &= \frac{\sum_{j=(i-1)g+1}^{ig} (I^0_j + I^0_jK +\psi_{1,j}) }{g} \nonumber
\end{aligned}
\end{equation}


%The picture averaging (aka frame averaging) has been studied before~\cite{JM:FrameAverage:1992}~\cite{Swindell:FrameAverage:1995}. 
%Although picture averaging can decrease the random noise, it can, however introduce motion blurring~\cite{Nayar:FrameAverage:2004}\cite{Kavanaugh1990}. The motion blurring can degrade the quality of the average image, and hence weaken the estimated PRNU noise. Considering the motion blurring factor, we can write the above equation as 

% \begin{equation}
%     I_i^{avg} = I_i^{0, avg, blur} + I_i^{0, avg, blur}K + \psi_{1, i}^{avg},
%     \label{eq:avg1}
% \end{equation}

% where $I_i^{0, avg, blur} = I_i^{0, avg}*B$ and $I_i^{0, avg}$ is the blur-free image, $B$ is the blurring kernel that degrades the image, and $*$ is the convolution operator. 

%The average image is more blurred when more number of images are used in averaging and the image content differs (citation). On the other hand, with a more number of images in averaging, the average image is more smoothed. As we discussed above, smooth images are better for estimating PRNU. Thus, a tradeoff between the effect due to blurring and smooth content is resulted due to image averaging.% Mathematically finding the value of $g$ that fine balances the effect of blurring and content smoothness is difficult as the derivation depends on the un-predictable image content. In this paper, we empirically obtained the ideal value of $g$ for a particular dataset of images and videos in Section TODO.

We can write the above equation as 
\begin{equation}
    I_i^{avg} = I_i^{0, avg} + I_i^{0, avg}K + \psi_{1, i}^{avg},
    \label{eq:avg1}
\end{equation}
where $I_i^{0, avg}$ is the noise free image, and $\psi_{1, i}^{avg}$ is the random noise in the average image. %The random noise also contais the blurring noise that results due to image averaging operation.
This random noise can be written as
$$
\psi_{1, i}^{avg} = \frac{\sum_{j=(i-1)g+1}^{ig} \psi_{1,j}}{g}.
$$
Suppose $\sigma_1^2$ is the variance of $\psi_{1}$'s (which is assumed to be white Gaussian noise). Then, the variance of $\psi_{1, i}^{avg}$ turns out to be $\frac{\sigma_1^2}{g}$.

Suppose $W^{avg}$ is the noise residual of each average image $I^{avg}$. Then, 
\begin{align}
W^{avg}  &= I^{avg} - F(I^{avg}) \nonumber \\
        &= I^{avg}_{0}K + \psi_{1}^{avg} + \psi_{2}^{\prime}\nonumber,
\end{align} 
where {\color{blue}$F$ is the denoising filter, and post-denoising noise $\psi_{2}^{\prime} = I^{0, avg} - F(I^{avg}) + \phi$. The $\phi$, such as filter modelling noise, is independent of the averaging operation. Also, the post-denoising noise is assumed to be independent of the content as this is very small \cite{Jessica:Sensor:2013}. Thus, we can assume $\psi_{2}^{\prime} = \psi_{2}$, and hence $\psi_{2}^{\prime}$ have variance $\sigma_2^2$.

Using the MLE, the PRNU can now be estimated from $d$ average frames $I_1^{avg}, I_2^{avg}, \dots, I_d^{avg}$ as
\begin{align} \nonumber
    \hat{K^{avg}} = \frac{\sum_{i=1}^{d} W_i^{avg} . I_i^{avg}}{\sum_{i=1}^{d} \big(I_i^{avg}\big)^2}.
\end{align}

Using the Cramer-Rao Lower Bound, the variance of the estimated PRNU $\hat{K^{avg}}$ can be found as
\begin{align} \label{eq:OurVar}
    Var (\hat{K^{avg}}) \ge \frac{ \frac{\sigma_1^2}{g} + \sigma_2^2}{\sum_{i=1}^d \big(I_i^{avg}\big)^2}.
\end{align}

In an ideal case, we want that the averaging operation does not degrade the quality of the estimated PRNU from the average frames. In other words, we want that $Var (\hat{K^{avg}})$ is approximately equal to the variance from the conventional method $Var (\hat{K})$. That is, 
$$
Var (\hat{K^{avg}}) \approx Var (\hat{K}).
$$
Therefore, using the results from Equation~\ref{eq:conv1} and Equation~\ref{eq:OurVar}, it is desired that
$$
\frac{ \frac{\sigma_1^2}{g} + \sigma_2^2}{\sum_{i=1}^d \big(I_i^{avg}\big)^2} \approx \frac{\sigma_1^2 + \sigma_2^2}{\sum_{i=1}^n I_i^2}.
$$
By simplifying the above equation, we get
$$
\frac{ \frac{\sigma_1^2}{g} + \sigma_2^2} {\sigma_1^2 + \sigma_2^2}  \approx \frac  {\sum_{i=1}^d \big(I_i^{avg}\big)^2}  {\sum_{i=1}^n I_i^2}.
$$

Suppose 
$$\frac  {\sum_{i=1}^d (I_i^{avg})^2}  {\sum_{i=1}^n I_i^2} = \frac{d}{n} \times N
$$ where 
$$k = \frac  {(\sum_{i=1}^d (I_i^{avg})^2)/d}  {(\sum_{i=1}^n I_i^2)/n}.$$ Note that the value of $k$ is greater than or equal to $1$. Putting these values in the above equation, we get
$$
\frac{d}{n} \times k \approx \frac{ \frac{\sigma_1^2}{g} + \sigma_2^2} {\sigma_1^2 + \sigma_2^2}.
$$
Putting $d=\frac{m}{g}$ in the above equation, we get
$$
\frac{m \times k}{g \times n} \approx \frac{\sigma_1^2 + g \times \sigma_2^2 }{g \times (\sigma_1^2 + \sigma_2^2)}.
$$
or,
\begin{align} \label{eq:finalourapproach}
 k \approx \frac{n}{m} \times \frac{\sigma_1^2 + g \times \sigma_2^2 }{\sigma_1^2 + \sigma_2^2}
\end{align}

As discussed above, $k \ge 1$. Thus, the number of images required in the proposed approach $m$ is greater than equal to the number of images required in the conventional method $n$. Ideally, we would like to have $m$ close to $n$. This can be achieved when $k = 1 + \epsilon$ (where $\epsilon$ is a small value) and $\sigma_2^2$ is also small. In other words, when we have smoother content.{{\color{blue} When the images are textured, $k$ tends to increase as $g$ increases.}

The analysis above indicates that \textit{(i)} when images are smooth, sda-based and conventional approaches are similar (i.e., $k \approx 1$) \textit{(ii)} when images are textured, sda-based approach requires more images that conventional one to achieve similar performance, and \textit{(iii)} for textured images whose post-denoising noise (i.e., $\sigma_2$) is low, as the sda-depth (i.e., $g$) increases, the total number of images required by the sda-based approach compared to the conventional way (i.e., $k$) also increases. In the following section, we experimentally validate these observations .



==> sections/old/4_our_approach_backup.tex <==
\section{Our Approach}
\label{sec:approach}

This paper investigates the effectiveness of the usage of spatial domain image averaging technique for camera fingerprint extraction. The main idea behind this schema is to create a reliable camera fingerprint from images or non-stabilized videos in a efficient way when many still images are available. 

%In this section, first the spatial domain picture averaging idea to compute a camera fingerprint from images and non-stabilized videos has been discussed. 

% \begin{figure}[!ht]
%     \centering
%     \subfloat[Example of a binning scheme (Obtained from ~\cite{jin2012analysis})]
%     {\label{Fig:binning}\includegraphics[width=66mm]{images/bin_lineskip/binning}}
    
%     \subfloat[Example of a line-skipping scheme]
%     {\label{Fig:lineskip}\includegraphics[width=66mm]{images/bin_lineskip/line_skipping}}
%     \caption{Two different in-camera resizing schemes}
%     \label{Fig:resizing schemes}
% \vspace{-2mm}
% \end{figure}

\begin{figure}[!ht]
\centering
\subfloat [1st] {\includegraphics[height=15mm]{images/avg_frame/im1.jpg}}~
\subfloat [2nd] {\includegraphics[height=15mm]{images/avg_frame/im2.jpg}}~
\subfloat [3rd] {\includegraphics[height=15mm]{images/avg_frame/im3.jpg}}~
\subfloat [SDA-picture] {\includegraphics[height=16mm]{images/avg_frame/avg.jpg}}
\caption{SDA-picture is the average of 1st, 2nd, and 3rd frames.}
\label{Fig:avgframe}
\end{figure}

\subsection{Spatial Domain Averaged Picture}
\label{sec:approach:sda_picture}
Given a set of still images taken by a "known camera", the first step is to extract its reference camera fingerprint which will, later, be compared against the PRNU noise of any visual media under questioning. This will help investigators prove if the questioned visual media is captured by the "known camera". The existing methods for camera fingerprint extraction (See Background) choose $m$ still images out of $n$ that is captured by the known camera ($1 \leq m \leq n$). The two weaknesses of this approach are \textit{(i)} low source attribution performance (i.e. unreliable camera fingerprint) when $m$ is low and \textit{(ii)} slow fingerprint extraction when $m$ is high. This research proposes an alternative technique, the usage Spatial Domain Averaged (sda-) picture that may significantly speed up the fingerprint extraction process when the number of still images is very high. Although some improvements can be achieved for images, the speed up is more compelling for videos.  

The method uses $t$ pictures ($m < t \leq n$) to compute the camera fingerprint. The $t$ pictures are divided into $k$ disjoint sets of equal number of pictures. An sda-picture is computed from each set using the arithmetic mean on member pictures. Each picture $F$ of a set can be considered as a matrix of $3 \times r$ color components (i.e., R, G, and B), where $r$ is the dimension of the pictures. The sda-picture $F_{sda}$ of the set can be computed as $F_{sda} = \frac{F_1 + F_2 + \dots + F_{t/k}}{t/k}$ (each set has $t/k$ elements). Figure~\ref{Fig:avgframe} shows an example of an sda-picture computed from three images. The $k$ sda-frames are then denoised, and the $k$ noise are further averaged to obtain the camera fingerprint. 

%The frame averaging method uses all $n$ frames of a video (i.e., all $n$ i-frames p-frames and b-frames) to compute the camera fingerprint. The $n$ frames are divided into $k$ disjoint sets of equal number of frames. An average frame (called as \textit{avg-frame}) is computed from each set using the arithmetic mean on member frames. Each frame $F$ of a set can be considered as a matrix of $3 \times r$ color components (i.e., R, G, and B), where $r$ is the dimension of the fame. The avg-frame $F_{avg}$ of the set can be computed as $F_{avg} = \frac{F_1 + F_2 + \dots + F_{n/k}}{n/k}$ (each set has $n/k$ elements). Figure~\ref{Fig:avgframe} shows an example of an avg-frame computed from three frames. The $k$ avg-frames are then denoised, and the $k$ noise are further averaged to obtain the camera fingerprint. In this paper, the value of $k$ is fixed to $30$, as a GoP (Group of Pictures) of the video in most cases contains $30$ frames. 

The picture averaging idea is inspired by the fact that the averaging operation can be used as a filter for reducing random noise. In PRNU-based method, the random noise $\psi$ (Equation~\ref{Eqn:im_noise}) contains both pre-denoising random noise $\psi_1$ (such as quantization noise, compression noise) and post-denoising random noise $\psi_2$. While the picture averaging can reduce $\psi_1$, the PRNU noise averaging can reduce both $\psi_1$ and $\psi_2$. In the case of the proposed picture averaging method, all the frames are used to reduce $\psi_1$ and PRNU noise of only $k$ sda-pictures are used to reduce $\psi_2$. 

\textbf{WE MAY PUT THE MATH PART HERE}




\subsection{SDA-picture for Videos}
\label{section:sda4videos}
Each video consists of many frames (I-, P- or B-frames) which are undergone a heavy compression. When the PRNU noise of a single video frame is extracted, the noise is highly contaminated with this compression noise, therefore, many frame must be denoised to extract a reliable camera fingerprint. 
Since denoising operation is computationally the most expensive step of camera fingerprint extraction, this process becomes very slow for videos. Hence, the usage of sda-picture for video fingerprint extraction is a very natural case. 


Section 3b (Related work) lays out the existing methods for fingerprint extraction. When the number of frames is fixed, the fingerprint obtained from I-frames is better than P-frames or B-frames in terms of True Positive Rate(TPR). When the fingerprint is obtained from all frames, the TPR (and average PCE) is better than the methods above. However, usage of all-frames significantly increases the time requirement for fingerprint extraction. For example, it takes around $45$ minutes for to extract a camera fingerprint from a $1$~minute Full HD video $@30$FPS (a total of 1800 frames) in a single-threaded Matlab code. 

When a camera fingerprint is extracted from only I-frames, low TPR problem occurs whereas using all-frame causes slow fingerprint extraction process which is not usable when there are several videos in the database. Therefore, it is a big necessity to provide solutions that will help extract fingerprint as fast as from I-frames and perform as good as from all-frames. The usage of sda-frame can help achieve this target. The first step is to divide the video into subgroups of $k$ frames each and sda-picture of each subgroup is obtained (See Section~\ref{sec:approach:sda_picture}) which are then denoised to create a fingerprint.


% ---I DIDNT LIKE HOW I EXPLAINED, MAKE IT BETTER!!!
% Besides decreasing the time complexity for fingerprint extraction, sda-picture can be used as a solution to other \textbf{video forensics issues}. Since the frames of a video are highly compressed, the noise of two frames from the same video are likely to not match. 
% The PCE result of the noise of two frames from the same video tends to be very low (below threshold) unless they are consecutive frames. This is due to the very strong compression applied to the videos. Therefore, it is almost impossible to tell if the two video frames are taken from the same

\textbf{STABILITY DETECTION}
\cite{taspinar2016source} has proposed stability detection algorithm that divides a video into two halves and a camera fingerprint is extracted from each half by denoising the I-frames. Then, the fingerprints are correlated to detect if the video is stabilized. However, the process, again, requires many denoising of the frames. Because the PRNU noise of each sda-picture is a much stronger signal than the noise of individual frames, the proposed approach can help achieve stability detection by only few denoising instead of many. 

%Another use case for this idea for videos is the detection of \textit{sequential foreign frames} which are multiple consecutive frames that are from another camera added to the video. To detect \textit{sequential foreign frames}, the sda-picture of each Group of Picture (GoP: from one I-frame to the next one, typically 30 frames), is extracted and the correlation of PRNU noise of each sda-picture is expected to be high; the ones which are below the threshold are potentially from another camera. One weakness of this idea is if the number of foreign frames are not consecutive or not a high number, the proposed idea will fail. 


% \textbf{NOPE: WE NEED TO ANALYZE THE EFFECT OF NUMBER OF FRAMES WHY $30$ NOT $15$ In this paper, the value of $k$ is fixed to $30$, as a GoP (Group of Pictures) of the video in most cases contains $30$ frames. }
% \textbf{BEST IS TO TEST WITH $15, 30, 60$}

% \textbf{SHUFFLING THE FRAMES}


\subsection{SDA-picture for Images}
The sda-picture can be used for videos as well as images. [Jessica] proposes $20-30$ images are required to obtain a good quality camera fingerprint. One of the reasons for this limitation is time requirement, i.e. the more images used for fingerprint extraction, the more time it takes. Therefore, one could ignore the rest of the images if the camera has more than $30$ images. The proposed technique can be used in such cases to speed up and/or create a better quality fingerprint in a shorter time. For example, if the camera has $100$ images, instead of omitting $70$ images, a number of sda-pictures can be obtained from all (or most of) the  images. Hence, a similar/better quality fingerprint can be created with less denoising operations. This will increase the I/O load but significantly decrease the memory load. %Note that, if the I/O speed is the bottleneck for a computer, this solution might lead to slowdown, however, the modern computers this difference.........

% \textbf{CAN WE USE IT FOR IMAGE CLUSTERING: i cant see how}



==> sections/old/5b_exp_video2jul.tex <==
% ------------------------------------------
\section{Application to computing video fingerprints}
\label{sec:exp:application}
% In this section, we investigate a more practical use case of the proposed SDA-based technique which is its usage for extracting fingerprints from videos. Specifically, we investigate how performance is affected when at least one of query or known media is a video which can be pristine (i.e., unmodified outside the camera) or from a social media. %As we mentioned in Section~\ref{sec:background}, the most common way to extract fingerprint from videos is to use only I-frames or ALL-frames. 

As Section~\ref{sec:background} explains, two of the most common ways to extract fingerprint are using only I-frames of a video or using all frames (or the first $n$ frames) of it. While the former results in low performance, the latter can be impractical in many real life application due to very high computational needs. For example, fingerprints from $50$ $1-$minute videos (i.e., approx. $1800$ frame per video) using a single-thread may take up to a day. In this section, we provide experimental results that demonstrate how using the SDA frame approach can provide significant improvements in computing fingerprint estimates from video, while retaining the same performance obtained using a significantly larger number of denoising operations using conventional approaches.  %the proposed solution for with the above techniques when at least one of query or known media is a video which can be pristine (i.e., unmodified outside the camera) or from a social media.

In the first experiment, we examine source matching  for  videos. That is given two videos, can we determine if they are from the same camera.  Different types of fingerprints (i.e., I-frames only, SDA-based and ALL-frames) were obtained from each video.   For the sake of simplicity, we refer to them as \textit{I-FE} (i.e., \textit{Fingerprint Estimate}), \textit{SDA-FE}, and \textit{ALL-FE} respectively.  Moreover, in some cases, we add an indication of the SDA-depth when we need to highlight it. For example, SDA-50-FE indicates that the video frames were divided into groups of $50$ and each group averaged to create an SDA-frame.
%In this experiment, we dealt with only pristine videos to avoid other factors that may impact the performance.

Next we investigate a more difficult that involves mixed media. In this subsection, we also analyze two important questions related to mixed media. Those are ``What is a good balance of SDA-depth which optimizes speed and performance?", and ``Does shuffling the frames before obtaining SDA-frames improve the performance?". 

In the next two subsections, we focused on the performance change when the visual objects are obtained from social media such as Facebook and YouTube. %This problem is particularly crucial as social media often involves in large number of visual objects, and the existing fingerprint extraction techniques both have weaknesses in terms of time or performance as mentioned in Section~\ref{sec:background}. So, the proposed method can be useful to in this context.
Finally, we focused on how the proposed technique can be used for moderate length stabilized videos (i.e.,  up to $4$ minutes) from which obtaining a ``reliable" fingerprint might take couple of hours each using all frames. %For example, [DARPA group X/citation] proposes that when stabilized videos are more than $4$ minutes, the attribution using ALL-FEs can reach close to $100\%$, however, extraction of these fingerprints can take up to $4-5$ hours each for a standard PC (e.g., the one we used in our experiments). 

Two datasets were used in all the experiments,  the NYUAD-MMD, and VISION datasets. The NYUAD-MMD dataset contains images and videos of various resolutions and aspect ratios from $78$ cameras from different models and brands. This  makes it a challenging dataset for mixed media attribution. Moreover, it contains stabilized videos longer than $4$ minutes from $5$ cameras. Hence, we used this dataset for experiments using mixed media and stabilized video.
The videos in the dataset are typically around $40$ seconds( i.e., each video is approx. $1200$ frames) and images are pristine (i.e., no out-camera operations). 
The VISION dataset contains different high quality videos and images from social media such as Facebook and YouTube. Hence, we used this dataset in  experiments involving social media. 


{\color{blue}
\subsection{Matching Two Stabilized Videos}
\label{exp:vision:two_vid}
In the first experiment, we examine source matching  for  videos using fingerprints computed from the three different approaches that have been presented.   Our goal was to estimate the length of videos and the resulting computation needed to achieve greater than $99\%$ TPR for I-FEs, SDA-FEs and ALL-FEs. This way, a clear comparison of the the three approaches can be made.

Fingerprints from the non-stabilized videos of the same resolution from the VISION dataset were created. Fingerprints were extracted from the first $5, 10, \dots40$ seconds of each video using the two techniques mentioned in Section~\ref{sec:background} and the proposed method. On average, each video had approx. one I-frame per second. We selected an SDA-depth of $30$ to create an SDA-frame from each second of the videos. So, the number of SDA-frames in this experiment is equal to the the chosen length in seconds (e.g., a $10$ second video has $10$ SDA-frames). 

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={2.9cm 9.5cm 2.8cm 9.5cm},clip] {images/twovid}}
\caption{TPR for different lengths of video using I-Frames, SDA-Frames and ALL-Frames Fingerprint Estimates. }
\label{fig:exp:two_vid}
\end{figure}

Figure~\ref{fig:exp:two_vid} shows TPR using  I-FE, SDA-FE, and ALL-FE as the length of the videos increases. As seen, SDA-FEs outperforms ALL-FEs in this setting for all video lengths. The difference varies between $0.5$ (for $5$ sec videos) and $1.7\%$(for $15$ sec videos). 
Both fingerprints achieve significantly higher TPR than I-FEs. For example, for $10$ seconds video, SDA-frames and ALL-frames result in $94.1\%$ and $95.6\%$ TPR, respectively,  whereas I-frames can only reach $62.2\%$ TPR. 

The highest TPR achieved using I-FEs was $83.7\%$ (i.e., for $40$ second videos) which is still lower than the TPR of SDA- and ALL-FEs when they were computed  from only $5$-second videos (i.e., more than $87\%$). This is because SDA- and ALL-FEs use all the $150$ frames in a 5 second video (i.e., I-, B- or P-frames) whereas the I-FEs use only $40$ I-frames on average and ``waste" the rest of the frames. Hence, for this setting, I-frame based technique fails to reach to a comparable accuracy as the other two methods. 

\begin{table}[!ht]
\centering
\caption{Time for video fingerprint extraction in second}
\vspace{-0.3em}
\begin{tabular}{|c|c|c|c|}
\hline
type           &  averaging & I/O + denoising  & total   \\ \hline
I-FE        & 0          & 50             & 50        \\ \hline
SDA-FE      & 12         & 50             & 62        \\ \hline
ALL-FE      & 0          & 1407           & 1407      \\ \hline
\end{tabular}
\label{tbl:vF_extraction}
\vspace{-1em}
\end{table}

% To understand how much improvement in computation time can be achieved using SDA-frames, we estimated fingerprint extraction time for a 40-second FullHD video captured @30 FPS. 
We then estimated the time required for extraction of fingerprints from a $40$ second Full HD video captured @30 FPS.
Table~\ref{tbl:vF_extraction} compares the average times for these approaches. It takes $50$, $62$, and $1407$ seconds for I-frames, SDA-frames and ALL-frames, respectively. However, these times are when each one is obtained from $40$ second videos. When we evaluate the required time to achieve $83\%$ TPR, we need less than $5$ seconds of video for SDA- and ALL-FEs whereas I-FEs require $40$ seconds of video. This suggest that the required time for SDA- and conventional ways are less than $8$ and $176$ seconds, respectively. Hence, SDA-based technique is at least $6$ times faster than I-FEs and requires $8$ times shorter videos, yet still achieves a higher TPR. Moreover, it performs up to $1.7\%$ higher than ALL-FEs in terms of TPR and speeds up approx. $22.5$ times in this setting. Moreover, while SDA-FEs can achieve $99\%$ TPR with 20 seconds videos, the same can be achieved with $30$ seconds for ALL-FEs. Therefore, close to $34$ times speedup can be achieve in this case when SDA-depth is set to $30$.

% These results show that the superiority of SDA-based fingerprint extraction over I-frame based. An SDA-based approach can easily replace the commonly used I-frame based approach. Moreover, its accuracy is very close to ALL-frames based approach with a speedup of $22$ in computation time. 

Notice that these results involve videos that did not undergo any processing such as scaling, compression in social media and so on. Also, all videos were taken with high luminance in the VISION dataset. %(i.e., no video is with low intensity such as less than)
Therefore, it is possible to have lower performance with more difficult datasets such as when videos are dark or processed. However, our intention here was to demonstrate the effectiveness of SDA approach first for the simplest of cases. We examine more challenging situations in further experiments below. 
}





% -------------------------------------------------------------

\subsection{Mixed Media Attribution}

% Since videos are often long, extracting a fingerprint from I-frames or even all the available frames (ALL-frames) may not cause a significant difference in terms of TPR when two video fingerprints are correlated.
As we have seen in the previous subsection, using only I-frames causes a significant drop in TPR  whereas $20-30$ seconds of video is enough to achieve more than $99\%$ TPR for both SDA-Frames or ALL-Frames approaches. In this subsection, we investigate a more challenging scenario which is matching a video fingerprint to a single image. 

In \cite{taspinar2019source}, source attribution with the mixed-media was investigated using the NYUAD-MMD dataset which contains images and videos of various resolutions from a number of cameras. The videos in the dataset are typically around $40$ seconds long, each having approximately $1200$ frames. Here, we performed ``Train on videos and test on images" experiment for I-, SDA-, and ALL-FEs. The resizing and cropping parameters to perform the matching were obtained from the ``Train on images, test on videos" experiment (for more details, please see~\cite{taspinar2019source}). 

In this subsection, we investigated two important points, namely, the impact of SDA-depth on performance and speed and whether shuffling the frames has an impact on the performance or is SDA-based technique independent of the order.


% In this subsection, we investigated two important points, namely, the impact of SDA-depth on performance and speed and whether shuffling the frames has an impact on the performance or is SDA-based technique independent of the order.


% To analyze how the proposed SDA-based approach performs compared to I-frames and ALL-frames, we performed a ``Train on videos and test on images" experiment. For each video, we created a fingerprint from I-frames, $40$ SDA-frames, and all $1200$ frames of the $40$ second videos. As in the previous experiment SDA-depth is set to $30$. We then resized the images with bilinear scaling using the resizing factors we have learned from the ``Train on images, test on videos" experiment and compare the resized images with the video fingerprints (For more details, please see~\cite{taspinar2019source}). 

% \begin{table}[!ht]
% \centering
% \caption{TPR comparison of I-, SDA-, ALL-frames for ``train on videos, test on images"}
% \vspace{-0.3em}

% \begin{tabular}{ |c|c|c|c|c| } 
%     \hline
%     type           & $\#match$ & $\#comparison$  & $ TPR $  & $\overline{PCE}$ \\  \hline
%     I-frame        &   15070   & 23571    & 63.93\%      &  379  \\  \hline
%     SDA-frame      &   18849   & 23571    & 79.97\%      &  844  \\  \hline
%     ALL-frame      &   19598   & 23571    & 83.14\%      &  879  \\  \hline
% \end{tabular}
% \label{table:vF2iN}
% \vspace{-0.3em}
% \end{table}


% Table~\ref{table:vF2iN} compares the average PCE and TPR when fingerprint is obtained using these three approaches. When the fingerprints are obtained using only I-frames, $63.93\%$ of the images can be correctly attributed to their sources, and $83.14\%$ when ALL-frames are used. The proposed SDA-based approach achieve slightly less that ALL-frames with TPR of $79.97\%$. %As seen, SDA-frame achieves $4.89\%$ less than ALL-frames and $14.89\%$ more than I-frames which shows it can be used as a middle way between I-frames only and ALL-frames approaches. 

% Notice that, the choice of SDA-depth (i.e., $30$) was just used for comparison purpose. In the next experiment, we investigate what is a good value for the SDA-depth that can give optimal performance in terms of time and speed.
% % The results show that choosing only I-frames due to its low time-complexity is not the most effective solution in terms of performance for difficult cases such as mixed media. On the other hand, 



\paragraph{Number of frames averaged in SDA-frame}
Here, we examined how performance changes as the SDA-depth (i.e., $d$) changes. Given a video of $m$ frames (in our case approx. $1200$ frames), we divided the frames into groups of $d = 1, 5, 10, 30, 50, 200, 1200$. Therefore, the number of SDA-frames,$g$, became $1200, 240, 120, 40, 24, 6, 1$ SDA-frames were created, respectively. When $g = 1$, the technique becomes same as using all frames whereas when $p = 1200$, only a single frame is created by averaging all frames. 
Similar to the previous experiment, each of these fingerprints were then correlated to the PRNU noise all the test images from the same camera.

Figure~\ref{figure:experiment:num_image_sda} shows the ROC curves for each SDA-FEs as well as I-FEs and ALL-FEs. The results show that ALL-FEs results in the highest performance, whereas I-FEs perform significantly poorer compared to others. The proposed SDA-based method performs close to conventional method for all depths. 

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={0.9cm 8.1cm 0.9cm 8cm}, clip]{images/sda_depth_roc.pdf}}
\caption{The ROC curves for varying SDA-depths}
\label{figure:experiment:num_image_sda}
\end{figure}


Table~\ref{tbl:sda_depth} shows more details about the results. $|\overline{PCE}|$ stands for average of the PCE ratios with respect to I-FEs. For example, when an ALL-FE from $i^{th}$ video is correlated with the noise of $j^{th}$ image, its PCE is on average $3.2\%$ times higher compared to the $I-FE$ obtained from the same video. The reason we used this parameter instead of average PCE is outliers have a big impact on average PCE. %For example, PCE of a few $SDA-1200-FE$ is close to $20,000$ higher compared to ALL-FE from the same video, which 
Moreover, the table shows the TPR for the PCE threshold of $60$, average time to extract fingerprint and the speedup compared to ALL-FEs. As seen, the results indicate that the TPR of SDA-based method are very close to conventional method, however, up to $52$ times speedup can be achieved using the SDA-based method. %In addition to these, the slim performance drop in sda-based technique can easily be overcome by using more of the available frames (when the video is longer than $40$ seconds) which may have a small increase in fingerprint computation. 

\begin{table}[!ht]
\centering
\renewcommand*{\arraystretch}{1.15}
\caption{Sda-depths}
\label{tbl:sda_depth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
            	 &I-FE    & ALL-FE 	& 5 	& 10   & 30   & 50   & 200  & 1200 \\ \hline
$|\overline{PCE}|$ & 1.00 & 3.20 & 3.05 & 2.88 & 2.64 & 2.58 & 2.50 & 2.42  \\ \hline
% $\overline{PCE}$ &379   & 879  	& 864	& 852  & 845  & 852  & 876	& \textbf{925}  \\\hline
TPR($\%$)	     &64.0  & \textbf{83.1} 	& 82.3	& 81.3 & 80.0 & 79.8 & 80.1 & 79.8 \\\hline
% auc              & 85.3 & 94.6  & 94.1  & 93.6 & 92.9 & 92.7 & 93.1 & 93.5 \\ \hline
time(s)          & 50   & 1407	&  276	& 142  & 62   & 48   &	32	& \textbf{27}   \\ \hline
speedup          &28.1 & 1.0 & 5.1 & 9.9 & 22.7 & 29.3 & 44.0 & \textbf{52.1}\\ \hline
\end{tabular}
\end{table}

Similar to the previous experiment using I-FEs have significantly lower accuracy. Approx. $16\%$ lower TPR (for SDA-depth $\geq 30$) doesn't help to have any speedup. 

Notice that when ALL-FEs are used, it takes approx. five days to extract all the fingerprints from the only $301$ videos of NYUAD-MMD in a single-threaded implementation which makes it impractical to use all frames for any real life applications.






\subsection{Train and test on YouTube videos}

This experiment explores the performance achieved when two video fingerprints from YouTube are correlated. Although this experiment is essentially the same as the Section~\ref{exp:vision:two_vid}, it is crucial as high compression is involved in for this case. We created fingerprints from all non-stabilized YouTube videos (i.e., the ones labeled flatYT, indoorYT, and outdoorYT) using only I-frames, SDA-$50$, SDA-$100$, SDA-$200$, and ALL-frames. Here, we used the first $10, 20, \dots 60$ seconds of YouTube videos to extract the above fingerprints. Each $60$ second video has approx $1800$ frames that are used for SDA- or ALL-FEs, whereas they contained $31.3$ I-frames on average. 
After fingerprint extraction, we correlate each video fingerprint with the others of the same type and same length taken by the same camera. For example, an I-FE from $20$ second of video is correlated with all I-FEs obtained from the rest of $20$ seconds videos from the same camera.
The same is valid for SDA- and ALL-FEs. This way, a total of $3124$ correlation has been done for each type.

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={2.9cm 9.5cm 2.8cm 9.5cm},clip] {images/youtube}}
\caption{The effect of texture in terms of PCE}
\label{fig:exp:youtube}
\end{figure}


Figure~\ref{fig:exp:youtube} shows the TPR for varying video lengths for each FE type. The figure shows that I-FEs perform very poorly for all cases that any fingerprint type more than $20$ seconds outperforms I-FEs. While ALL-FEs perform higher than SDA-FEs for the same-length videos, which has also been suggested in Section~\ref{sec:approach}. This difference can be overcome by increasing the video length. For example, SDA$-50$ obtained from $50$ seconds videos or SDA$-100$ from $60$ seconds videos, perform approx. the same as ALL-FEs obtained from $30$ seconds (within $\mypm1\%$ TPR range). Hence, instead of using $900$ frames for ALL-FEs, using $1800$ frames for SDA$-100$ can help speedup significantly with no loss in TPR. While an ALL-FE from $900$ frame of a Full HD video takes $1045$ seconds to extract, and SDA$-100$ from $1800$ frames, which only does $18$ denoising instead of $900$, takes $56$ seconds. Therefore, a speedup of close to $19$ times can be achieved with SDA$-100$ with $1\%$ increase in TPR. Notice that, because most videos are around $60$ seconds on VISION dataset, it limits the maximum length we can use in the experiments. 

% In our experiments, a total $350$ videos from YouTube were used, most of them being HD resolution (i.e., $1280\times720$). When ALL-FEs are extracted from $60$ seconds of each of these videos, it takes at least four days which indicates any identification system collects YouTube videos cannot be practical if ALL-FEs are used. 

% Table~\ref{tbl:exp:ns:2yt} show that the fingerprints from I-frames results in significantly worse performance compared to SDA- and ALL-frames. Moreover, extracting fingerprint using ALL-frames is $30-50$ times slower compared SDA-frames while the performance is $10-19\%$ higher. These results differs slightly from the previous results. One reason the videos that are labeled ``still" and ``outdoor" tend to give lower PCE values for fingerprint from SDA-frames compared to ALL-frames.

% \begin{table}[!ht]
% \centering
% \caption{TPR for train and test YouTube videos experiment}
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
%     & I-     & SDA-$50$  & SDA-$200$ & SDA-$600$ & ALL-   \\ \hline
% TPR & 29.29   & 59.54    & 54.58     & 50.74     & 69.62  \\ \hline
% \end{tabular}
% \label{tbl:exp:ns:2yt}
% \end{table}


\subsection{Train on Facebook images, test on YouTube videos}
From the previous experiments, we know that the SDA-based fingerprint extraction can help achieve a significant speedup for both videos and images with a very small loss in performance which can be overcome by increasing the number of still images used for fingerprint extraction if available. In this part, our goal is to show that the proposed method can be successfully applied to other social media. Specifically, in this part, we will do ``Train on Facebook images, test on YouTube videos" experiment. The importance of this experiment is both media sharing services contains billions of visual media that the conventional fingerprint extraction approaches from these web pages has very high time complexity. Therefore, fingerprint extraction methods (along with search techniques) that speeds up the search is highly crucial.

In this experiment, for the camera in VISION dataset that has non-stabilized videos, we created fingerprints from $100$ Facebook images (i.e., the ones labeled FBH) using conventional fingerprint extraction methods. 
We then used the already created fingerprints from non-stabilized YouTube videos (see previous experiment). We again used I-frames, SDA-$50$, SDA-$200$, SDA-$600$, and ALL-frames that are computed from the first $60$ seconds of YouTube videos.

In this experiment, we correlated the image fingerprints with each video fingerprint of each type using the efficient search proposed in ~\cite{taspinar2019source} and a total of $343$ pair have been compared for each fingerprint type. 

Table~\ref{tbl:exp:ns:fb_yt} shows the TPR of these correlations. Similar to ``Train on videos, test on images" experiment, these results show that for fingerprints obtained from Facebook images matches with $81.34\%$ of the videos for SDA-$50$ which is higher than both ALL-frames and I-frames. On the other hand, the fingerprints from I-frames yield approx. $30\%$ lower TPR for this setting. This results show that SDA-based approach is a good replacement for usage of I-frames or ALL-frames for this case.

\begin{table}[!ht]
\centering
\caption{TPR of different fingerprint types when a fingerprint from Facebook images and another from  YouTube videos are correlated}
\label{tbl:exp:ns:fb_yt}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & I-FE   & SDA-$50$  & SDA-$200$ & SDA-$600$ & ALL-FE   \\ \hline
TPR & 51.60  &  81.4     & 79.88     & 78.13     & 79.59    \\ \hline
\end{tabular}
\end{table}

% These results also show that SDA-based technique is always superior compared to I-frames based in terms of performance and comparable in terms of speed. 

% \subsection{{\color{blue} Train on pristine videos, test on YouTube videos}}
% \subsection{{\color{blue} Train on non-stabilized, test on stabilized videos}}



% ------------------------------------------
\subsection{Non-Stabilized videos}
% \label{sec:exp:stab}

A recent work [cite] has shown that a fingerprint obtained from a long stabilized video can successfully be matched with other videos from the same camera. However, as above, thousands of frames must be denoised for this which may not be practical in some settings. A potential alternative for this problem is the usage of SDA-frames which may lead to a significant speed up. To evaluate this, we captured long stabilized videos from $5$ cameras, a total of $37$ videos which adds up to $260$ minutes. As shown in \cite{taspinar2016source, iuliani2017hybrid}, the first frame of the videos are typically not geometrically transformed. But as \cite{mandelli2019facing} pointed out, they may not always be available or some cameras may transform them as well, hence, we ignored those frames.

For this experiment, we extracted fingerprints from the frames of $20, 40, \dots 240$ seconds using conventional method as well as SDA-based method for SDA-depth of $30, 50,$ and $200$ as these are reasonable choices from the previous experiments.
We correlated each fingerprint with other fingerprints of different videos from the same camera that are created using the same number of frames. For example, SDA-30 fingerprints of $20$ second videos are correlated with the same type fingerprints from the same camera. 

Figure~\ref{figure:exp:stab_res} shows the TPR for three cameras (i.e., Huawei Honor, Samsung S8, and iPhone 6plus) and the total average of all the five cameras. 

% The results show that as the videos get longer, the TPR increases which supports the idea proposed in [the recent study/cite].   



\begin{figure} [!ht]
\centering
{\includegraphics[trim={1.2cm 8cm 1.4cm 8.3cm}, clip, keepaspectratio=true,width=\linewidth]{images/total_stab3.pdf}}
% {\includegraphics[trim={2.75cm 9.3cm 2.75cm 9.3cm}, clip, keepaspectratio=true,width=\linewidth]{images/stab_res.pdf}}
\caption{TPR for stabilized videos for varying SDA-depths}
\label{figure:exp:stab_res}
\end{figure}

The results show that as videos get longer, fingerprints obtained using conventional or SDA-based approach get more reliable. Moreover, the effect of increased SDA-depth is more significant for this case in comparison to non-stabilized videos. %This is because SDA-based approach performs poorly for iPhone cameras whereas for others, the performance is not almost as good as conventional approach. Figure X shows TPR of 

While for some cameras conventional and SDA-based approaches perform similarly (Huawei and Samsung cameras), for others (i.e., iPhone cameras) there is a significant difference between the two. For example, for Samsung S8 $SDA-200$ fingerprint from $120$ seconds video, perform similarly as $180$ seconds conventional fingerprint. Therefore, for this particular case, $SDA-200$ can speedup $66$ times \big(i.e. $\frac{180}{120}\times \frac{1407}{32}$\big)(see Table~\ref{tbl:sda_depth} for times). On the other hand for iPhone 6 plus, $60$ seconds video with conventional and $160$ seconds $SDA-50$ have similar TPR. Therefore, $11x$ \big(i.e., $\frac{60}{160}\times \frac{1407}{48}$\big) speedup can be achieved in this case. Overall, a speedup between these numbers (i.e. $11$ and $60$) can be achieved without any loss in TPR if a long video is available.


Overall, this subsection shows that the proposed SDA-based fingerprint extraction outperforms  the commonly used I-frame-only technique in all the cases for videos. These include for mixed media, stabilized videos, and social media. On the other hand, the SDA-based method achieves comparable results as ALL-frames-used fingerprint extraction with up to 50 times speedup. We also show the impact of SDA-depth on the performance that can be achieved in various cases. Finally, we show that SDA-based method order of frames doesn't have an impact on performance, yet shuffling the frames cause either a significant slow down or high I/O cost. Therefore, ordered access to videos is preferable to random access.



% \subsection{Seam carved video} --> this can be itself a short paper?




% \subsection{Train and test on short videos}
% {\color{red} Another challenging source identification cases that researchers often encounters is when at least one of the fingerprints is a short video. In other words, either query or known video is a less than couple of seconds. In such a case fingerprints extracted from such videos are not often not reliable due to low number of highly compressed video frames. In DARPA Camera Identification Challenge~\cite{darpa2018medifor}, $4$ of $6$ challenges involved in videos that are quite short. 

% In this subsection, we evaluate how SDA-based technique will perform in such a highly challenging case. To evaluate this, we used SOCRatES dataset~\cite{galdisocrates} which contains a total of $1046$ videos from $96$ cameras. These videos are typically one to five seconds. We created $3$ fingerprints from each video in the dataset: using only I-frames, a single SDA-frame where the SDA-frame is the average of all available frames of the camera (we call this SDA-n where n is the total number of frames), and ALL-frames. 
% For this experiment, we correlated each fingerprint with the rest of the fingerprints of the same type from the same camera (i.e., fingerprints from I-frames correlated only with each other etc.). If none of the video fingerprints match (i.e., PCE $> 60$) for a camera, we considered that the videos are all stabilized and skipped the camera. Otherwise, we obtained their PCE scores for all those correlations. 

% In the dataset, the average number of frames per video is A, and average I-frames is B. Hence for I-frame only technique B and for ALL-frames A denoising operation is performed. On the other hand, only one denoising operation is done for SDA-based technique which makes it faster than I-frame only technique. (i.e., average times is a,b,c for I-, SDA- and ALL-frame based techniques respectively.)

% Table X shows the average PCE and the TPR for this experiment. As the table shows, fingerprint from I-frames performs very poorly that the accuracy is very low. On the other hand 

% \begin{table}[!ht]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
%               & I-frames & SDA-n & ALL-frames \\ \hline
% \#frames      & & 1 &               \\ \hline
% time(sec)     & & &                 \\ \hline
% PCE & 2792    & 7911  &  13895      \\ \hline
% TPR & 26.34   & 50.77 &  57.30      \\ \hline

% \end{tabular}
% \end{table}


% Notice that, in this experiment, some of the videos may still be stabilized, hence, drop the TPR for each technique. However, since our goal is to determine relative performance of these techniques, the impact of stabilized videos is irrelevant with the experiment.

% }


% \subsection{stability check}
% Another important issue that 

==> sections/old/5b_exp_video_backup.tex <==
% ------------------------------------------
\section{Application to computing video fingerprints}
\label{sec:exp:application}
In this section, we investigate a more practical use case of the proposed SDA-based technique which is its usage for extracting fingerprints from videos. Specifically, we investigate how performance is affected when at least one of query or known media is a video which can be pristine (i.e., unmodified outside the camera) or from a social media. %As we mentioned in Section~\ref{sec:background}, the most common way to extract fingerprint from videos is to use only I-frames or all-frames. 

In the first step, we analyzed the most intuitive source attribution case for videos which is the comparison of two videos. In this case, different types of fingerprints (i.e., I-frames only, SDA-based and all-frames) obtained from a video compared against others from the same camera. For the sake of simplicity, we refer \textit{I-FE} (i.e., \textit{Fingerprint Estimate}), \textit{SDA-FE}, and \textit{all-FE} to indicate fingerprints obtained using different types of frames. Moreover, in some cases, we add the SDA-depth to SDA-FE when we prefer to highlight it. For example, SDA-50-FE indicates that the frames of video, $m$, is divided into groups of $50$ and each group is average to create an SDA-frame.
In this experiment, we dealt with only pristine ones to avoid other factors that may impact the performance.

Secondly, we investigated a more difficult use case which is the accuracy on mixed media. In this subsection, we also analyzed two important questions related to mixed media. Those are ``What is a good balance of SDA-depth which optimizes speed and performance?", and ``Does shuffling the frames before obtaining SDA-frames improve the performance?". 

In the next two subsections, we focused on the performance change when the visual objects are obtained from social media such as Facebook and YouTube. This problem is particularly crucial as social media often involves in large number of visual objects, and the existing fingerprint extraction techniques both have weaknesses in terms of time or performance as mentioned in Section~\ref{sec:background}. So, the proposed method can be useful to in this context.

Finally, we focused on how the proposed technique can be used for moderate length stabilized videos (i.e.,  up to $4$ minutes) from which obtaining a ``reliable" fingerprint might take couple of hours each. For example, [DARPA group X/citation] proposes that when stabilized videos are more than $4$ minutes, the attribution using all-FEs can reach close to $100\%$, however, extraction of these fingerprints can take up to $4-5$ hours each for a standard PC (e.g., the one we used in our experiments). 

For this section, we used two datasets that are NYUAD-MMD, and VISION both of which have different strengths. NYUAD-MMD contains images and videos of various resolutions and aspect ratios from $78$ cameras with various models and brands which makes it a challenging dataset for mixed media attribution. Moreover, it contains stabilized videos longer than $4$ minutes from $5$ cameras. Hence, we used this dataset for mixed media and stabilization experiments.
%The videos in the dataset are typically around $40$ seconds( i.e., each video is approx. $1200$ frames) and images are pristine (i.e., no out-camera operations). 
On the other hand, The VISION dataset contains various pristine videos and visual objects from social media such as Facebook and YouTube. Hence, we used this dataset in the first experiment and social media experiments. %In this section, the term ``video" we will refer to non-stabilized videos unless otherwise is stated.

% As mentioned in the Section~\ref{sec:background}, a video fingerprint can be extracted from I-frames or all-frames. Although, fingerprint from I-frames is faster to extract, the letter one creates a more reliable fingerprint, hence, likely to achieve higher performance. %In this subsection, we first investigate (i) the TPR for the mixed media case in NYUAD-MMD. We then analyze (ii) the number of frames in an SDA-frame, (iii) whether order of frames have an impact, %(iv) the number of frames that is required for conventional method perform a similar performance as SDA-based method, 
% and finally, we evaluated (v) and (vi) the performance on YouTube and %WhatsApp. %The experiments in this subsection were done using NYUAD-MMD except (v) and (vi) for which we have used VISION dataset.

{\color{blue}
\subsection{Train and test on videos}
\label{exp:vision:two_vid}
Since comparison of two non-stabilized videos is the easiest/most natural/intuitive case for video source attribution, in this subsection, we investigated this case as the first step.
To be more precise, our goal is to estimate the length of videos needed to achieve more than $99\%$ TPR for I-FEs, SDA-FEs and all-FEs. This way, a clear comparison of the fingerprints can be made.

For this purpose, we created fingerprints from the non-stabilized videos of VISION dataset all of which are same resolution. The reason we choose the same resolution videos is to prevent an extra phase of downsizing which may lead to a decrease in the TPR. We extracted fingerprints from the first $5, 10, \dots40$ seconds of each video using the two techniques mentioned in Section~\ref{sec:background} and the proposed method. On average, each video had approx. one I-frame per second. We selected SDA-depth as $30$ to create an SDA-frame from each second of the videos. So, the number of SDA-frame in this experiment is equal to the the chosen length in seconds (e.g., a $10$ second video has $10$ SDA-frames). 

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={2.9cm 9.5cm 2.8cm 9.5cm},clip] {images/twovid}}
\caption{The effect of texture in terms of PCE}
\label{fig:exp:two_vid}
\end{figure}

Figure~\ref{fig:exp:two_vid} shows the TPR for I-, SDA-, and all-FEs as the length of the videos increase. As seen, SDA-FEs outperforms all-FEs in this setting for all video lengths. This difference varies between $0.5$ (for $5$ sec videos) and $1.7\%$(for $15$ sec videos). 
Both fingerprints achieve significantly better accuracy that I-FEs. For example, when videos are $10$ seconds, SDA-based and all-frames performs $94.1\%$ and $95.6\%$ TPR, respectively, whereas fingerprint from only I-frames, reaches to only $62.2\%$ TPR. 

The highest TPR achieved using I-FEs is $83.7\%$ (i.e., when the videos are $40$ seconds) which is still lower than the TPR of SDA- and all-FEs when they are obtained from $5$-second videos (i.e., more than $87\%$).

This is because SDA- and all-FEs use $150$ frames of all types (i.e., I-, B- or P-frames) whereas the I-FEs use only $40$ I-frames on average and ``waste" the rest of the frames. Hence, for this setting, I-frame based technique fails to reach to a comparable accuracy as the other two methods. 

\begin{table}[!ht]
\centering
\caption{Time for video fingerprint extraction in second}
\vspace{-0.3em}
\begin{tabular}{|c|c|c|c|}
\hline
type           &  averaging & I/O + denoising  & total   \\ \hline
I-FE        & 0          & 50             & 50        \\ \hline
SDA-FE      & 12         & 50             & 62        \\ \hline
all-FE      & 0          & 1407           & 1407      \\ \hline
\end{tabular}
\label{tbl:vF_extraction}
\vspace{-1em}
\end{table}

% To understand how much improvement in computation time can be achieved using SDA-frames, we estimated fingerprint extraction time for a 40-second FullHD video captured @30 FPS. 
We then estimated the time required for extraction of fingerprints from a $40$ second Full HD video captured @30 FPS.
Table~\ref{tbl:vF_extraction} compares the average times for these approaches. It takes $50$, $62$, and $1407$ seconds for I-frames, SDA-frames and all-frames, respectively. However, these times are when each one is obtained from $40$ second videos. When we evaluate the required time to achieve $83\%$ TPR, we need less than $5$ seconds of video for SDA- and all-FEs whereas I-FEs require $40$ seconds of video. This suggest that the required time for SDA- and conventional ways are less than $8$ and $176$ seconds, respectively. Hence, SDA-based technique is at least $6$ times faster than I-FEs and requires $8$ times shorter videos, yet still achieves a higher TPR. Moreover, it performs up to $1.7\%$ higher than conventional way in terms of TPR and speeds up approx. $22.5$ times in this setting. Moreover, while SDA-FEs can achieve $99\%$ TPR with 20 seconds videos, the same can be achieved with $30$ seconds for all-FEs. Therefore, close to $34$ times speedup can be achieve in this case when SDA-depth is set to $30$.

% These results show that the superiority of SDA-based fingerprint extraction over I-frame based. An SDA-based approach can easily replace the commonly used I-frame based approach. Moreover, its accuracy is very close to all-frames based approach with a speedup of $22$ in computation time. 

Notice that these results are showing almost the best case scenario as the videos did not undergo any processing such as scaling, compression in social media and so on. Also, all videos are taken with high luminance in VISION dataset. %(i.e., no video is with low intensity such as less than)
Therefore, it is possible to have lower performance with more difficult datasets such as when videos are dark or processed. 
}





% -------------------------------------------------------------

\subsection{Train on video, test on images}

% Since videos are often long, extracting a fingerprint from I-frames or even all the available frames (all-frames) may not cause a significant difference in terms of TPR when two video fingerprints are correlated.
As we have seen in the previous subsection, using only I-frames causes a significant drop in TPR in any case we examined (i.e., all videos less than $40$ seconds in our experiment) whereas $20-30$ seconds of videos is enough to achieve more than $99\%$ TPR for both SDA- or all-FEs. In this subsection, we investigate a more challenging scenario which is matching a video fingerprint to a single image. 

In \cite{taspinar2019source}, we investigated TPR with the mixed-media in NYUAD-MMD which contains images and videos of various resolutions from a number of cameras. The videos in the dataset were typically around $40$ seconds long, each having approximately $1200$ frames. To analyze how the proposed SDA-based approach performs compared to I-frames and all-frames, we performed a ``Train on videos and test on images" experiment. For each video, we created a fingerprint from I-frames, $40$ SDA-frames, and all $1200$ frames of the $40$ second videos. As in the previous experiment SDA-depth is set to $30$. We then resized the images with bilinear scaling using the resizing factors we have learned from the ``Train on images, test on videos" experiment and compare the resized images with the video fingerprints (For more details, please see~\cite{taspinar2019source}). 

\begin{table}[!ht]
\centering
\caption{TPR comparison of I-, SDA-, all-frames for ``train on videos, test on images"}
\vspace{-0.3em}

\begin{tabular}{ |c|c|c|c|c| } 
    \hline
    type           & $\#match$ & $\#comparison$  & $ TPR $  & $\overline{PCE}$ \\  \hline
    I-frame        &   15070   & 23571    & 63.93\%      &  379  \\  \hline
    SDA-frame      &   18849   & 23571    & 79.97\%      &  844  \\  \hline
    all-frame      &   19598   & 23571    & 83.14\%      &  879  \\  \hline
\end{tabular}
\label{table:vF2iN}
\vspace{-0.3em}
\end{table}


Table~\ref{table:vF2iN} compares the average PCE and TPR when fingerprint is obtained using these three approaches. When the fingerprints are obtained using only I-frames, $63.93\%$ of the images can be correctly attributed to their sources, and $83.14\%$ when all-frames are used. The proposed SDA-based approach achieve slightly less that all-frames with TPR of $79.97\%$. %As seen, SDA-frame achieves $4.89\%$ less than all-frames and $14.89\%$ more than I-frames which shows it can be used as a middle way between I-frames only and all-frames approaches. 

Notice that, the choice of SDA-depth (i.e., $30$) was just used for comparison purpose. In the next experiment, we investigate what is a good value for the SDA-depth that can give optimal performance in terms of time and speed.
% The results show that choosing only I-frames due to its low time-complexity is not the most effective solution in terms of performance for difficult cases such as mixed media. On the other hand, 


% Instead of using only I-frames, SDA-based approach may significantly 

% These results show that the proposed approach can be a middle solution for fingerprint extraction from videos. %This technique compromises from performance to achieve a significant speed up.
% Furthermore, as mentioned in Section~\ref{sec:approach:sda_picture}, when the video is long enough (i.e. few minutes), more frames can be used in SDA-frame which is expected to improve the performance.




\paragraph{Number of frames averaged in SDA-frame}
Next, we examined how performance changes as the SDA-depth (i.e., $d$) changes. Given a video of $m$ frames (in our case approx. $1200$ frames), we divided the frames into groups of $d = 1, 5, 10, 30, 50, 200, 1200$. Therefore, the number of SDA-frames,$g$, became $1200, 240, 120, 40, 24, 6, 1$ SDA-frames were created, respectively. When $g = 1$, the technique becomes same as using all frames whereas when $p = 1200$, only a single frame is created by averaging all frames. 
Similar to the previous experiment, each of these fingerprints were then correlated to the PRNU noise all the test images from the same camera.

Figure~\ref{figure:experiment:num_image_sda} shows the ROC curves for each SDA-depth as well as I-frames-only and all-frames. The results show that the conventional fingerprint extraction method results in the highest performance, whereas I-frame-only scheme performs significantly poorer compared to others. The proposed SDA-based method performs close to conventional method for all depths.

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={0.9cm 8.1cm 0.9cm 8cm}, clip]{images/sda_depth_roc.pdf}}
\caption{The ROC curves for varying SDA-depths}
\label{figure:experiment:num_image_sda}
\end{figure}


Table~\ref{tbl:sda_depth} shows more details about the results as well as TPR when PCE threshold is set to $60$, average PCE, and average time it takes to create a fingerprint. As seen, the results indicate that the TPR of SDA-based method are very close to conventional method, however, up to $50$ times speedup can be achieved using the SDA-based method. In addition to these, the slim performance drop in sda-based techniques can easily be overcome by using more of the available frames (when the video is longer than $40$ seconds) which may have a small increase in fingerprint computation. 


\begin{table}[!ht]
\centering
\renewcommand*{\arraystretch}{1.15}
\caption{Sda-depths}
\label{tbl:sda_depth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
            	 &I-    & all- 	& 5 	& 10   & 30   & 50   & 200  & 1200 \\\hline
$\overline{PCE}$ &379   & 879  	& 864	& 852  & 845  & 852  & 876	& 925  \\\hline
TPR($\%$)	     &64.0  & 83.1 	& 82.3	& 81.3 & 80.0 & 79.8 & 80.1 & 79.8 \\\hline
% auc              & 85.3 & 94.6  & 94.1  & 93.6 & 92.9 & 92.7 & 93.1 & 93.5 \\ \hline
time(s)          & 50   & 1407	&  276	& 142  & 62   & 48   &	32	& 27   \\ \hline
speedup          &28.1 & 1.0 & 5.1 & 9.9 & 22.7 & 29.3 & 44.0 & 52.1\\ \hline
\end{tabular}
\end{table}

On the other hand, using I-frames only approach performs poorly compared to all other methods. Moreover, it does not achieve any speedup compared to SDA-based method when SDA-depth is greater than $50$. Notice that when all-frames are used, it takes approx. five days to extract all the fingerprints from the $301$ videos in NYUAD-MMD in a single-threaded implementation which makes it infeasible to use all frames in many applications. 



\paragraph{Order of frames}
Since a video is an ordered set of frames, each frame has significant similarity with the previous and next frame. This section analyzes if the order of video has any impact on the proposed approach. In other words, our goal is to evaluate whether the TPR will change if the video frames are shuffled before SDA-frames are created. For this purpose, we compared the TPR of when the images in SDA-frames are ordered and they are shuffled in the same experimental setting  used above for the SDA-depths experiment. Clearly, for SDA-depth of $1$ and $1200$, there will be no difference because the same SDA-frame(s) will be denoised and averaged.  

\begin{table}[!ht]
\centering
\caption{Effect of order of frames on TPR($\%$)}
\label{table:exp:order}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
           & $1$    & $5$   & $10$  & $30$  & $50$  & $200$ & $1200$ \\ \hline
ordered    & 83.14 	& 82.25	& 81.30 & 79.97 & 79.85 & 80.05 & 79.77  \\ \hline
shuffled   & 83.14  & 82.35 & 81.32 & 80.09 & 79.82 & 80.15 & 79.77  \\ \hline
\end{tabular}

\end{table}

As seen in Fig.~\ref{table:exp:order}, the order of frames doesn't have a significant impact on TPR (i.e., approx. $0.05$ higher TPR on average).  However, random access to frames is not as efficient as ordered access. Since P- and B- frames requires previous I-frames to be read first which makes  shuffled access significantly slower. For example, when the SDA-depth is $30$, a fingerprint from the same video (as in Table~\ref{tbl:vF_extraction}) takes $299$ seconds with random access instead of $63$ seconds. If all the frames are extracted first, approx. 7 GB temporary storage is required for an uncompressed image format which also will increase the I/O time. Hence, the ordered version is favorable given that a negligible performance improvement of shuffling comes at an expense of significant increase in either storage usage or time requirement. 



\subsection{Train and test on YouTube videos}

This experiment explores the performance achieved when two video fingerprints from YouTube are correlated. Although this experiment is essentially same as the Section~\ref{exp:vision:two_vid}, it is crucial as compression is involved in for this case. We created fingerprints from all non-stabilized YouTube videos (i.e., the ones labeled flatYT, indoorYT, and outdoorYT) using only I-frames, SDA-$50$, SDA-$200$, SDA-$600$, and all-frames. Here, we used the first $60$ seconds of YouTube videos to extract the above fingerprints. When we use SDA- or all-frames, we approx. use $1800$ frames for each video whereas for the first $60$ seconds of the videos have $31.3$ I-frames on average. 
We then correlate each video fingerprint with the others of the same type taken by the same camera. In other words, the fingerprints obtained from I-frames are correlated only the ones extracted using I-frames. The same is valid for SDA- and all-frames. This way, a total of $3124$ correlation has been done for each type. 

Table~\ref{tbl:exp:ns:2yt} show that the fingerprints from I-frames results in significantly worse performance compared to SDA- and all-frames. Moreover, extracting fingerprint using all-frames is $30-50$ times slower compared SDA-frames while the performance is $10-19\%$ higher. These results differs slightly from the previous results. One reason the videos that are labeled ``still" and ``outdoor" tend to give lower PCE values for fingerprint from SDA-frames compared to all-frames.

\begin{table}[!ht]
\centering
\caption{TPR for train and test YouTube videos experiment}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & i-     & SDA-$50$  & SDA-$200$ & SDA-$600$ & all-   \\ \hline
TPR & 29.29   & 59.54    & 54.58     & 50.74     & 69.62  \\ \hline
\end{tabular}
\label{tbl:exp:ns:2yt}
\end{table}

Even though an SDA-based technique provides lower performance compared to an all-frame-based approach for YouTube videos, this drawback can easily be overcome by increasing the number of frames used by SDA-based approach. {\color{blue}Since YouTube videos are often longer than $60$ seconds, this solution can be easily applied in such cases with a small increase in time.}

\subsection{Train on Facebook images, test on YouTube videos}
From the previous experiments, we know that the SDA-based fingerprint extraction can help achieve a significant speedup for both videos and images with a very small loss in performance which can be overcome by increasing the number of still images used for fingerprint extraction if available. In this part, our goal is to show that the proposed method can be successfully applied to other social media. Specifically, in this part, we will do ``Train on Facebook images, test on YouTube videos" experiment. The importance of this experiment is both media sharing services contains billions of visual media that the conventional fingerprint extraction approaches from these web pages has very high time complexity. Therefore, fingerprint extraction methods (along with search techniques) that speeds up the search is highly crucial.

In this experiment, for the camera in VISION dataset that has non-stabilized videos, we created fingerprints from $100$ Facebook images (i.e., the ones labeled FBH) using conventional fingerprint extraction methods. 
We then used the already created fingerprints from non-stabilized YouTube videos (see previous experiment). We again used I-frames, SDA-$50$, SDA-$200$, SDA-$600$, and all-frames that are computed from the first $60$ seconds of YouTube videos.

In this experiment, we correlated the image fingerprints with each video fingerprint of each type using the efficient search proposed in ~\cite{taspinar2019source} and a total of $343$ pair have been compared for each fingerprint type. 

Table~\ref{tbl:exp:ns:fb_yt} shows the TPR of these correlations. Similar to ``Train on videos, test on images" experiment, these results show that for fingerprints obtained from Facebook images matches with $81.34\%$ of the videos for SDA-$50$ which is higher than both all-frames and I-frames. On the other hand, the fingerprints from I-frames yield approx. $30\%$ lower TPR for this setting. This results show that SDA-based approach is a good replacement for usage of I-frames or all-frames for this case.

\begin{table}[!ht]
\centering
\caption{TPR of different fingerprint types when a fingerprint from Facebook images and another from  YouTube videos are correlated}
\label{tbl:exp:ns:fb_yt}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & i-     & SDA-$50$  & SDA-$200$ & SDA-$600$ & all-   \\ \hline
TPR & 51.60  &  81.34    & 79.88    & 78.13      & 79.59  \\ \hline
\end{tabular}
\end{table}

These results also show that SDA-based technique is always superior compared to I-frames based in terms of performance and comparable in terms of speed. 

% \subsection{{\color{blue} Train on pristine videos, test on YouTube videos}}
% \subsection{{\color{blue} Train on non-stabilized, test on stabilized videos}}



% ------------------------------------------
\subsection{Stabilized videos}
% \label{sec:exp:stab}

A recent work [cite] has shown that a fingerprint obtained from a long stabilized video can successfully be matched with other videos from the same camera. However, as above, thousands of frames must be denoised for this which may not be practical in some settings. A potential alternative for this problem is the usage of SDA-frames which may lead to a significant speed up. To evaluate this, we captured long stabilized videos from $5$ cameras, a total of $37$ videos which adds up to $260$ minutes. As shown in \cite{taspinar2016source, iuliani2017hybrid}, the first frame of the videos are typically not geometrically transformed. But as \cite{mandelli2019facing} pointed out, they may not always be available or some cameras may transform them as well, hence, we ignored those frames.

For this experiment, we extracted fingerprints from the frames of $20, 40, \dots 240$ seconds using conventional method as well as SDA-based method for SDA-depth of $30, 50,$ and $200$ as these are reasonable choices from the previous experiments.
We correlated each fingerprint with other fingerprints of different videos from the same camera that are created using the same number of frames. For example, SDA-30 fingerprints of $20$ second videos are correlated with the same type fingerprints from the same camera. 

Figure~\ref{figure:exp:stab_res} shows the TPR for three cameras (i.e., Huawei Honor, Samsung S8, and iPhone 6plus) and the total average of all the five cameras. 

% The results show that as the videos get longer, the TPR increases which supports the idea proposed in [the recent study/cite].   



\begin{figure} [!ht]
\centering
{\includegraphics[trim={1.2cm 8cm 1.4cm 8.3cm}, clip, keepaspectratio=true,width=\linewidth]{images/total_stab3.pdf}}
% {\includegraphics[trim={2.75cm 9.3cm 2.75cm 9.3cm}, clip, keepaspectratio=true,width=\linewidth]{images/stab_res.pdf}}
\caption{TPR for stabilized videos for varying SDA-depths}
\label{figure:exp:stab_res}
\end{figure}

The results show that as videos get longer, fingerprints obtained using conventional or SDA-based approach get more reliable. Moreover, the effect of increased SDA-depth is more significant for this case in comparison to non-stabilized videos. %This is because SDA-based approach performs poorly for iPhone cameras whereas for others, the performance is not almost as good as conventional approach. Figure X shows TPR of 

While for some cameras conventional and SDA-based approaches perform similarly (Huawei and Samsung cameras), for others (i.e., iPhone cameras) there is a significant difference between the two. For example, for Samsung S8 $SDA-200$ fingerprint from $120$ seconds video, perform similarly as $180$ seconds conventional fingerprint. Therefore, for this particular case, $SDA-200$ can speedup $66$ times \big(i.e. $\frac{180}{120}\times \frac{1407}{32}$\big)(see Table~\ref{tbl:sda_depth} for times). On the other hand for iPhone 6 plus, $60$ seconds video with conventional and $160$ seconds $SDA-50$ have similar TPR. Therefore, $11x$ \big(i.e., $\frac{60}{160}\times \frac{1407}{48}$\big) speedup can be achieved in this case. Overall, a speedup between these numbers (i.e. $11$ and $60$) can be achieved without any loss in TPR if a long video is available.


Overall, this subsection shows that the proposed SDA-based fingerprint extraction outperforms  the commonly used I-frame-only technique in all the cases for videos. These include for mixed media, stabilized videos, and social media. On the other hand, the SDA-based method achieves comparable results as all-frames-used fingerprint extraction with up to 50 times speedup. We also show the impact of SDA-depth on the performance that can be achieved in various cases. Finally, we show that SDA-based method order of frames doesn't have an impact on performance, yet shuffling the frames cause either a significant slow down or high I/O cost. Therefore, ordered access to videos is preferable to random access.



\subsection{Seam carved video} --> this can be itself a short paper?




% \subsection{Train and test on short videos}
% {\color{red} Another challenging source identification cases that researchers often encounters is when at least one of the fingerprints is a short video. In other words, either query or known video is a less than couple of seconds. In such a case fingerprints extracted from such videos are not often not reliable due to low number of highly compressed video frames. In DARPA Camera Identification Challenge~\cite{darpa2018medifor}, $4$ of $6$ challenges involved in videos that are quite short. 

% In this subsection, we evaluate how SDA-based technique will perform in such a highly challenging case. To evaluate this, we used SOCRatES dataset~\cite{galdisocrates} which contains a total of $1046$ videos from $96$ cameras. These videos are typically one to five seconds. We created $3$ fingerprints from each video in the dataset: using only I-frames, a single SDA-frame where the SDA-frame is the average of all available frames of the camera (we call this SDA-n where n is the total number of frames), and all-frames. 
% For this experiment, we correlated each fingerprint with the rest of the fingerprints of the same type from the same camera (i.e., fingerprints from I-frames correlated only with each other etc.). If none of the video fingerprints match (i.e., PCE $> 60$) for a camera, we considered that the videos are all stabilized and skipped the camera. Otherwise, we obtained their PCE scores for all those correlations. 

% In the dataset, the average number of frames per video is A, and average I-frames is B. Hence for I-frame only technique B and for all-frames A denoising operation is performed. On the other hand, only one denoising operation is done for SDA-based technique which makes it faster than I-frame only technique. (i.e., average times is a,b,c for I-, SDA- and all-frame based techniques respectively.)

% Table X shows the average PCE and the TPR for this experiment. As the table shows, fingerprint from I-frames performs very poorly that the accuracy is very low. On the other hand 

% \begin{table}[!ht]
% \centering
% \begin{tabular}{|c|c|c|c|}
% \hline
%               & I-frames & SDA-n & all-frames \\ \hline
% \#frames      & & 1 &               \\ \hline
% time(sec)     & & &                 \\ \hline
% PCE & 2792    & 7911  &  13895      \\ \hline
% TPR & 26.34   & 50.77 &  57.30      \\ \hline

% \end{tabular}
% \end{table}


% Notice that, in this experiment, some of the videos may still be stabilized, hence, drop the TPR for each technique. However, since our goal is to determine relative performance of these techniques, the impact of stabilized videos is irrelevant with the experiment.

% }


\subsection{stability check}
Another important issue that 

==> sections/old/5c_exp_image.tex <==

\section{Analysis on image fingerprints}
\label{sec:exp:img}

To verify the theoretical analysis and understand the properties of the sda-based fingerprint extraction method, we have done some experimental analysis on images. The experiments help clarify three main issues related to images that potentially have impact on the performance: (i) the effect of texture, (ii) the depth of an sda-frame (i.e., the number of images an sda-frame)  (iii) the effect of compression. Moreover, we investigated (iv) the equivalence of conventional fingerprint extraction and proposed approach. In these experiments, we used VISION dataset \cite{shullani2017vision} as it is a comprehensive set containing flatfield and textured images as well as the compressed social media versions of those (i.e., compressed in WhatsApp or Facebook). 



\subsection{Social media images}
% \textbf{THIS IS MORE LIKE SOCIAL MEDIA}
Another factor that might impact performance of sda-based method is the compression of the images used for reference fingerprint. To understand this batter, we used the images of VISION dataset. Fortunately, each image in the vision dataset has three compressed versions: WhatsApp(WA), Facebook high-resolution (FBH), and Facebook low-resolution (FBL). While the average size of original natural images are 2.88 MB, the average size of WA, FBH, and FBL are 327 KB, 337 KB, and 122 KB, respectively. Note that the resolution of FBH is typically higher than WA which indicates that the compression of FBH is higher than WA. So WA images has the lowest compression and FBL has the highest.

In this experiment, for each type of data (i.e., FBH, FBL, and WA), we used the $50$ textured images as training set and compared the fingerprints with rest of the images of a camera. We have done the same experiment as (sda-depth) and obtained\textbf{ ...}

\begin{table}[!ht]
\centering
\begin{tabular}{|c|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{WA} & \multicolumn{2}{c|}{FBH} & \multicolumn{2}{c|}{FBL} \\\hline 
       & PCE     & TPR     & PCE       & TPR    & PCE      & TPR  \\ \hline
sda-1  & 945.1   & 0.92    & 902.6     & 0.88   & 190.9    & 0.49 \\ \hline
sda-2  & 624.6   & 0.89    & 622.5     & 0.81   & 123.3    & 0.38 \\ \hline
sda-5  & 383.4   & 0.80    & 398.6     & 0.69   & 70.0     & 0.27 \\ \hline
sda-10 & 297.6   & 0.74    & 312.1     & 0.61   & 51.3     & 0.23 \\ \hline
sda-25 & 241.9   & 0.69    & 246.3     & 0.53   & 41.2     & 0.20 \\ \hline
sda-50 & 215.8   & 0.66    & 212.4     & 0.49   & 37.5     & 0.18 \\ \hline
\end{tabular}
\caption{compression}
\label{table:exp:img:compress}
\end{table}

As seen in the Table~\ref{table:exp:img:compress}, the higher the compression, the lower the PCE and TPR, which is already known in the field. However, based on these results, we can say that compression does not seem to affect  sda-depths. For example, the ratio of the average PCE for sda-10 and sda-25 is $\frac{297.6}{241.9}=1.23$ for WA, $\frac{312.1}{246.3}=1.27$ for FBH, and $\frac{51.3}{41.2}=1.25$ for FBL which shows compression does not have impact on sda-depth. 

An interesting behaviour to note that even though the average PCE for FBH is greater than WA, the TPR is lower. Based on the results, when the average PCE is low (i.e. below a few hundred), WA images tend to have higher average PCE, whereas when it is high, FBH tends to give higher average PCE than WA. Thus, total averages becomes approximately equal but the TPR of WA is significantly higher. However, we couldn't find the reason for this characteristic.

Note that, because the resolutions of images are lower in this experiment (due to social media resizing), we didn't employ block-wise correlation; instead we did the correlations on full resolutions.
% We also compressed the textured images by changing the quality factor of each image. Assuming the quality factor of original images is $100$, we compressed the images with quality factor $80, 60, 40,$ and $20$. This way, we created $5$ samples of each.



==> sections/old/6_experiment.tex <==
\section{Experiment}
\label{sec:experiment}

% \textbf{EXPERIMENTS WE NEED TO DO: }
% \textbf{fast verification via sda-frame (think about 1-2 second videos)}
% \begin{enumerate}
11

%     \item videos
%     \begin{enumerate}
%         \item effect of num images
%         \item order of frames/shuffling
%         \item stability check
%     \end{enumerate}
%     \item images
%     \begin{enumerate}
%         \item fp equivalence
%         \item texture
%         \item effect of image quality (compression)
%     \end{enumerate}
% \end{enumerate}

This section experimentally evaluates the effectiveness of the proposed fingerprint extraction technique and gives an insight for various aspect of it.

The implementation for this paper is done using Matlab 2016a on Windows 7 PC with 32 GB memory and Intel Xeon(R) E5-2687W v2 @3.40GHz CPU. The wavelet denoising algorithm \cite{mihcak:filter} has been used to obtain fingerprint and PRNU noise. PCE and NCC  methods are used for comparison. The preset threshold of 60 \cite{jessica:crop} is considered as threshold that when the PCE results two fingerprints are less than this threshold, they are considered to null hypothesis ($H_0$), otherwise, alternate hypothesis ($H_1$). The \textit{NYUAD Mixed Media Dataset (NYUAD MMD)}cite{media paper} was used for the experiments which consists of visual media from $78$ smartphone cameras ($19$ brands, $58$ different models). There are a total of images, and $301$ videos of various resolutions in this dataset. Along with NYUAD MMD, VISION dataset \cite{shullani2017vision} was used which consists of $35$ cameras having $16,100$ images and $315$ pristine videos. To create a camera fingerprint, images having same resolution taken by a camera are clustered together (using \cite{bloy2008blind}) before creating a camera fingerprint from images. 

\subsection{Videos}
Section~\ref{section:sda4videos} explains the main approaches to create a camera fingerprint from videos: from i-frames, all-frames and the proposed sda-frames. Table~\ref{tbl:vF_extraction} compares the average time it takes to extract fingerprint from a FullHD @30FPS video using the first $40$ i-frames, $40$ sda-frames, all-frames in the first $40$ seconds (approx. $40\times30$ frames). The results show that extracting fingerprint from all $1200$ frames takes about $28$ minutes. Thus, obtaining fingerprints of all $301$ videos requires almost $6$ days for a single threaded Matlab code when all-frames ($1200$ frames) are used for extraction. On the other hand, the same takes $5$ and $10$ hours when i-frames and sda-frames ($40$ frames each) are used, respectively. Therefore, sda-frames is half speed as i-frames and $13.5$ times faster than all-frames in our experimental setting. 

\begin{table}[!h]
\centering
\caption{Time for video fingerprint extraction in second}
\vspace{-0.3em}
\begin{tabular}{|c|c|c|c|c|}
\hline

type        & I/O time  & averaging  & noise extraction  & total      \\ \hline
i-frame     & 3         & 0          & 56                & 59         \\ \hline
sda-frame & 15        & 54         & 56                & 125        \\ \hline
all-frame   & 15        & 0          & 1680              & 1695       \\ \hline
\end{tabular}
\label{tbl:vF_extraction}
\vspace{-1em}
\end{table}

To evaluate the effectiveness of the proposed approach, each fingerprint from a video (from i-frames, sda-frames, and all-frames) is correlated with the noise of images captured by the same camera. The resizing factors of images and videos are obtained from \cite{media paper}. 

\begin{table}[!h]
\centering
\caption{Performance comparison of image source identification for video fingerprints}
\vspace{-0.3em}

\begin{tabular}{ |c|c|c|c|c| } 
    \hline
    type           & $\#match$ & $\#comparison$  & $ performance $  \\  \hline
    i-frame        & 15187     & 24077           & 63.07\%          \\  \hline
    sda-frame    & 18769     & 24077           & 77.96\%          \\  \hline
    all-frame      & 19948     & 24077           & 82.85\%          \\  \hline
\end{tabular}
\label{table:vF2iN}
\vspace{-0.3em}
\end{table}

Table~\ref{table:vF2iN} compares the True Positive Rates (TPR) when fingerprint is obtained from the three ways. When fingerprint is obtained by i-frames, only $63.07\%$ of the images can be correctly attributed to their sources and all-frames can achieve the highest TPR, $82.85\%$. As seen, sda-frame achieves $4.89\%$ less than all-frames and $14.89$ more than i-frames. 

The results show that the proposed approach can be a middle solution for fingerprint extraction from videos. This technique compromises from performance to achieve a significant speed up. Furthermore, as mentioned in Section~\ref{sec:approach:sda_picture}, when the video is long enough (i.e. few minutes), more frames can be used in sda-frame which is expected to improve the performance.


\subsubsection{\textbf{Number of Frames in Sda-frame}}
To understand the schema, it is crucial to examine how the performance changes as $p$ (number of frames to be averaged for an sda-frame) changes. Given a video of $n$ frames (in our case approx. $1200$ frames), we divided $n$ into groups of $p = 1, 5, 10, 30, 50, 200, 1200$. Therefore, $q = 1200, 240, 120, 40, 24, 6, 1$ sda-frames were created, respectively. When $p = 1$, the technique becomes same as using all frames whereas when $p = 1200$, all frames are used to create a single sda-frame. For this experiment, we used NYUAD-mmd that for each video, a fingerprint from each sda-level is created (a total of $7$ videos). 
Each of these fingerprints are compared with the noise all images from the same camera for acquiring $H_1$ hypothesis and image noise from random cameras for $H_0$ hypothesis. Figure~\ref{figure:experiment:num_image_sda} shows the ROC curves for each sda-level (i.e. $p$). The results show that the sda-level achieving the highest performance are $p = 1$ and then $30$ whereas the lowest performing one is when $1200$ and $200$. Because $p = 1$ is same as conventional approach, this is an expected result. Similarly, when $p = 1200, 200$, the results were expected to be lowest. (\textbf{why $p = 30$ works second best? find out. I think it is related to i-frames. like each sda-frame has one i-frame on average})

\begin{figure} [!h]
\centering
{\includegraphics[keepaspectratio=true,width=82mm]{images/results/num_image_sda/num_image.jpg}}
\caption{The ROC curves for varying sda-levels}
\label{figure:experiment:num_image_sda}
\end{figure}

Table~\ref{table:auc:num_image} shows the Area Under Curve (AUC) for Figure~\ref{figure:experiment:num_image_sda}. 


\begin{table}[!h]
\centering
\caption{AUC for proposed and conventional methods}
\label{table:auc:num_image}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline

$p$      & 1     & 5      & 10    & 30     & 50    & 200   & 1200  \\ \hline
auc      & 0.946 & 0.9195 & 0.912 & 0.929  & 0.91 & 0.913 & 0.879 \\ \hline
\end{tabular}
\end{table}



\subsubsection{\textbf{Order of Frames}}
A video is a set of sequential frames that each frame .... (tell about order). This section analyzes if the order of video has any impact on the proposed approach. In other words, our goal is to evaluate whether the performance or average PCE will change if the video frames are shuffled before sda-frames are created. For this purpose, ...

\begin{table}[!h]
\centering
\caption{TPR change for  }
\label{table:sda_shuffle:TPR}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
             & $1$ & $5$     & $10$    &   $30$      & $50$    & $200$  & $1200$ \\ \hline
% ordered      & 0.7795 &  0.7444 &  0.7275 &   0.7202    &  0.7206 & 0.7030 & 0.6324 \\ \hline
% shuffled     &   &  0.7459 & 0.7272  &   0.7208    &  0.7211 & 0.7048 & 0.6316 \\ \hline

% corr-ord   & 82.85  &  74.44 &  72.75 &  72.02 &  72.06 & 70.30 & 63.24 \\ \hline
ordered    & 82.85  &  79.47 &  78.55 &  77.95 &  77.06 & 75.30 & 68.24 \\ \hline
shuffled   & 82.85  &  79.62 &  78.72 &  78.00 &  77.11 & 75.48 & 68.16 \\ \hline
\end{tabular}
\end{table}

%In this section, we analyzed the effect of number of frames that are used to create a sda-frame. In other words, given $n$ frames, $p$ sda-frames and $q$ number of frames forming an sda-frame (i.e. $n=p \times q$), we investigated time and performance of the approach for different values of $p$ and $q$. 


\subsection{Images}

\begin{table}[!h]
\centering
\caption{Time to Extract Fingerprints with proposed and conventional methods}
\label{table:time:sda-conv}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
     & $5$     & $10$    & $20$    & $30$       & $50$   \\ \hline
sda  & 4.9655  & 5.9898  & 8.2220  & 10.3463  & 14.6933  \\ \hline
conv & 21.5697 & 40.8120 & 79.9615 & 118.7870 & 196.5942 \\ \hline
\end{tabular}
\end{table}


\subsubsection{\textbf{Effect of texture}}
As Section~\ref{sec:math} shows image texture(content) is one of the most significant noise source that differs conventional fingerprint extraction method from usage of sda-frame. The conventional method can remove/decrease content noise whereas usage of sda-frame fails to achieve it. Therefore, the difference between conventional and proposed approaches is expected to be minimized when training set consists of flat-field images. In other words, the experimental results (such as average PCE, TPR and so on.) should have a little or no difference for conventional and proposed fingerprint extraction methods when the training set is flat-field images whereas high difference between the two approaches when the training images are textured.

To verify the mathematical analysis, we created two sets of $50$ images for fingerprint extraction (training sets): textured and flat-field images. Two types of fingerprint were extracted from each group: via conventional way and sda-frame. From each of these categories, we extracted fingerprints using $5$, $10$, $20$, $30$, and $50$ images. Therefore, a total of $20$ fingerprints we obtained for each camera ($2$ types of images, $2$: fingerprint extraction techniques, $5$: for different number of images used for extraction). Each of these fingerprints is correlated with the noise of the test set which consists of both textured and flat-field images. We, then, correlated the fingerprints with the noise of the test set which consists of both textured and flat-field images. In this experiment, VISION dataset \cite{shullani2017vision} has been used as it is a comprehensive data containing flat-field and textured images. 

\begin{table}[]
\centering
\caption{Average PCE change by image type, extraction type and number of images used for fingerprint}
\label{table:texture:avg_PCE}
\begin{tabular}{|c|c|c|c|c|c|c|}
 \hline
                           &      & $5$   & $10$  & $20$  & $30$  & $50$  \\ \hline
\multirow{2}{*}{flatfield} & sda  & 11307 & 17307 & 24172 & 28116 & 32555 \\ 
                           & conv & 10402 & 17526 & 27316 & 33908 & 42556 \\ \hline
\multirow{2}{*}{textured}  & sda  & 2772  & 3786  & 5666  & 6869  & 9228  \\ 
                           & conv & 4006  & 6656  & 11494 & 14626 & 21333 \\ \hline
\end{tabular}\end{table}


Table~\ref{table:texture:avg_PCE} shows the average PCE of the comparison of fingerprints with the PRNU noise of the same camera images ($H_1$ hypothesis). For example, when fingerprint is extracted from $20$ flatfield images using sda-frame for fingerprint extraction, the average PCE is $24,172$, whereas using conventional approach, it is equal to $27,316$.  



\begin{figure} [!h]
\centering
\subfloat [Average PCE ratio for conv/sda] {\includegraphics[width=82mm]{images/results/texture/texture_blockwise_pce.png}}
\caption{The effect of texture in terms of PCE ratio}
\label{figure:experiment:texture}
\end{figure}

To elaborate the difference of the two approaches for textured and flatfield images, we show the normalized the results (i.e. $conventional/proposed$). Figure~\ref{figure:experiment:texture} shows the ratio of the average PCE of the $H_1$ hypothesis. As seen, when fingerprint is extracted from flatfield images, both approaches have performs similar. However, this difference becomes more significant when texture images are textured. For example, conventional approach results in $13\%$ higher PCE compared to proposed method when $20$ flatfield images are used whereas it achieves $103\%$ higher PCE when textured images are used.  

Figure~\ref{figure:experiment:TPR_texture} shows the TPR of each fingerprint type as the number of images used to extract fingerprint changes for both flat-field and textured images. The results show the fingerprint extracted using conventional approach achieves slightly higher TPR than the other fingerprints. On the other hand, fingerprints obtained using the proposed approach achieves almost the same performance as the conventional approach; even higher in some cases.


\begin{figure} [!h]
\centering
\subfloat [TPR of sda and conventional approaches: textured vs flatfield] {\includegraphics[keepaspectratio=true,width=82mm]{images/results/texture/texture_blockwise_tpr.png}}
\caption{The effect of texture in terms of TPR}
\label{figure:experiment:TPR_texture}
\end{figure}



The results indicate that, when the images are flat-field, the difference between the two fingerprint extraction is not very significant whereas the difference of conventional method and proposed method becomes higher for textured images. These results aligns with the mathematical analysis. 


\subsubsection{\textbf{Fingerprint Equivalence}}
In this section, our goal is to compare conventional and proposed fingerprint extraction approaches in terms of number images that achieves the same TPR and average PCE. For example, if a fingerprint is extracted from $m$ still images using conventional approach, how many images should be used to obtain an sda-frame to achieve the same performance? 
To evaluate this, we used VISION dataset \cite{shullani2017vision} that $19$ camera fingerprint is obtained from $2$ to $20$ images using conventional approach and $2$ to $50$ images using sda-frames. The training set consists only of textured images as it is a worse case compared to flat-field images(\textbf{explain better}). Furthermore, we divided each fingerprint to $500\times 500$ blocks and compared them with the corresponding blocks of the test PRNU noise. A total of $244,127$ comparison has been done. 

Figure~\ref{figure:exp:fp_equi:perf} shows the number of images required for sda-frame to achieve at least the same (i) TPR (ii) average PCE as the conventional fingerprint extraction. On the other hand, Figure~\ref{figure:exp:fp_equi:perf} shows the speed up achieved by sda-frame approach compared to the conventional way. 

For example, if a fingerprint obtained by sda-frame of $21$ images achieves the same TPR as a fingerprint by conventional approach using $10$ images. This fingerprint can be obtained $3.75$ times faster compared to conventional approach.

\begin{figure} [!h]
\centering
{\includegraphics[keepaspectratio=true, width=88mm]{images/results/fp_equiv/fp_equi_perf_plot.jpg}}
\caption{Fingerprint Equivalence}
\label{figure:exp:fp_equi:perf}
\end{figure}

\begin{figure} [!h]
\centering
{\includegraphics[keepaspectratio=true, width=88mm]{images/results/fp_equiv/fp_equi_time_plot.jpg}}
\caption{Fingerprint Equivalence}
\label{figure:exp:fp_equi:time}
\end{figure}

\subsection{Stabilized Videos}
A recent research [cite] has shown that when a stabilized video is at least 4-minute long, it can be attributed to its source camera when all its frames (i.e., $7200$ frames) are denoised. As mentioned in \ref{sec:background}, extracting fingerprint from so many frames can take a very long time, hence, may not be practical in some settings. A potential alternative for this problem is the usage of SDA-frames which may lead to a significant speed up. To evaluate this, we captured $4+$ minute stabilized videos from $10$ cameras, a total of $100$ videos. As shown in \cite{taspinar2016source, iuliani2017hybrid}, the first frame of the videos are typically not geometrically transformed. But as \cite{mandelli2018facing} pointed out, they may not always be available or some cameras may transform them as well, hence, we ignored those frames.

For this experiment, we extracted fingerprint from $1000, 2000,\dots 7000$ frames using conventional method. Then, we correlated each fingerprint with other fingerprints from the same camera that are created using the same number of frames to get $H_1$ hypothesis. Similarly, we compared each fingerprint with other fingerprints from random cameras to obtain $H_0$ hypothesis.
For the proposed method we used $7000$ frames of each video and we created sda-groups of $5, 10, 20, 30, 50, 500$. This way we obtained $1400, 700, 350, 234, 140, 14$ sda-frames, respectively. Then, we obtained $6$ fingerprints using these sda-frames and correlated each fingerprint with other fingerprints of same category ($H_1$ and $H_0$ are obtained in similar manner as above). 
Table XXX shows the average PCE of 



==> sections/old/6_experiment_backup.tex <==
\section{Experiment}
\label{sec:experiment}

% \textbf{EXPERIMENTS WE NEED TO DO: }
% \textbf{fast verification via sda-picture (think about 1-2 second videos)}
% \begin{enumerate}
%     \item videos
%     \begin{enumerate}
%         \item effect of num images
%         \item order of frames/shuffling
%         \item stability check
%     \end{enumerate}
%     \item images
%     \begin{enumerate}
%         \item fp equivalence
%         \item texture
%         \item effect of image quality (compression)
%     \end{enumerate}
% \end{enumerate}

This section experimentally evaluates the effectiveness of the proposed fingerprint extraction technique and gives an insight for various aspect of it. 

The implementation for this paper is done using Matlab 2016a on Windows 7 PC with 32 GB memory and Intel Xeon(R) E5-2687W v2 @3.40GHz CPU. The wavelet denoising algorithm \cite{mihcak:filter} has been used to obtain fingerprint and PRNU noise. PCE and NCC  methods are used for comparison. The preset threshold of 60 \cite{jessica:crop} is considered as threshold that when the PCE results two fingerprints are less than this threshold, they are considered to null hypothesis ($H_0$), otherwise, alternate hypothesis ($H_1$). The \textit{NYUAD Mixed Media Dataset (NYUAD MMD)}cite{media paper} was used for the experiments which consists of visual media from $78$ smartphone cameras ($19$ brands, $58$ different models). There are a total of images, and $301$ videos of various resolutions in this dataset. Along with NYUAD MMD, VISION dataset \cite{shullani2017vision} was used which consists of $35$ cameras having $16,100$ images and $315$ pristine videos. To create a camera fingerprint, images having same resolution taken by a camera are clustered together (using \cite{bloy2008blind}) before creating a camera fingerprint from images. 

\subsection{Videos}
Section~\ref{section:sda4videos} explains the main approaches to create a camera fingerprint from videos: from i-frames, all-frames and the proposed sda-pictures. Table~\ref{tbl:vF_extraction} compares the average time it takes to extract fingerprint from a FullHD @30FPS video using the first $40$ i-frames, $40$ sda-pictures, all-frames in the first $40$ seconds (approx. $40\times30$ frames). The results show that extracting fingerprint from all $1200$ frames takes about $28$ minutes. Thus, obtaining fingerprints of all $301$ videos requires almost $6$ days for a single threaded Matlab code when all-frames ($1200$ frames) are used for extraction. On the other hand, the same takes $5$ and $10$ hours when i-frames and sda-pictures ($40$ frames each) are used, respectively. Therefore, sda-pictures is half speed as i-frames and $13.5$ times faster than all-frames in our experimental setting. 

\begin{table}[!h]
\centering
\caption{Time for video fingerprint extraction in second}
\vspace{-0.3em}
\begin{tabular}{|c|c|c|c|c|}
\hline

type        & I/O time  & averaging  & noise extraction  & total      \\ \hline
i-frame     & 3         & 0          & 56                & 59         \\ \hline
sda-picture & 15        & 54         & 56                & 125        \\ \hline
all-frame   & 15        & 0          & 1680              & 1695       \\ \hline
\end{tabular}
\label{tbl:vF_extraction}
\vspace{-1em}
\end{table}

To evaluate the effectiveness of the proposed approach, each fingerprint from a video (from i-frames, sda-pictures, and all-frames) is correlated with the noise of images captured by the same camera. The resizing factors of images and videos are obtained from \cite{media paper}. 

\begin{table}[!h]
\centering
\caption{Performance comparison of image source identification for video fingerprints}
\vspace{-0.3em}

\begin{tabular}{ |c|c|c|c|c| } 
    \hline
    type           & $\#match$ & $\#comparison$  & $ performance $  \\  \hline
    i-frame        & 15187     & 24077           & 63.07\%          \\  \hline
    sda-picture    & 18769     & 24077           & 77.96\%          \\  \hline
    all-frame      & 19948     & 24077           & 82.85\%          \\  \hline
\end{tabular}
\label{table:vF2iN}
\vspace{-0.3em}
\end{table}

Table~\ref{table:vF2iN} compares the True Positive Rates (TPR) when fingerprint is obtained from the three ways. When fingerprint is obtained by i-frames, only $63.07\%$ of the images can be correctly attributed to their sources and all-frames can achieve the highest TPR, $82.85\%$. As seen, sda-picture achieves $4.89\%$ less than all-frames and $14.89$ more than i-frames. 

The results show that the proposed approach can be a middle solution for fingerprint extraction from videos. This technique compromises from performance to achieve a significant speed up. Furthermore, as mentioned in Section~\ref{sec:approach:sda_picture}, when the video is long enough (i.e. few minutes), more frames can be used in sda-picture which is expected to improve the performance.


\subsubsection{\textbf{Number of Frames in Sda-picture}}
To understand the schema, it is crucial to examine how the performance changes as $p$ (number of frames to be averaged for an sda-picture) changes. Given a video of $n$ frames (in our case approx. $1200$ frames), we divided $n$ into groups of $p = 1, 5, 10, 30, 50, 200, 1200$. Therefore, $q = 1200, 240, 120, 40, 24, 6, 1$ sda-pictures were created, respectively. When $p = 1$, the technique becomes same as using all frames whereas when $p = 1200$, all frames are used to create a single sda-picture. For this experiment, we used NYUAD-mmd that for each video, a fingerprint from each sda-level is created (a total of $7$ videos). 
Each of these fingerprints are compared with the noise all images from the same camera for acquiring $H_1$ hypothesis and image noise from random cameras for $H_0$ hypothesis. Figure~\ref{figure:experiment:num_image_sda} shows the ROC curves for each sda-level (i.e. $p$). The results show that the sda-level achieving the highest performance are $p = 1$ and then $30$ whereas the lowest performing one is when $1200$ and $200$. Because $p = 1$ is same as conventional approach, this is an expected result. Similarly, when $p = 1200, 200$, the results were expected to be lowest. (\textbf{why $p = 30$ works second best? find out. I think it is related to i-frames. like each sda-frame has one i-frame on average})

\begin{figure} [!h]
\centering
{\includegraphics[keepaspectratio=true,width=82mm]{images/results/num_image_sda/num_image.jpg}}
\caption{The ROC curves for varying sda-levels}
\label{figure:experiment:num_image_sda}
\end{figure}

Table~\ref{table:auc:num_image} shows the Area Under Curve (AUC) for Figure~\ref{figure:experiment:num_image_sda}. 


\begin{table}[!h]
\centering
\caption{AUC for proposed and conventional methods}
\label{table:auc:num_image}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
$p$      & 1     & 5      & 10    & 30     & 50    & 200   & 1200  \\ \hline
auc      & 0.946 & 0.9195 & 0.912 & 0.929  & 0.91 & 0.913 & 0.879 \\ \hline
\end{tabular}
\end{table}


\begin{table}[!h]
\centering
\caption{Time to Extract Fingerprints with proposed and conventional methods}
\label{table:time:sda-conv}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
     & $5$     & $10$    & $20$    & $30$       & $50$   \\ \hline
sda  & 4.9655  & 5.9898  & 8.2220  & 10.3463  & 14.6933  \\ \hline
conv & 21.5697 & 40.8120 & 79.9615 & 118.7870 & 196.5942 \\ \hline
\end{tabular}
\end{table}

\subsubsection{\textbf{Order of Frames}}
A video is a set of sequential frames that each frame .... (tell about order). This section analyzes if the order of video has any impact on the proposed approach. In other words, our goal is to evaluate whether the performance or average PCE will change if the video frames are shuffled before sda-pictures are created. For this purpose, ...

\begin{table}[!h]
\centering
\caption{TPR change for  }
\label{table:sda_shuffle:TPR}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
             & $5$     & $10$    &   $30$      & $50$    & $200$  & $1200$ \\ \hline
ordered     &    0.7444 &  0.7275 &   77.95    &  0.7206 & 0.7030 & 0.6324 \\ \hline
shuffled      &  0.7459 & 0.7272  &   78.00    &  0.7211 & 0.7048 & 0.6316 \\ \hline
\end{tabular}
\end{table}
\textbf{results for ordered-5 is wrong, re-create the fingerprints and re-run the tests for it}

%In this section, we analyzed the effect of number of frames that are used to create a sda-picture. In other words, given $n$ frames, $p$ sda-pictures and $q$ number of frames forming an sda-picture (i.e. $n=p \times q$), we investigated time and performance of the approach for different values of $p$ and $q$. 


\subsection{Images}

\subsubsection{\textbf{Effect of texture}}
As Section~\ref{sec:math} shows image texture(content) is one of the most significant noise source that differs conventional fingerprint extraction method from usage of sda-picture. The conventional method can remove/decrease content noise whereas usage of sda-picture fails to achieve it. Therefore, the difference between conventional and proposed approaches is expected to be minimized when training set consists of flat-field images. In other words, the experimental results (such as average PCE, TPR and so on.) should have a little or no difference for conventional and proposed fingerprint extraction methods when the training set is flat-field images whereas high difference between the two approaches when the training images are textured.

To verify the mathematical analysis, we created two sets of $50$ images for fingerprint extraction (training sets): textured and flat-field images. Two types of fingerprint were extracted from each group: via conventional way and sda-picture. From each of these categories, we extracted fingerprints using $5$, $10$, $20$, $30$, and $50$ images. Therefore, a total of $20$ fingerprints we obtained for each camera ($2$ types of images, $2$: fingerprint extraction techniques, $5$: for different number of images used for extraction). Each of these fingerprints is correlated with the noise of the test set which consists of both textured and flat-field images. We, then, correlated the fingerprints with the noise of the test set which consists of both textured and flat-field images. In this experiment, VISION dataset \cite{shullani2017vision} has been used as it is a comprehensive data containing flat-field and textured images. 

\begin{table}[]
\centering
\caption{Average PCE change by image type, extraction type and number of images used for fingerprint}
\label{table:texture:avg_PCE}
\begin{tabular}{|c|c|c|c|c|c|c|}
 \hline
                           &      & $5$   & $10$  & $20$  & $30$  & $50$  \\ \hline
\multirow{2}{*}{flatfield} & sda  & 11307 & 17307 & 24172 & 28116 & 32555 \\ 
                           & conv & 10402 & 17526 & 27316 & 33908 & 42556 \\ \hline
\multirow{2}{*}{textured}  & sda  & 2772  & 3786  & 5666  & 6869  & 9228  \\ 
                           & conv & 4006  & 6656  & 11494 & 14626 & 21333 \\ \hline
\end{tabular}\end{table}


Table~\ref{table:texture:avg_PCE} shows the average PCE of the comparison of fingerprints with the PRNU noise of the same camera images ($H_1$ hypothesis). For example, when fingerprint is extracted from $20$ flatfield images using sda-picture for fingerprint extraction, the average PCE is $24,172$, whereas using conventional approach, it is equal to $27,316$.  



\begin{figure} [!h]
\centering
\subfloat [Average PCE ratio for conv/sda] {\includegraphics[width=82mm]{images/results/texture/texture_blockwise_pce.png}}
\caption{The effect of texture in terms of PCE ratio}
\label{figure:experiment:texture}
\end{figure}

To elaborate the difference of the two approaches for textured and flatfield images, we show the normalized the results (i.e. $conventional/proposed$). Figure~\ref{figure:experiment:texture} shows the ratio of the average PCE of the $H_1$ hypothesis. As seen, when fingerprint is extracted from flatfield images, both approaches have performs similar. However, this difference becomes more significant when texture images are textured. For example, conventional approach results in $13\%$ higher PCE compared to proposed method when $20$ flatfield images are used whereas it achieves $103\%$ higher PCE when textured images are used.  

Figure~\ref{figure:experiment:TPR_texture} shows the TPR of each fingerprint type as the number of images used to extract fingerprint changes for both flat-field and textured images. The results show the fingerprint extracted using conventional approach achieves slightly higher TPR than the other fingerprints. On the other hand, fingerprints obtained using the proposed approach achieves almost the same performance as the conventional approach; even higher in some cases.


\begin{figure} [!h]
\centering
\subfloat [TPR of sda and conventional approaches: textured vs flatfield] {\includegraphics[keepaspectratio=true,width=82mm]{images/results/texture/texture_blockwise_tpr.png}}
\caption{The effect of texture in terms of TPR}
\label{figure:experiment:TPR_texture}
\end{figure}



The results indicate that, when the images are flat-field, the difference between the two fingerprint extraction is not very significant whereas the difference of conventional method and proposed method becomes higher for textured images. These results aligns with the mathematical analysis. 


\subsubsection{\textbf{Fingerprint Equivalence}}
In this section, our goal is to compare conventional and proposed fingerprint extraction approaches in terms of number images that achieves the same TPR and average PCE. For example, if a fingerprint is extracted from $m$ still images using conventional approach, how many images should be used to obtain an sda-picture to achieve the same performance? 
To evaluate this, we used VISION dataset \cite{shullani2017vision} that $19$ camera fingerprint is obtained from $2$ to $20$ images using conventional approach and $2$ to $50$ images using sda-pictures. The training set consists only of textured images as it is a worse case compared to flat-field images(\textbf{explain better}). Furthermore, we divided each fingerprint to $500\times 500$ blocks and compared them with the corresponding blocks of the test PRNU noise. A total of $244,127$ comparison has been done. 

Figure~\ref{figure:exp:fp_equi:perf} shows the number of images required for sda-picture to achieve at least the same (i) TPR (ii) average PCE as the conventional fingerprint extraction. On the other hand, Figure~\ref{figure:exp:fp_equi:perf} shows the speed up achieved by sda-picture approach compared to the conventional way. 

For example, if a fingerprint obtained by sda-picture of $21$ images achieves the same TPR as a fingerprint by conventional approach using $10$ images. This fingerprint can be obtained $3.75$ times faster compared to conventional approach.

\begin{figure} [!h]
\centering
{\includegraphics[keepaspectratio=true, width=88mm]{images/results/fp_equiv/fp_equi_perf_plot.jpg}}
\caption{Fingerprint Equivalence}
\label{figure:exp:fp_equi:perf}
\end{figure}

\begin{figure} [!h]
\centering
{\includegraphics[keepaspectratio=true, width=88mm]{images/results/fp_equiv/fp_equi_time_plot.jpg}}
\caption{Fingerprint Equivalence}
\label{figure:exp:fp_equi:time}
\end{figure}

\subsection{Stabilized Videos}
A recent research [cite] has shown that when a stabilized video is at least 4-minute long, it can be attributed to its source camera when all its frames (i.e., $7200$ frames) are denoised. As mentioned in \ref{sec:background}, extracting fingerprint from so many frames can take a very long time, hence, may not be practical in some settings. A potential alternative for this problem is the usage of SDA-frames which may lead to a significant speed up. To evaluate this, we captured $4+$ minute stabilized videos from $10$ cameras, a total of $100$ videos. As shown in \cite{taspinar2016source, iuliani2017hybrid}, the first frame of the videos are typically not geometrically transformed. But as \cite{mandelli2018facing} pointed out, they may not always be available or some cameras may transform them as well, hence, we ignored those frames.

For this experiment, we extracted fingerprint from $1000, 2000,\dots 7000$ frames using conventional method. Then, we correlated each fingerprint with other fingerprints from the same camera that are created using the same number of frames to get $H_1$ hypothesis. Similarly, we compared each fingerprint with other fingerprints from random cameras to obtain $H_0$ hypothesis.
For the proposed method we used $7000$ frames of each video and we created sda-groups of $5, 10, 20, 30, 50, 500$. This way we obtained $1400, 700, 350, 234, 140, 14$ sda-pictures, respectively. Then, we obtained $6$ fingerprints using these sda-pictures and correlated each fingerprint with other fingerprints of same category ($H_1$ and $H_0$ are obtained in similar manner as above). 
Table XXX shows the average PCE of 



==> sections/old/6_experiment_new.tex <==
\section{Experiment}
\label{sec:experiment}

This section experimentally validates the theoretical analysis as well as evaluates the effectiveness of the proposed fingerprint extraction technique. Moreover, it gives an insight for various aspect of it. Specifically, experimental analysis have been conducted to enlighten how the proposed technique can be effective for non-stabilized or stabilized videos as well as images. NYUAD-MMD \cite{taspinar2019source} and VISION dataset \cite{shullani2017vision} were used for these experiments. The experimental analysis also investigates when the visual media is obtained from social media, namely, Facebook, YouTube, or WhatsApp.

The implementations for this paper are done using Matlab 2016a on Windows 7 PC with 32 GB memory and Intel Xeon(R) E5-2687W v2 @3.40GHz CPU. The wavelet denoising algorithm \cite{mihcak:filter} has been used to obtain fingerprint and PRNU noise. PCE and NCC  methods are used for comparison. The preset threshold of 60 \cite{jessica:crop} is considered as threshold that when the PCE results two fingerprints are less than this threshold, they are considered to null hypothesis ($H_0$), otherwise, alternate hypothesis ($H_1$).

% \textbf{Should we explain datasets here? We use nyuad-mmd and vision...}








==> sections/old/experiment_bkp.tex <==
\section{Experiment}
\label{sec:experiment}

This section experimentally evaluates the effectiveness of the proposed fingerprint extraction technique and gives an insight for various aspect of it.

The implementation for this paper is done using Matlab 2016a on Windows 7 PC with 32 GB memory and Intel Xeon(R) E5-2687W v2 @3.40GHz CPU. The wavelet denoising algorithm \cite{mihcak:filter} has been used to obtain fingerprint and PRNU noise. PCE and NCC  methods are used for comparison. The preset threshold of 60 \cite{jessica:crop} is considered as threshold that when the PCE results two fingerprints are less than this threshold, they are considered to null hypothesis ($H_0$), otherwise, alternate hypothesis ($H_1$). The \textit{NYUAD Mixed Media Dataset (NYUAD MMD)}cite{media paper} was used for the experiments which consists of visual media from $78$ smartphone cameras ($19$ brands, $58$ different models). There are a total of images, and $301$ videos of various resolutions in this dataset. Along with NYUAD MMD, VISION dataset \cite{shullani2017vision} was used which consists of $35$ cameras having $16,100$ images and $315$ pristine videos. To create a camera fingerprint, images having same resolution taken by a camera are clustered together (using \cite{bloy2008blind}) before creating a camera fingerprint from images. 


\subsection{Images}
\label{sec:exp:img}
To verify the theoretical analysis and understand the properties of the sda-based fingerprint extraction method, we have done some experimental analysis on images. The experiments help clarify three main issues related to images that potentially have impact on the performance: (i) the effect of texture, (ii) the depth of an sda-frame (i.e., the number of images an sda-frame)  (iii) the effect of compression. Moreover, we investigated (iv) the equivalence of conventional fingerprint extraction and proposed approach. In these experiments, we used VISION dataset \cite{shullani2017vision} as it is a comprehensive set containing flatfield and textured images as well as the compressed social media versions of those (i.e., compressed in WhatsApp or Facebook). 


\paragraph{(i) Effect of texture}
As Section~\ref{sec:math} shows image texture (content) is one of the most significant noise source that differs conventional method from sda-frame based fingerprint extraction. The conventional method can remove/decrease content noise whereas usage of sda-based method fails to achieve it as successfully. Therefore, when training set is flatfield images, the difference between conventional and sda-based method should be minimal (i.e., quality of fingerprints should be very similar).
In other words, the experimental results (such as average PCE, TPR and so on.) should have a little or no difference for both techniques when the training set is flat-field images whereas high difference between the two approaches when the training images are textured. 

To verify the theoretical analysis, we created two sets of $50$ images for fingerprint extraction (training sets): textured and flat-field images. 

Two types of fingerprint were extracted from each group: via conventional and sda-based method. From each of these categories, we extracted fingerprints using $5$, $10$, $20$, $30$, and $50$ images. Therefore, a total of $20$ fingerprints we obtained for each camera (i.e., $2$ types of images, (textured or flatfield), $2$ methods (conventional vs sda-based), and $5$ different number of images in a fingerprint). We, then, correlated each fingerprint with the noise of the test images which consists of both textured and flat-field images. Because correlation of full resolution fingerprint and query noise can be very high so that difference between the two approach may not be clear, we employed block-by-block comparison of the two where each block is $512\times512$.


\begin{figure} [!ht]
\centering
% trim={2.35cm 19.7cm 4.25cm 2.39cm},clip,
\subfloat [The effect of texture in terms of PCE] {\includegraphics[width=82mm] {images/texture_pce2}\label{fig:exp:texture:pce}}

\subfloat [The effect of texture in terms of TPR] {\includegraphics[width=82mm]{images/texture_tpr2}\label{fig:exp:texture:tpr}}
\caption{The effect of image content}
\end{figure}

Fig.~\ref{fig:exp:texture:pce} shows a comparison of average PCE for this experiment that shows how texture effects the PCE for fingerprints obtained from varying number of flatfield and textured images. On the other hand, Fig.~\ref{fig:exp:texture:tpr} shows the TPR for the same results. These figures support the theoretical analysis that when the images are the images are flatfield, both approaches result in similar PCE and TPR, whereas the difference of the two approaches is more clear when the training images are textured. The other implications of these figures are already well-known in the field (i.e., flatfield images are better than textured and as the number of images increase quality of fingerprint also increases.)

Since both techniques perform similarly for flatfield images, we can have a time comparison of the two approaches in that case. In other words, we know from this experiment that when we extract the fingerprint from $k$ flatfield images using conventional and sda-based technique, both will perform similarly. Therefore, it is important to provide time comparison for this case. 

\begin{table}[!ht]
\centering
\caption{{\color{red}Time to extract fingerprints with proposed and conventional methods (in sec)}}
\label{table:time:flat}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
     & $5$     & $10$    & $20$    & $30$       & $50$   \\ \hline
sda  & 4.9655  & 5.9898  & 8.2220  & 10.3463  & 14.6933  \\ \hline
conv & 21.5697 & 40.8120 & 79.9615 & 118.7870 & 196.5942 \\ \hline
\end{tabular}
\end{table}

Table~\ref{table:time:flat} shows the time it takes to extract fingerprint in either case. Notice that in both cases $k$ images are read from the disk but for sda-based technique, only one denoising where as for conventional way $k$ denoising operations are done. This shows as the training images increase, the speed up also increases. These results aligns with the mathematical analysis.


\paragraph{(ii) Sda-depth}
Another crucial issue is to understand the effect of the number of images in each sda-frame on performance and time. Suppose there are $k$ textured images from a camera and we want to create a fingerprint using the proposed technique. For this, we can create $g$ groups of $d$ images (where $k=d \times g$). So, we create $g$ sda-frames resulting in $g$ denoising operations rather than $k$. For example, in the above experiment $d=k$ (i.e., sda) or $d=1$ (i.e., conv.) was chosen. Since we already know that flatfield images doesn't have much impact on correlation, we only use textured images for training set. 

In this experiment, for each camera in VISION dataset, we create fingerprints using $50$ textured images. We set the sda-depth to $1, 2, 5, 10, 25$ and $50$. Therefore, we create $50, 25, 10, 5, 2,$ and $1$ sda-frames, respectively. The rest of the images were used as test images. We, then, correlated each fingerprint with the noise of those query images in the block-wise manner explained above. 

% Fig.X shows Y...
\begin{table}[!ht]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
    & sda-1    & sda-2    & sda-5    & sda-10  & sda-25   & sda-50   \\ \hline
PCE & 663.1 & 514.6 & 390.0 & 332.2  & 285.0  & 252.4 \\ \hline
TPR & 0.80  & 0.78  & 0.75  & 0.72   & 0.69   & 0.67   \\ \hline
\end{tabular}
\caption{SDA-depth vs TPR and PCE, change with figure, slight difference with fig 3/4?}
\label{table:sda_depth_perf}
\end{table}

Table~\ref{table:sda_depth_perf} shows that as the sda-depth increases, the average PCE decreases. This characteristic is consistent with the right columns in Fig.~\ref{fig:exp:texture:pce} and ~\ref{fig:exp:texture:tpr}. For textured images, the more images we combine to create an sda-frame, the lower PCE and TPR will be. As seen, when the depth is one (i.e., sda-1 which is same as conventional approach), the average PCE of $512\times512$ blocks is $663$ which gets lower when we combine more images. %Although the difference in of the two approaches is not very high in this setting, it might be higher when compression is higher.

\paragraph{(iii) Effect of compression}
Another factor that might impact performance of sda-based method is the compression of the images used for reference fingerprint. To understand this batter, we used the images of VISION dataset. Fortunately, each image in the vision dataset has three compressed versions: WhatsApp(WA), Facebook high-resolution (FBH), and Facebook low-resolution (FBH). While the average size of original natural images are 2.88 MB, the average size of WA, FBH, and FBL are 327 KB, 337 KB, and 122 KB, respectively. Note that the resolution of FBH is typically higher than WA which indicates that the compression of WA is lowest and FBL is the highest.

In this experiment, for each type of data (i.e., FBH, FBL, and WA), we used the $50$ textured images as training set and compared the fingerprints with rest of the images of a camera. We have done the same experiment as (sda-depth) and obtained ...

\begin{table}[!ht]
\centering
\begin{tabular}{|c|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{WA} & \multicolumn{2}{c|}{FBH} & \multicolumn{2}{c|}{FBL} \\\hline 
       & PCE     & TPR     & PCE       & TPR    & PCE      & TPR  \\ \hline
sda-1  & 945.1   & 0.92    & 902.6     & 0.88   & 190.9    & 0.49 \\ \hline
sda-2  & 624.6   & 0.89    & 622.5     & 0.81   & 123.3    & 0.38 \\ \hline
sda-5  & 383.4   & 0.80    & 398.6     & 0.69   & 70.0     & 0.27 \\ \hline
sda-10 & 297.6   & 0.74    & 312.1     & 0.61   & 51.3     & 0.23 \\ \hline
sda-25 & 241.9   & 0.69    & 246.3     & 0.53   & 41.2     & 0.20 \\ \hline
sda-50 & 215.8   & 0.66    & 212.4     & 0.49   & 37.5     & 0.18 \\ \hline
\end{tabular}
\caption{compression}
\label{table:exp:img:compress}
\end{table}

As seen in the Table~\ref{table:exp:img:compress}, the higher the compression, the lower the PCE and TPR which is already known in the field. However, based on these results, we can say that compression does not seem to affect  sda-depths. For example, the ratio of the average PCE for sda-10 and sda-25 is $\frac{297.6}{241.9}=1.23$ for WA, $\frac{312.1}{246.3}=1.27$ for FBH, and $\frac{51.3}{41.2}=1.25$ for FBL which shows compression does not have impact on sda-depth. 

An interesting behaviour to note that even though the average PCE for FBH is greater than WA, the TPR is lower. Based on the results, when the average PCE is low (i.e. below a few hundred), WA images tend to have higher average PCE, whereas when it is high, FBH tends to give higher average PCE than WA. Thus, total averages becomes approximately equal but the TPR of WA is significantly higher. However, we couldn't find the reason for this characteristic.

Note that, because the resolutions of images are lower in this experiment (due to social media resizing), we didn't employ block-wise correlation, instead we did the correlations on full resolutions.
% We also compressed the textured images by changing the quality factor of each image. Assuming the quality factor of original images is $100$, we compressed the images with quality factor $80, 60, 40,$ and $20$. This way, we created $5$ samples of each.

\paragraph{(iv) Fingerprint equivalence}
Finally, we evaluated the number of images required for both techniques that achieves similar PCE and TPR. For example, if $m$ still images are used in conventional approach, here we find the number of images that achieves similar performance using sda-based approach. 
To evaluate this, we used VISION dataset that $19$ camera fingerprint is obtained from $2$ to $20$ images using conventional approach and $49$ fingerprints from $2$ to $50$ images using sda-based approach. We then found the lowest number of images for sda-based method that achieves at least the same PCE and TPR as conventional approach. 

Furthermore, we again have employed block-wise comparison and a total of $244,127$ comparison has been made. 

\begin{figure} [!ht]

\subfloat[Equivalence of sda and conv]{\includegraphics[keepaspectratio=true, width=85mm]{images/im_fp_eq.pdf}\label{figure:exp:fp_equi:perf}}

\subfloat[Speed up achieved by sda]{\includegraphics[keepaspectratio=true, width=88mm]{images/im_fp_eq_speedup2.pdf}\label{figure:exp:fp_equi:time}}
\caption{Fingerprint Equivalence}
\label{figure:exp:fp_equi}
\end{figure}



% \begin{figure} [!ht]
% \centering
% % trim={2.35cm 19.7cm 4.25cm 2.39cm},clip,
% \subfloat [The effect of texture in terms of PCE] {\includegraphics[width=82mm] {images/texture_pce2}\label{fig:exp:texture:pce}}

% \subfloat [The effect of texture in terms of TPR] {\includegraphics[width=82mm]{images/texture_tpr2}\label{fig:exp:texture:tpr}}
% \caption{The effect of image content}
% \end{figure}


Figure~\ref{figure:exp:fp_equi:perf} shows the number of images required for sda-frame to achieve at least the same (i) TPR (ii) average PCE as the conventional fingerprint extraction. On the other hand, Figure~\ref{figure:exp:fp_equi:time} shows the speed up achieved by sda-frame approach compared to the conventional way. For example, to obtain same TPR of a fingerprint obtained using $10$ images using conventional way, $21$ images are needed using sda-based method. In this case $3.75x$ speedup can be achieved compared to conventional approach. On the other hand, to achieve approx. same PCE value $22$ images are needed which results in $3.6x$ speedup. 

Notice that all images used in fingerprints are textured as it is the worst case scenario for sda-based approach based on theoretical analysis (and experiment (i)). When, more flatfield images exists in the sda-frames, the improvement will be higher for sda-based approach (see Table~\ref{table:time:flat}). 

% ------------------------------------------
\subsection{Non-stabilized videos}
\label{sec:exp:nstab}
In the above subsection, we have verified the theoretical analysis as well as we investigated various issues that might potentially impact the sda-based approach. 
Here, we investigate a more practical case that the proposed technique can be helpful which is its usage for non-stabilized videos. As mentioned in the Section~\ref{sec:background}, a video fingerprint can be extracted from i-frames or all-frames. Although, fingerprint from i-frames is faster to extract, the letter one creates a more reliable fingerprint, hence, likely to achieve higher performance. In this subsection, we first investigate (i) the TPR for the mixed media case in NYUAD-MMD. Then, we analyze (ii) the number of frames in an sda-frame, (iii) whether order of frames have an impact, (iv) the number of frames that is required for conventional method perform a similar performance as sda-based method, and finally, we evaluated (v) and (vi) the performance on YouTube and WhatsApp. The experiments in this subsection were done using NYUAD-MMD except (v) and (vi) for which we have used VISION dataset.


{\color{blue}
\paragraph{(i) TPR for mixed-media in \cite{taspinar2019source}}}

Since videos are often long enough, extracting fingerprint from i-frames or all-frames may not cause significant difference in terms of TPR. However, in challenging cases such as matching a video fingerprint to a single image, the difference is likely to be very significant.
In \cite{taspinar2019source}, we investigated the TPR of the mixed-media NYUAD-mmd which contains images and videos from a number of cameras. The videos in the dataset are typically around $40$ seconds, so each video has approx. $1200$ frames. To analyze how the proposed sda-based approach performs compared to i-frames and all-frames, we have done ``Train on videos and test on images" experiment for these three cases. For each video, we created a fingerprint from $40$ i-frames, $40$ sda-frames, and all $1200$ frames of the $40$ second videos. This way we can evaluate whether or not sda-based approach can be useful. Notice that, here, sda-depth is equal to $30$ as we have $40$ sda-frame for each video. 
We then resized the images with bilinear scaling using the resizing factors we have learnt from the ``Train on images, test on videos" experiment and compare the resized images with the video fingerprints (For more details, please see~\cite{taspinar2019source}). 

\begin{table}[!ht]
\centering
\caption{TPR comparison of i-, sda-, all-frames for ``train on videos, test on images"}
\vspace{-0.3em}

\begin{tabular}{ |c|c|c|c|c| } 
    \hline
    type           & $\#match$ & $\#comparison$  & $ TPR $  & $\overline{PCE}$ \\  \hline
    i-frame        &   15070   & 23571    & 63.93\%      &  379  \\  \hline
    sda-frame      &   18849   & 23571    & 79.97\%      &  844  \\  \hline
    all-frame      &   19598   & 23571    & 83.14\%      &  879  \\  \hline
\end{tabular}
\label{table:vF2iN}
\vspace{-0.3em}
\end{table}



Table~\ref{table:vF2iN} compares the average PCE and TPR when fingerprint is obtained using these three approaches. When the fingerprints are obtained using only i-frames, $63.07\%$ of the images can be correctly attributed to their sources, and $82.85\%$ when all-frames are used. The proposed sda-based approach achieve slightly less that all-frames with TPR of $79.97\%$. %As seen, sda-frame achieves $4.89\%$ less than all-frames and $14.89\%$ more than i-frames which shows it can be used as a middle way between i-frames only and all-frames approaches. 


\begin{table}[!ht]
\centering
\caption{Time for video fingerprint extraction in second}
\vspace{-0.3em}
\begin{tabular}{|c|c|c|c|}
\hline
type           &  averaging & I/O + denoising  & total      \\ \hline
i-frame        & 0          & 50-x             & 50         \\ \hline
sda-frame      & 14         & 50-x             & 63        \\ \hline
all-frame      & 0          & 1373-x           & 1373       \\ \hline
\end{tabular}
\label{tbl:vF_extraction}
\vspace{-1em}
\end{table}

To understand how much time improvement can be achieved using sda, we estimated fingerprint extraction time for a 40-second FullHD video captured @30 FPS. Table~\ref{tbl:vF_extraction} compares the average times for these approaches that it takes 50, 63, 1373 seconds for i-frames, sda-frames and all-frames, respectively. This results show that due to the superiority of sda-based fingerprint extraction over i-frame based, sda-based approach can easily replace commonly used i-frame based approach. Moreover, its accuracy is very close to all-frames based approach with a speedup of $22$ times. 

Notice that, the choice of sda-depth (i.e., $30$) is for comparison purpose. In the following experiment, we will investigate what is a good value for this.
% The results show that choosing only i-frames due to its low time-complexity is not the most effective solution in terms of performance for difficult cases such as mixed media. On the other hand, 


% Instead of using only i-frames, sda-based approach may significantly 

% These results show that the proposed approach can be a middle solution for fingerprint extraction from videos. %This technique compromises from performance to achieve a significant speed up.
% Furthermore, as mentioned in Section~\ref{sec:approach:sda_picture}, when the video is long enough (i.e. few minutes), more frames can be used in sda-frame which is expected to improve the performance.



{\color{blue}
\paragraph{Number of frames in sda-frame}}
% 0.8314&0.82250.8130&0.7997&0.7985&0.8005&0.7977

To understand the schema, it is crucial to examine how the performance changes as $g$ (number of frames to be averaged for an sda-frame) changes. Given a video of $k$ frames (in our case approx. $1200$ frames), we divided $n$ into groups of $g = 1, 5, 10, 30, 50, 200, 1200$. Therefore, $d = 1200, 240, 120, 40, 24, 6, 1$ sda-frames were created, respectively. When $g = 1$, the technique becomes same as using all frames whereas when $p = 1200$, all frames are used to create a single sda-frame. 

Each of these fingerprints are then compared with the noise all images from the same cameras in the above experiment. 

Figure~\ref{figure:experiment:num_image_sda} shows the ROC curves for each sda-level (i.e. $p$). The results show that the sda-level achieving the highest performance are $p = 1$ and then $30$ whereas the lowest performing one is when $1200$ and $200$. Because $p = 1$ is same as conventional approach, this is an expected result. Similarly, when $p = 1200, 200$, the results were expected to be lowest. 


\begin{table}[!ht]
\centering
\caption{Sda-depth}
\label{tbl:sda_dept}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
	& 1 	& 5 	& 10 	& 30  	& 50  & 200 & 1200 \\\hline
TPR ($\%$)	& 83.14 	& 82.25	& 81.30 & 79.97 & 79.8  & 80.05 & 79.77 \\\hline
PCE	& 879  	&  864		& 852 & 845	& 852 & 876	& 925	   \\\hline
time(sec)& 1373	&	276	 &142	& 62 	& 48   &	32	& 27 \\ \hline
\end{tabular}
\end{table}


\begin{figure} [!ht]
\centering
{\includegraphics[keepaspectratio=true,width=82mm]{images/results/num_image_sda/num_image.jpg}}
\caption{The ROC curves for varying sda-levels}
\label{figure:experiment:num_image_sda}
\end{figure}

Table~\ref{table:auc:num_image} shows the Area Under Curve (AUC) for Figure~\ref{figure:experiment:num_image_sda}. 


\begin{table}[!ht]
\centering
\caption{AUC for proposed and conventional methods}
\label{table:auc:num_image}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
    $p$      & 1     & 5      & 10    & 30     & 50    & 200   & 1200  \\ \hline
    auc      & 0.946 & 0.9195 & 0.912 & 0.929  & 0.91 & 0.913 & 0.879 \\ \hline
\end{tabular}
\end{table}



\paragraph{{\color{blue}Order of frames}}
A video is a set of sequential frames that each frame has significant similarity with previous frames. This section analyzes if the order of video has any impact on the proposed approach. In other words, our goal is to evaluate whether the performance or average PCE will change if the video frames are shuffled before sda-frames are created. For this purpose, we compared the TPR of when the images in sda-frames are ordered and they are shuffled in the same experimental setting above for a the sda-depth we used above. Clearly, for sda-depth of $1$ and $1200$, there will be no difference because the same sda-image(s) will be denoised and average. For example, when sda-depth is $1200$, there will be only one sda-frame for both ordered and shuffled case.  

\begin{table}[!ht]
\centering
\caption{Effect of order of frames on TPR: REDO}
\label{table:exp:order}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
           & $1$    & $5$   & $10$  & $30$  & $50$  & $200$ & $1200$ \\ \hline
ordered    & 83.14 	& 82.25	& 81.30 & 79.97 & 79.85 & 80.05 & 79.77 \\ \hline
shuffled   & 83.14  & 82.35 & 81.32 & 80.09 & 79.82 & 80.15 & 79.77 \\ \hline
\end{tabular}

\end{table}

As seen in Fig.~\ref{table:exp:order}, the order of frames doesn't have a significant impact on TPR. In most cases, there is a very slim difference. Overall, neither is has significant difference in terms of TPR. However, random access to frames is not as efficient as ordered access. Since p- and b- frames requires previous i-frames to be read first which makes the shuffled one will be significantly slower. For example, when the sda-depth is $30$, a fingerprint from the same video (as in Table~\ref{tbl:vF_extraction}) takes $299$ seconds with random access instead of $63$ seconds. If all the frames are extracted first, approx. 7 GB temporary storage is required for an uncompressed format which also will increase the I/O time. Overall, the ordered version is favorable as the very small performance improvement of shuffling comes at an expense of significant increase on either storage usage or time requirement. 


\paragraph{{\color{red}(iv) The number of frames to achieve similar TPR}}
Finally, it is known that the quality of fingerprint is not linearly improving as the number of frames increases. After a certain number of frames, the improvement in fingerprint quality gets smaller. In other words, it is possible to say that the TPR or PCE achieved using all $k$ frames (in our case $1200$), can be achieved using $k-l$ frames. Therefore, if $k-l$ frames are used instead of $k$, $\frac{l}{k}$ times speed up can be achieved. In this experiment, our goal is to find an approximate value of $l$ that achieves similar TPR and PCE as sda-frames. Specifically, we estimated TPR of fingerprints obtained using the first $100, 200, 300, \dots 1200$ frames as well as sda-frame from $1200$ frames whose depth is $1, 5, 10, 30, 50, 200,$ and $1200$ which is already available from Table~\ref{table:exp:order}.

Table A shows ...


\paragraph{{\color{blue}Train on Facebook images, test on YouTube videos}}
From the previous experiments, we know that the sda-based fingerprint extraction can help achieve a significant speedup for both videos and images with a very small loss in performance which can be overcome by increasing the number of still images used for fingerprint extraction if available. (See experiment x for images, and y for videos). In this part, our goal is to show that the proposed method can be successfully applied to social media. Specifically, in this part, we will do ``Train on Facebook images, test on YouTube videos" experiment. The importance of this experiment is both media sharing services contains billions of visual media that the conventional fingerprint extraction approaches from these web pages has very high time complexity. Therefore, fingerprint extraction methods (along with search techniques) that speeds up the search is highly crucial.

In this experiment, for each camera in VISION dataset that has non-stabilized videos, we created fingerprints from $100$ Facebook images (i.e., the ones labeled FBH) using conventional fingerprint extraction methods. 
We then created fingerprints from all non-stabilized YouTube videos (i.e., the ones labeled flatYT, indoorYT, and outdoorYT) using only i-frames, sda-50, sda-200, sda-600, and all-frames. Here, we used the first $60$ seconds of YouTube videos to extract the above fingerprints. When we use sda- or all-frames, we approx. use $1800$ frames for each video whereas for the first $60$ seconds of the videos have $31.3$ i-frames on average. 

In this experiment, we correlated the image fingerprints with each video fingerprint of each type using the efficient search proposed in ~\cite{taspinar2019source} and a total of $343$ pair have been compared for each fingerprint type. 

Table~\ref{tbl:exp:ns:fb_yt} shows the TPR of these correlations. Similar to ``Train on videos, test on images" experiment, these results show that for fingerprints obtained from Facebook images matches with $81.34\%$ of the videos for sda-50 which is higher than both all-frames and i-frames. On the other hand, all-frames achieves slightly lower performance, fingerprints from i-frames yield approx. $30\%$ lower TPR for this setting. This results show that sda-based approach is a good replacement for usage of i-frames or all-frames for this case.

\begin{table}[!ht]
\centering
\caption{TPR of different fingerprint types when a fingerprint from Facebook images and another from  YouTube videos are correlated}
\label{tbl:exp:ns:fb_yt}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & i      & sda-50   & sda-200  & sda-600  & all-   \\ \hline
TPR & 0.5160 & 0.8134 & 0.7988 & 0.7813 & 0.7959 \\ \hline
\end{tabular}
\end{table}


\paragraph{{\color{blue}Train and test on YouTube videos}}
This experiment aims to explore the performance achieved when two video fingerprints are correlated. Here, similar to the above experiment, we used the three fingerprints of each YouTube video. We correlate each video fingerprint with the others of the same type taken by the same camera. In other words, the fingerprints obtained from i-frames are correlated only the ones extracted using i-frames. The same is valid for sda- and all-frames. This way, a total of $3124$ correlation has been done for each type. 

Table~\ref{tbl:exp:ns:2yt} show that the fingerprints from i-frames results in significantly worse performance compared to sda- and all-frames. Moreover, the fingerprint extracted from all-frames takes 50x more times compared sda-frames while the performance is $x\%$ higher. These results differs slightly from the previous results. One reason the videos that are labeled ``still" and ``outdoor" tend to give lower PCE values for fingerprint from sda-frames compared to all-frames.
It is still show that sda-frames are always superior compared to i-frames in both time and speed.

\begin{table}[!ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & i      & sda-50   & sda-200  & sda-600  & all-   \\ \hline
TPR & 0.2929 & 0.5954 & 0.5458 & 0.5074 & 0.6962 \\ \hline
\end{tabular}
\caption{TPR of different fingerprint types when two YouTube videos are correlated}
\label{tbl:exp:ns:2yt}
\end{table}

% ------------------------------------------
\subsection{Stabilized videos}
\label{sec:exp:stab}

A recent research [cite] has shown that when a stabilized video is at least 4-minute long, it can be attributed to its source camera when all its frames (i.e., $7200$ frames) are denoised. As mentioned in \ref{sec:background}, extracting fingerprint from so many frames can take a very long time, hence, may not be practical in some settings. A potential alternative for this problem is the usage of SDA-frames which may lead to a significant speed up. To evaluate this, we captured $4+$ minute stabilized videos from $10$ cameras, a total of $100$ videos. As shown in \cite{taspinar2016source, iuliani2017hybrid}, the first frame of the videos are typically not geometrically transformed. But as \cite{mandelli2018facing} pointed out, they may not always be available or some cameras may transform them as well, hence, we ignored those frames.

For this experiment, we extracted fingerprint from $1000, 2000,\dots 7000$ frames using conventional method. Then, we correlated each fingerprint with other fingerprints from the same camera that are created using the same number of frames to get $H_1$ hypothesis. Similarly, we compared each fingerprint with other fingerprints from random cameras to obtain $H_0$ hypothesis.
For the proposed method we used $7000$ frames of each video and we created sda-groups of $5, 10, 20, 30, 50, 500$. This way we obtained $1400, 700, 350, 234, 140, 14$ sda-frames, respectively. Then, we obtained $6$ fingerprints using these sda-frames and correlated each fingerprint with other fingerprints of same category ($H_1$ and $H_0$ are obtained in similar manner as above). 
Table XXX shows the average TPR of  


\begin{table}[!ht]
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
       & 20 sec & 40 sec & 60 sec & 80 sec & 10 sec \\ \hline
all    & 0.5321 & 0.8705 & 0.9659 & 0.9918 & 0.9981 \\ \hline
sda-50 & 0.0346 & 0.2033 & 0.4239 & 0.5938 & 0.7172 \\ \hline
\end{tabular}
\end{table}

==> sections/old/intro_bkp.tex <==
\section{Introduction}
\label{sec:intro}

% SAMET - Overall, we are on Track. But I think, we have to change the structure bit as follows.

% \textbf{INTRO:}

% (i) Motivation (Research on PRNU)
% (ii) Good PRNU methods available for images (some citations)
% (iii) PRNU for video unexplored (some citations)---
% (iv) What are the challenges for video. Here, we can discuss how to choose frames for fingerprint computation.  
% (v) Then we discuss about what we proposed. Basically, our approach to address above challenges


Digital forensics facilitate investigation of digital crimes which may have previously been undiscovered. This helps law enforcement agencies bring criminals to justice. 
One of the well-studied techniques in digital forensics is source camera attribution which focuses on determining the camera that has captured a particular visual media object (i.e., an image or a video) \cite{kharrazi2004blind, lukas2005digital}. Although various attempts have been made \cite{bayram2005source, san2006source, long2006image}, the most successful among them is Photo Response Non-Uniformity (PRNU)-based approach \cite{lukas2006digital}.
%One of the well-studied techniques in digital forensics is source camera attribution via Photo Response Non-Uniformity (PRNU) \cite{lukas:camera, lukas2006digital}. It is a technique to determine the camera that has captured a particular visual media object (i.e., an image or a video) that is under questioning\cite{kharrazi2004blind}. 
The technique is based on the fact that the camera sensors are imperfect and the sensitivity of sensing elements (i.e., pixels) to light is inhomogeneous. Because this artifact is as a result of the manufacturing process, PRNU noise appears to be random and unique to each imaging sensor.
In other words, any visual media can be attributed to its origin camera using the PRNU-based technique. To achieve this, one need to collect multiple images or video(s) captured by a camera to ``learn" its unique PRNU-based camera fingerprint. Then, the PRNU noise of the visual media under questioning is extracted and correlated with the camera fingerprint. The strength of this correlation indicates how likely it is that the camera has captured the query visual media. 
% This means if the visual media is captured by the camera, the correlation will be high and a match decision will be given, otherwise

Previous research has shown that PRNU-based camera fingerprint is hard to remove or forge and survives a multitude of operations performed on the image such as cropping and/or scaling \cite{jessica:crop}, compression \cite{alles2008source, kurt:prnu}, blurring \cite{alles2008source}, and even printing and scanning \cite{ lukas:printed}. 

PRNU based technique has been used mainly ... crimes, however, it research has shown that it can be used in image tamper detection~\cite{chierchia2010influence, korus2017multi} , image clustering~\cite{marra2017blind, caldelli2010fast}, file carving~\cite{durmus2017image} and so on. 
% Although most research were image-centric, there are research on applying it to video domain. [citations in this paragraph]. 

The simplest use case of the technique is to check if a visual media object is captured by a certain suspect camera. When a suspect camera is not available, the problem becomes to determine the origin camera in the wild (i.e., identification). For successful identification, one may need to collect visual media of a large number of cameras (e.g., from Facebook, Flickr, and social media) and extract their fingerprints. This could lead to two main issues: the time-complexity of search and extraction of camera fingerprints.

% Write about search ... (linear search), short digest, composite, hybrid, binarization etc. Any time a query visual media comes, the media need to be searched in the entire dataset (or part of it). 

For efficient fingerprint matching in large databases, various approaches have been proposed. Fridrich at al. \cite{goljan2010managing} proposed the use of fingerprint digests in which a subset of fingerprint elements having highest sensitivity is used instead of the entire fingerprint. Bayram {\em et al.} \cite{bayram2012efficient} introduced binarization that each fingerprint element is represented by a single bit. Then, Valsesia {\em et al.} \cite{valsesia:ranproj} proposed the idea of applying random projections to reduce fingerprint dimension. Their results show the technique can perform better in comparison to fingerprint digest when same storage limitations are applied. These methods reduces the fingerprint size in an effective way such that they can speed up the process. On the other hand, Bayram et. al. introduced group testing via composite fingerprint that focuses on decrease the number of correlation rather than decreasing the size (storage) of a fingerprint. Later, Taspinar et al. \cite{taspinar2017fast} utilize both decreasing the size of a fingerprint and the number of correlation and come up hybrid search which can speed up the search up to 400 times.

% The source camera attribution problem can be evaluated under two main categories: verification and identification. In the first case, there is at least one suspect camera which may have taken the anonymous media and the goal is to verify if the media is indeed captured by the suspect camera. In the letter case, there is no suspect camera, so the source camera of the anonymous media must be searched for in the wild. Since the number of cameras in the world is on the order of billions, for a successful identification, investigators may need to collect a huge number of camera fingerprints extracted from videos and images. 

On the other hand, the speed of fingerprint extraction has not been studied as much. This is partly because fingerprint extraction is a ``one time" operation which means each visual media in the dataset will be denoised only once.
Initially, Lukas et al. \cite{lukas2006digital} have proposed to use wavelet filter to denoise the media\cite{mihcak:filter} and Jessica et al. have suggested denoising $20-30$ JPEG images may be sufficient to extract a "good quality" camera fingerprint [cite]. Although, to the best of our knowledge, no such number for videos is given in any research but it is reasonable to assume this number is significantly greater because of strong compression applied on videos in comparison to images. 

Two straightforward ways to extract fingerprints from videos are using least compressed frames (i.e., I-frames) or all frames (i.e., I-, P-, B-frames) of a video \cite{chuang2011exploring}. According to Chuang et al. fingerprints obtained from I-frames may not be very reliable (i.e., low performance), whereas using all frames produces more reliable fingerprints can be obtained but it is significantly slower. For example, given a 1-minute Full HD video $@30$FPS (with approx. $60$ I-frames and a total of $1800$ frames), it takes 1-2 minute(s) to extract a fingerprint, whereas it may take around $30-40$ minutes if all frames are used. Although using only I-frames may be enough in many cases such as correlation of two long videos, for challenging task such as ``Training on a video, testing on a single image", the technique may fail if only I-frames are used.

% Since denoising is a computationally expensive operation, denoising so many images/frames will be time consuming and not practical for big data. 
Moreover, the usage of advanced video processing techniques such as video stabilization make it harder to do source attribution \cite{taspinar2016source, iuliani2017hybrid} as it cause misalignment between camera fingerprint and PRNU noise. This issue can be overcome by denoising a large number of video frames (i.e., $>5000$) if available. [cite Darpa presentation]
% \textbf{IS THERE OTHER RESEARCH ABOUT NUMBER OF FRAMES/IMAGES ETC} 
%[Darpa group] proposes that when a $4$ minute stabilized video is available, extracting fingerprint using the conventional approach \cite{lukas2006digital} (i.e., without reversing the geometric transformations) helps obtain a reliable camera fingerprint


Given the amount of visual media that can be used to create a big fingerprint dataset and the time it takes to extract a camera fingerprint from a set of images or a video, this is a valid and noteworthy issue that needs to be addressed.

% For H264 video encoding, most widely used compression standard, there are $3$ types of frames: intra-coded (I-), predicted (P-), and bi-directional predicted (B-) frames. I-frames have the lowest compression while B-frames have the highest. As a result, the PRNU noise of an I-frame typically has "better" quality than a P- or B-frame.

% The two straightforward ways to create a camera fingerprint are to use either I-frames or all frames of a video. Creating a fingerprint from a low number of I-frames is expected to create a low-quality camera fingerprint which yields many false negatives (i.e., the technique is unable to attribute a video to its source camera) whereas usage of all/most frames will take more processing time (a one-minute Full HD $@30FPS$ video can take $45$ minutes when all $1800$ frames are used). Chuang \textit{et. al.} \cite{chuang2011exploring} compared the performance of extracting camera fingerprint from $50$ I-frames, $50$ P-frames which shows pattern noise estimated from I-frames yields better PCE results. Furthermore, Scheelen \textit{et. al} shows the performance increases as the number of frames increases \cite{scheelen2012camera}.
 
This paper proposes to use a computation-efficient frame averaging method, which gets the arithmetic mean of still images (i.e., images or video frames) in spatial domain, for fingerprint extraction. For example, given a video with $m$ frames, $d$ non-intersecting equal-sized subgroups (i.e., each subgroup has $g = \frac{m}{d}$ frames) are formed and a \textit{Spatial Domain Averaged frame (SDA-frame)} (Figure~\ref{Fig:avgframe}) is created from each subgroup. Each SDA-frame is denoised and a camera fingerprint estimate is created similar manner as \cite{lukas2006digital}.
%The benefit of this method is all $m$ frames are used but $g$ denoising operation is done which significantly speeds up the fingerprint extraction.
The benefit of this technique is when $m$ is a large number (i.e., bigger than proposed numbers), instead of discarding some of the still images, all of them can be used to speed up the fingerprint extraction process. 

Experiment with VISION dataset~\cite{shullani2017vision} and NYUAD-MMD~\cite{taspinar2019source} show that the proposed approach can be useful for challenging video cases when many frames are available as well as for images. When it is used for stabilized or non-stabilized videos, it can help speed up X times. On the other hand, for images, $4$ to $14$ times speed up can be achieved with no loss in performance depending on the number of images and their content (i.e., textured or flat-field).

% Experiment with a dataset of $6892$ images, $301$ videos taken from $78$ cameras shows that for the first two use cases, the current work has a true positive rates $todo$ and $todo$ respectively. For these cases, the previous works reported true positive rate $todo$ and $todo$ respectively (by experimenting with a smaller dataset).

%The rest of the paper has been organized as follows. Section~\ref{sec:background} summarizes the PRNU and provide an overview of how an image and a video is captured by a camera. Section~\ref{sec:our_approach} explains the proposed brute forced-based fingerprint comparison method. Section~\ref{sec:experiment} reports  experimental result, and Section~\ref{sec:conclusion} concludes.



==> sections/old/our_approach_bkp.tex <==
\section{Our Approach}
\label{sec:approach}

This paper investigates the effectiveness of the usage of spatial domain image averaging technique for camera fingerprint extraction. The main goal is to create a reliable camera fingerprint from images or video frames in an efficient way when many of them are available. This goal is achieved by creating an averaging image (or frame) from multiple given images  (as shown in Figure~\ref{Fig:avgframe}) and using this average image in place of an individual image (for example, as shown in Figure~\ref{Fig:avgframe} using the SDA-frame in the place of 1st image) in computing the fingerprint.

%In this section, first the spatial domain picture averaging idea to compute a camera fingerprint from images and non-stabilized videos has been discussed. 

% \begin{figure}[!ht]
%     \centering
%     \subfloat[Example of a binning scheme (Obtained from ~\cite{jin2012analysis})]
%     {\label{Fig:binning}\includegraphics[width=66mm]{images/bin_lineskip/binning}}
    
%     \subfloat[Example of a line-skipping scheme]
%     {\label{Fig:lineskip}\includegraphics[width=66mm]{images/bin_lineskip/line_skipping}}
%     \caption{Two different in-camera resizing schemes}
%     \label{Fig:resizing schemes}
% \vspace{-2mm}
% \end{figure}

\begin{figure}[!ht]
\centering
\subfloat [1st] {\includegraphics[height=15mm]{images/avg_frame/im1.jpg}}~
\subfloat [2nd] {\includegraphics[height=15mm]{images/avg_frame/im2.jpg}}~
\subfloat [3rd] {\includegraphics[height=15mm]{images/avg_frame/im3.jpg}}~
\subfloat [SDA-frame] {\includegraphics[height=16mm]{images/avg_frame/avg.jpg}}
\caption{SDA-frame is the average of 1st, 2nd, and 3rd frames.}
\label{Fig:avgframe}
\end{figure}

%\subsection{Spatial Domain Averaged Picture}
%\label{sec:approach:sda_picture}
%Given a set of still images taken by a "known camera", the first step is to extract its reference camera fingerprint which will, later, be compared against the PRNU noise of any visual media under questioning. This will help investigators prove if the questioned visual media is captured by the "known camera". The existing methods for camera fingerprint extraction (See Background) choose $m$ still images out of $n$ that is captured by the known camera ($1 \leq m \leq n$). The two weaknesses of this approach are \textit{(i)} low source attribution performance (i.e. unreliable camera fingerprint) when $m$ is low and \textit{(ii)} slow fingerprint extraction when $m$ is high. This research proposes an alternative technique, the usage Spatial Domain Averaged (sda-) picture that may significantly speed up the fingerprint extraction process when the number of still images is very high. Although some improvements can be achieved for images, the speed up is more compelling for videos.  

%Given $m$ pictures to compute the camera fingerprint, the proposed method divides the pictures are divided into $d$ disjoint sets of equal number of pictures. An sda-frame is then computed from each set using the arithmetic mean on member pictures. Each picture $F$ of a set can be considered as a matrix of $3 \times r$ color components (i.e., R, G, and B), where $r$ is the dimension of the pictures. Thus, the sda-frame $F_{sda}$ of the set can be computed as $F_{sda} = \frac{F_1 + F_2 + \dots + F_{m/d}}{m/d}$ (each set has $m/d$ elements).% Figure~\ref{Fig:avgframe} shows an example of an sda-frame computed from three images.
%Similar to how conventional method works (discussed in Section~\ref{sec:background:PRNU}), the $k$ sda-frames are then denoised, and the $k$ noise are used to obtain the camera fingerprint. 

%The frame averaging method uses all $n$ frames of a video (i.e., all $n$ i-frames p-frames and b-frames) to compute the camera fingerprint. The $n$ frames are divided into $k$ disjoint sets of equal number of frames. An average frame (called as \textit{avg-frame}) is computed from each set using the arithmetic mean on member frames. Each frame $F$ of a set can be considered as a matrix of $3 \times r$ color components (i.e., R, G, and B), where $r$ is the dimension of the fame. The avg-frame $F_{avg}$ of the set can be computed as $F_{avg} = \frac{F_1 + F_2 + \dots + F_{n/k}}{n/k}$ (each set has $n/k$ elements). Figure~\ref{Fig:avgframe} shows an example of an avg-frame computed from three frames. The $k$ avg-frames are then denoised, and the $k$ noise are further averaged to obtain the camera fingerprint. In this paper, the value of $k$ is fixed to $30$, as a GoP (Group of Pictures) of the video in most cases contains $30$ frames. 

The proposed picture averaging idea is inspired by the fact that the averaging operation can be used as a filter for reducing some random noise from an image. In the PRNU-based method, a random noise can be either a pre-denoising random noise such as quantization noise, compression noise or post-denoising random noise which is created due to the denoising operation. The picture averaging method can reduce the pre-denoising random noise and make a stronger PRNU noise. However, since post-denoising random noise cannot removed, several sda-frames will still be required. 
%the random noise $\psi$ (Equation~\ref{Eqn:im_noise}) contains both pre-denoising random noise $\psi_1$ (such as quantization noise, compression noise) and post-denoising random noise $\psi_2$. While the picture averaging can reduce $\psi_1$, the PRNU noise averaging can reduce both $\psi_1$ and $\psi_2$. In the case of the proposed picture averaging method, all the frames are used to reduce $\psi_1$ and PRNU noise of only $k$ sda-frames are used to reduce $\psi_2$. 

\subsection{Mathematical Analysis}
\label{sec:math}
This section provides mathematical justification of the
proposed sda-frames scheme. To this end, we
first provide some mathematical background of the conventional (non-sda-based) PRNU-based method, and then discuss our scheme.

\subsubsection{Conventional method}
As discussed in Section~\ref{sec:background}, in the conventional method, the camera fingerprint is estimated from $n$ given images. Each image $I$ can be modeled as $I = I_0 + I_0K + \psi_1$, where $\psi_1$ is the pre-denoising random noise (Equation~\ref{Eq:im_noise}). 

To estimate the PRNU noise $K$, a denoising filter (such as Wavelet Denoising\cite{mihcak1999low}, BM3D\cite{dabov2009bm3d}) is used to estimate the noise free signal $I^0$. Using the denoising filter, the noise residual, $W = I^{(0)}K + \psi_1 + \psi_2$, where $\psi_2$ is the post-denoising noise, is obtained. Then, the estimated PRNU noise $\hat{K}$ can be estimated  using Maximum Likelihood Estimation (MLE) as
\begin{equation}
    \hat{K} = \frac{\sum_{i=1}^{n} W_i . I_i}{\sum_{i=1}^{n} I_i^2}
\end{equation}
where $W_i$ is noise pattern extracted from $I_i$, and all the operations are element-wise. %Jessica et al suggests when $N$ is more than 20, a reliable camera fingerprint estimate can be extracted from images, [citation].  Talk more about images.

Note that in the estimated PRNU noise $\hat{K}$, the PRNU noise is the signal of interest whereas the random noise $\psi_1$ and $\psi_2$ are the unwanted noise. The quality of $\hat{K}$'s can be assessed from its variance $Var(\hat{K})$. The lower the variance, the higher the quality (and vice-versa). Assuming that $\psi_1$ and $\psi_2$ are White Gaussian noise with variances $\sigma_1^2$ and $\sigma_2^2$ respectively, the $Var(\hat{K})$ can be found as (using Cramer-Rao Lower Bound as shown by Jessica et al.\cite{Jessica:Sensor:2013})
\begin{align} \label{eq:conv1}
    Var(\hat{K}) \ge \frac{\sigma_1^2 + \sigma_2^2}{\sum_{i=1}^n I_i^2}.
\end{align}
Thus a better PRNU is obtained from lower $\sigma_1^2$ (smoother image) and $\sigma_2^2$, and high luminance.

\subsubsection{Proposed Sda-based method}
We will mathematically derive the variance of the estimated PRNU noise obtained using our approach (i.e., sda-frame). We will then compare this variance with the variance obtained by conventional approach (in Equation~\ref{eq:conv1}).    

Suppose $I_1, I_2, \dots, I_m$ are $m$ given pictures to compute the camera fingerprint. In our approach, these $m$ pictures are divided into $d = \frac{m}{g}$ disjoint sets of equal number of pictures with $g$ pictures in each set. From each set, an average picture is computed using the arithmetic mean on member pictures. Thereafter, the process is similar to the conventional approach. Each average picture is denoised, and the PRNU noise is estimated from $d$ noise residuals using the MLE.

Suppose, $I_i^{avg}$ is the average picture obtained from the $i^{th}$ image-set. Then 
\begin{equation}
\begin{aligned}
I_i^{avg} &= \frac{\sum_{j=(i-1)g+1}^{ig} I_j}{g} \nonumber \\
          &= \frac{\sum_{j=(i-1)g+1}^{ig} (I^0_j + I^0_jK +\psi_{1,j}) }{g} \nonumber
\end{aligned}
\end{equation}


%The picture averaging (aka frame averaging) has been studied before~\cite{JM:FrameAverage:1992}~\cite{Swindell:FrameAverage:1995}. 
%Although picture averaging can decrease the random noise, it can, however introduce motion blurring~\cite{Nayar:FrameAverage:2004}\cite{Kavanaugh1990}. The motion blurring can degrade the quality of the average image, and hence weaken the estimated PRNU noise. Considering the motion blurring factor, we can write the above equation as 

% \begin{equation}
%     I_i^{avg} = I_i^{0, avg, blur} + I_i^{0, avg, blur}K + \psi_{1, i}^{avg},
%     \label{eq:avg1}
% \end{equation}

% where $I_i^{0, avg, blur} = I_i^{0, avg}*B$ and $I_i^{0, avg}$ is the blur-free image, $B$ is the blurring kernel that degrades the image, and $*$ is the convolution operator. 

%The average image is more blurred when more number of images are used in averaging and the image content differs (citation). On the other hand, with a more number of images in averaging, the average image is more smoothed. As we discussed above, smooth images are better for estimating PRNU. Thus, a tradeoff between the effect due to blurring and smooth content is resulted due to image averaging.% Mathematically finding the value of $g$ that fine balances the effect of blurring and content smoothness is difficult as the derivation depends on the un-predictable image content. In this paper, we empirically obtained the ideal value of $g$ for a particular dataset of images and videos in Section TODO.

We can write the above equation as 
\begin{equation}
    I_i^{avg} = I_i^{0, avg} + I_i^{0, avg}K + \psi_{1, i}^{avg},
    \label{eq:avg1}
\end{equation}
where $I_i^{0, avg}$ is noise free image, and $\psi_{1, i}^{avg}$ is the random noise of the average image. %The random noise also contais the blurring noise that results due to image averaging opeartion.
This random noise can be written as
$$
\psi_{1, i}^{avg} = \frac{\sum_{j=(i-1)g+1}^{ig} \psi_{1,j}}{g}.
$$
Suppose $\sigma_1^2$ is the variance of $\psi_{1}$'s (which is assumed to be white Gaussian noise). Then, using probability theory, the variance of $\psi_{1, i}^{avg}$ is $\frac{\sigma_1^2}{g}$.

Suppose $W^{avg}$ is the noise residual of each average image $I^{avg}$. Then, 
\begin{align}
W^{avg}  &= I^{avg} - F(I^{avg}) \nonumber \\
        &= I^{avg}_{0}K + \psi_{1}^{avg} + \psi_{2}^{\prime}\nonumber,
\end{align} 
where post-denoising noise $\psi_{2}^{\prime} = I^{0, avg} - F(I^{avg}) + \phi$. The $\phi$, such as filter modelling noise, is independent of the averaging operation. Also, the post-denoising noise is assumed to be independent of the content as this is very small \cite{Jessica:Sensor:2013}. Thus, we can assume $\psi_{2}^{\prime} = \psi_{2}$, and hence $\psi_{2}^{\prime}$ have variance $\sigma_2^2$.

Using the MLE, the PRNU can now be estimated from $d$ average frames $I_1^{avg}, I_2^{avg}, \dots, I_d^{avg}$ as
\begin{align} \nonumber
    \hat{K^{avg}} = \frac{\sum_{i=1}^{d} W_i^{avg} . I_i^{avg}}{\sum_{i=1}^{d} \big(I_i^{avg}\big)^2}.
\end{align}

Using the Cramer-Rao Lower Bound, the variance of the estimated PRNU $\hat{K^{avg}}$ can be found as
\begin{align} \label{eq:OurVar}
    Var (\hat{K^{avg}}) \ge \frac{ \frac{\sigma_1^2}{g} + \sigma_2^2}{\sum_{i=1}^d \big(I_i^{avg}\big)^2}.
\end{align}

In an ideal case, we want that the averaging operation does not degrade the quality of the estimated PRNU from the average frames. In other words, we want that $Var (\hat{K^{avg}})$ is approximately equal to the variance from the conventional method $Var (\hat{K})$ as follows
$$
Var (\hat{K^{avg}}) \approx Var (\hat{K}).
$$
Therefore, using the results from Equation~\ref{eq:OurVar} and Equation~\ref{eq:conv1}, the following equation must hold 
$$
\frac{ \frac{\sigma_1^2}{g} + \sigma_2^2}{\sum_{i=1}^d \big(I_i^{avg}\big)^2} \approx \frac{\sigma_1^2 + \sigma_2^2}{\sum_{i=1}^n I_i^2}.
$$
By simplifying the above equation, we get
$$
\frac{ \frac{\sigma_1^2}{g} + \sigma_2^2} {\sigma_1^2 + \sigma_2^2}  \approx \frac  {\sum_{i=1}^d \big(I_i^{avg}\big)^2}  {\sum_{i=1}^n I_i^2}.
$$

Suppose $\frac  {\sum_{i=1}^d (I_i^{avg})^2}  {\sum_{i=1}^n I_i^2} = \frac{d}{n} \times N$, where $N = \frac  {(\sum_{i=1}^d (I_i^{avg})^2)/d}  {(\sum_{i=1}^n I_i^2)/n}$. Note that the value of $N$ is greater than or equal to $1$. Putting these values in the above equation, we get
$$
\frac{d}{n} \times N \approx \frac{ \frac{\sigma_1^2}{g} + \sigma_2^2} {\sigma_1^2 + \sigma_2^2}.
$$
Putting $d=\frac{m}{g}$ in the above equation, we get
$$
\frac{m \times N}{g \times n} \approx \frac{\sigma_1^2 + g \times \sigma_2^2 }{g \times (\sigma_1^2 + \sigma_2^2)}.
$$
or,
\begin{align} \label{eq:finalourapproach}
 m \approx \frac{n}{N} \times \frac{\sigma_1^2 + g \times \sigma_2^2 }{\sigma_1^2 + \sigma_2^2}
\end{align}

As discussed above, $N \ge 1$. Thus, the number of images required in our approach $m$ is greater than equal to the number of images required in the conventional method $n$. Ideally, we would like to have $m$ close to $n$. This can be achieved when $N = 1 + \epsilon$ (where $\epsilon$ is a small value) and $\sigma_2^2$ is also small. In other words, when we have smoother content. 



\subsection{\textbf{Usages}}
\subsubsection{\textbf{Images}}
As mentioned in  \ref{sec:background}, [Jessica] proposes $20-30$ images is required to obtain a good quality camera fingerprint. In many cases, more than $30$ images from a camera might be available that if $30$ images are used, the rest of the images will be discarded in fingerprint extraction step. Instead of discarding those images, the proposed technique can be used in such a way to speed up fingerprint extraction as well as to create a more reliable fingerprint in a shorter time. For example, if $100$ images from a camera is available, instead of omitting $70$ images, a number of sda-frames can be obtained from all (or most of) the  images. Then, with less denoising operations, similar or a better quality fingerprint can be obtained. This will increase the I/O load but significantly decrease the memory load. 

Moreover, the proposed number in [cite jessica] (i.e., $20-30$) is for pristine images or images with low in- or out-camera processing. However, given the ease of image editing and the compression caused by social media more than $30$ images might be needed. This may lead to significant slow-downs in fingerprint extraction. Similar to above, when many images are available, the proposed sda-frame can help speed up. 

Note that, in this section, we assume HDR, zoom or any other source of geometric transformation is turned off for the images.  

\subsubsection{\textbf{Non-Stabilized Videos}}
Non-stabilized videos are (as mentioned in background) resized and cropped with respect to camera sensor. However, these settings are typically fixed for all videos captured by a camera. Hence, all frames of a video are "aligned"\cite{taspinar2017prnu}(MIXED MEDIA). In this case, various frames are available for each video. Because of the high compression applied on a video, so many frames are needed \textit{(more than a few hundred)} such that a reliable fingerprint from the video can be extracted. 




\subsubsection{For Stabilized Videos}


-------------------------------------------------


\label{section:sda4videos}
As mentioned in \ref{sec:background}, each frame of a video is undergone a heavy compression. When a single video frame denoised, the noise residual is highly contaminated with this compression noise, therefore, many frame must be denoised to extract a reliable camera fingerprint. 
Since denoising operation is computationally the most expensive step of camera fingerprint extraction, this process becomes very slow for videos. Hence, the usage of sda-frame for video fingerprint extraction is a very natural case. 


Section 3b (Related work) lays out the existing methods for fingerprint extraction. When the number of frames is fixed, the fingerprint obtained from I-frames is better than P-frames or B-frames in terms of True Positive Rate(TPR). When the fingerprint is obtained from all frames, the TPR (and average PCE) is better than the methods above. However, usage of all-frames significantly increases the time requirement for fingerprint extraction. For example, it takes around $45$ minutes for to extract a camera fingerprint from a $1$~minute Full HD video $@30$FPS (a total of 1800 frames) in a single-threaded Matlab code. 

When a camera fingerprint is extracted from only I-frames, low TPR problem occurs whereas using all-frame causes slow fingerprint extraction process which is not usable when there are several videos in the database. Therefore, it is a big necessity to provide solutions that will help extract fingerprint as fast as from I-frames and perform as good as from all-frames. The usage of sda-frame can help achieve this target. The first step is to divide the video into subgroups of $k$ frames each and sda-frame of each subgroup is obtained (See Section~\ref{sec:approach:sda_picture}) which are then denoised to create a fingerprint.


% \textbf{CAN WE USE IT FOR IMAGE CLUSTERING: i cant see how}



% \subsection{\textbf{Use Cases}}
% \subsubsection{SDA-frame for Videos}
% \label{section:sda4videos}
% As mentioned in \ref{sec:background}, each frame of a video is undergone a heavy compression. When a single video frame denoised, the noise residual is highly contaminated with this compression noise, therefore, many frame must be denoised to extract a reliable camera fingerprint. 
% Since denoising operation is computationally the most expensive step of camera fingerprint extraction, this process becomes very slow for videos. Hence, the usage of sda-frame for video fingerprint extraction is a very natural case. 


% Section 3b (Related work) lays out the existing methods for fingerprint extraction. When the number of frames is fixed, the fingerprint obtained from I-frames is better than P-frames or B-frames in terms of True Positive Rate(TPR). When the fingerprint is obtained from all frames, the TPR (and average PCE) is better than the methods above. However, usage of all-frames significantly increases the time requirement for fingerprint extraction. For example, it takes around $45$ minutes for to extract a camera fingerprint from a $1$~minute Full HD video $@30$FPS (a total of 1800 frames) in a single-threaded Matlab code. 

% When a camera fingerprint is extracted from only I-frames, low TPR problem occurs whereas using all-frame causes slow fingerprint extraction process which is not usable when there are several videos in the database. Therefore, it is a big necessity to provide solutions that will help extract fingerprint as fast as from I-frames and perform as good as from all-frames. The usage of sda-frame can help achieve this target. The first step is to divide the video into subgroups of $k$ frames each and sda-frame of each subgroup is obtained (See Section~\ref{sec:approach:sda_picture}) which are then denoised to create a fingerprint.


% % ---I DIDNT LIKE HOW I EXPLAINED, MAKE IT BETTER!!!
% % Besides decreasing the time complexity for fingerprint extraction, sda-frame can be used as a solution to other \textbf{video forensics issues}. Since the frames of a video are highly compressed, the noise of two frames from the same video are likely to not match. 
% % The PCE result of the noise of two frames from the same video tends to be very low (below threshold) unless they are consecutive frames. This is due to the very strong compression applied to the videos. Therefore, it is almost impossible to tell if the two video frames are taken from the same

% \textbf{STABILITY DETECTION}
% \cite{taspinar2016source} has proposed stability detection algorithm that divides a video into two halves and a camera fingerprint is extracted from each half by denoising the I-frames. Then, the fingerprints are correlated to detect if the video is stabilized. However, the process, again, requires many denoising of the frames. Because the PRNU noise of each sda-frame is a much stronger signal than the noise of individual frames, the proposed approach can help achieve stability detection by only few denoising instead of many. 

% %Another use case for this idea for videos is the detection of \textit{sequential foreign frames} which are multiple consecutive frames that are from another camera added to the video. To detect \textit{sequential foreign frames}, the sda-frame of each Group of Picture (GoP: from one I-frame to the next one, typically 30 frames), is extracted and the correlation of PRNU noise of each sda-frame is expected to be high; the ones which are below the threshold are potentially from another camera. One weakness of this idea is if the number of foreign frames are not consecutive or not a high number, the proposed idea will fail. 


% % \textbf{NOPE: WE NEED TO ANALYZE THE EFFECT OF NUMBER OF FRAMES WHY $30$ NOT $15$ In this paper, the value of $k$ is fixed to $30$, as a GoP (Group of Pictures) of the video in most cases contains $30$ frames. }
% % \textbf{BEST IS TO TEST WITH $15, 30, 60$}

% % \textbf{SHUFFLING THE FRAMES}


% \subsubsection{SDA-frame for Images}
% The sda-frame can be used for videos as well as images. [Jessica] proposes $20-30$ images are required to obtain a good quality camera fingerprint. One of the reasons for this limitation is time requirement, i.e. the more images used for fingerprint extraction, the more time it takes. Therefore, one could ignore the rest of the images if the camera has more than $30$ images. The proposed technique can be used in such cases to speed up and/or create a better quality fingerprint in a shorter time. For example, if the camera has $100$ images, instead of omitting $70$ images, a number of sda-frames can be obtained from all (or most of) the  images. Hence, a similar/better quality fingerprint can be created with less denoising operations. This will increase the I/O load but significantly decrease the memory load. 

% % \textbf{CAN WE USE IT FOR IMAGE CLUSTERING: i cant see how}



==> sections/old/z6_experiment.tex <==
\section{Experiment}
\label{sec:experiment}

This section experimentally validates the theoretical analysis as well as evaluates the effectiveness of the proposed fingerprint extraction technique. Moreover, it gives an insight for various aspect of it. Specifically, experimental analysis have been conducted to enlighten how the proposed technique can be effective for non-stabilized or stabilized videos as well as images. NYUAD-MMD \cite{taspinar2019source} and VISION dataset \cite{shullani2017vision} were used for these experiments. The experimental analysis also investigates when the visual media is obtained from social media, namely, Facebook, YouTube, or WhatsApp.

The implementations for this paper are done using Matlab 2016a on Windows 7 PC with 32 GB memory and Intel Xeon(R) E5-2687W v2 @3.40GHz CPU. The wavelet denoising algorithm \cite{mihcak:filter} has been used to obtain fingerprint and PRNU noise. PCE and NCC  methods are used for comparison. The preset threshold of 60 \cite{jessica:crop} is considered as threshold that when the PCE results two fingerprints are less than this threshold, they are considered to null hypothesis ($H_0$), otherwise, alternate hypothesis ($H_1$).

% \textbf{Should we explain datasets here? We use nyuad-mmd and vision...}

\subsection{Validation of theoretical analysis}
As we mentioned the above theoretical analysis has two main contributions: conventional and sda-based fingerprints performs similarly for smooth (flatfield) images, and sda-based approach requires more images that conventional one to achieve similar performance when images are textured. In this subsection, we will experimentally verify these observations using the flatfield and textured images in VISION dataset~\cite{shullani2017vision} which is a comprehensive data containing flat-field and textured images. 

\paragraph{{\color{blue}Studying the effect of smoothness}}
%As Section~\ref{sec:math} shows image texture(content) is one of the most significant noise source that differs conventional fingerprint extraction method from usage of sda-frame. The conventional method can remove/decrease content noise whereas usage of sda-frame fails to achieve it. Therefore, the difference between conventional and proposed approaches is expected to be minimized when training set consists of flat-field images. In other words, the experimental results (such as average PCE, TPR and so on.) should have a little or no difference for conventional and proposed fingerprint extraction methods when the training set is flat-field images whereas high difference between the two approaches when the training images are textured.

To verify the first observation of the theoretical analysis, we created the first type of fingerprint from up to $50$ textured images (i.e., the ones labelled as nat in VISION) and another type from $50$ flatfield images (i.e., the ones labelled as flat in VISION). For each fingerprint type, two categories of fingerprints were obtained: one using the conventional approach and another using the sda-frame approach. From each of these categories, we extracted fingerprints using $5$, $10$, $20$, $30$, and $50$ images. Therefore, a total of $20$ fingerprints were obtained for each camera ($2$ types of images, $2$: fingerprint extraction techniques, $5$: for different number of images used for extraction). Each of these fingerprints is correlated with the PRNU noise of the rest of the images from the same camera which consists of both textured and flat-field images. 
While doing this we employed block by block comparison to better highlight the differences in TPR where each block is $500\times500$.


% Table~\ref{fig:exp:texture:pce} shows the average PCE of the comparison of fingerprints with the PRNU noise of the same camera images ($H_1$ hypothesis). For example, when fingerprint is extracted from $20$ flatfield images using sda-frame for fingerprint extraction, the average PCE is $24,172$, whereas using conventional approach, it is equal to $27,316$.  


\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={1.8cm 20.6cm 4.8cm 3.57cm},clip]{images/texture1}}
\caption{The effect of texture in terms of PCE}
\label{fig:exp:texture:pce}
\end{figure}

Fig.~\ref{fig:exp:texture:pce} shows a comparison of average PCE for this experiment which shows how image content affects the PCE for fingerprints obtained from varying number of flatfield and textured images. The figure indicates that sda-based fingerprints performs similarly as conventional way when the images are smooth whereas conventional way outperforms the proposed approach for textured images. 


On the other hand, Fig.~\ref{fig:exp:texture:tpr} shows the TPR for the same results where the threshold is set to $60$ as proposed in [jessica's relevant paper]. These figures support the theoretical analysis that when the images are the images are flatfield, both approaches result in similar PCE and TPR, whereas the difference of the two approaches is more clear when the training images are textured. The other implications of these figures are already well-known in the field (i.e., flatfield images are better than textured and as the number of images increase quality of fingerprint also increases.)

% To elaborate the difference of the two approaches for textured and flatfield images, we show the normalized results (i.e. $conventional/proposed$). Figure~\ref{figure:experiment:texture} shows the ratio of the average PCE under the $H_1$ hypothesis. As shown, when fingerprint is extracted from flatfield images, both approaches have similar performance. However, this difference becomes more significant when images are textured. For example, conventional approach results in $13\%$ higher PCE compared to proposed method when $20$ flatfield images are used whereas it achieves $103\%$ higher PCE when textured images are used.

% Figure~\ref{fig:exp:texture:tpr} shows the TPR of each fingerprint type as the number of images used to extract fingerprint changes for both flat-field and textured images. The results show the fingerprint extracted using conventional approach achieves slightly higher TPR than the other fingerprints. On the other hand, fingerprints obtained using the proposed approach achieves almost the same performance as the conventional approach; even higher in some cases.

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={1.8cm 20.4cm 4.8cm 3.78cm},clip]{images/texture2}}
\caption{The effect of texture in terms of TPR}
\label{fig:exp:texture:tpr}
\end{figure}


Since both techniques perform similarly for flatfield images, we can have a time comparison of the two approaches in that case. In other words, we know from this experiment that when we extract the fingerprint from $k$ flatfield images using conventional and sda-based technique, both will perform similarly. Therefore, it is important to provide time comparison for this case to illustrate the speed up that can be achieved for flatfield images. 

\begin{table}[!ht]
\centering
\caption{Time to extract fingerprints with proposed and conventional methods (in sec)}
\label{table:time:flat}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
     & $5$     & $10$    & $20$    & $30$   & $50$   \\ \hline
sda  & 4.97    & 5.99    & 8.22    & 10.35  & 14.49  \\ \hline
conv & 21.57   & 40.81   & 79.96   & 118.79 & 196.59 \\ \hline
speedup & 4.34 & 6.81    & 9.73    & 11.48  & 13.57  \\ \hline
\end{tabular}
\end{table}

Table~\ref{table:time:flat} shows the time it takes to extract fingerprint in both methods. Notice that in both cases $k$ images are read from the disk but for sda-based technique, only one denoising whereas for conventional way $k$ denoising operations are done. This shows as the training images increase, the speedup also increases. In case of flatfield images for training set, $13.5$ times speedup can be achieved for $50$ images.

The results indicate that, when the images are flatfield, the difference between the two fingerprint extraction is not very significant whereas the difference of conventional method and proposed method becomes higher for textured images. These results aligns with the mathematical analysis.


\paragraph{{\color{blue}Fingerprint equivalence}}

In the above experiment, we show that for flatfield images, both techniques perform similarly, however, conventional approach performs better than sda-based when images are textured. In this experiment, our goal is to find out the relationship between the number of images required by sda-based approach and the conventional approach when the images are textured. This experiment is performed using public images from the VISION dataset~\cite{shullani2017vision}. 
% compare conventional and proposed fingerprint extraction approaches in terms of the number images that achieves the same TPR and average PCE.
%For example, if a fingerprint is extracted from $m$ still images using conventional approach, how many images should be used to obtain an sda-frame to achieve the same performance? 
We created a training set from $50$ textured images for each camera in VISION dataset. We created $19$ fingerprints using $2$ to $20$ images for conventional approach, and $2$ to $50$ images when sda-frames approach is used. %The training set consists only of textured images (with lots of content) as it is a worse case compared to flat-field images. 
To create more testing scenarios, we divided each fingerprint to $500\times 500$ blocks and compared them with the corresponding blocks of the test PRNU noise. A total of $244,127$ comparisons have been done. 

% As shown in the figure, when content-heavy textured images are used, our approach requires between two to three times more images than the conventional approach. However, as shown in Figure~\ref{figure:exp:fp_equi:time}, we can achieve significant speed up compared to the conventional way. For example, a fingerprint obtained by sda-frame of $21$ images achieves the same TPR as a fingerprint obtained by the conventional approach using $10$ images. Our approach, however, can obtain fingerprint $3.75$ times faster the conventional approach.


\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={3cm 9cm 2.9cm 9cm},clip] {images/im_fp_equi.pdf}}
\caption{Fingerprint equivalence for sda-based and conventional approaches. x-axis indicates number of images for conventional. The left of y-axis (red) is the number of images required for sda-based and the right one (blue) is the speedup gained in this case.}
\label{figure:exp:fp_equi}
\end{figure}

Figure~\ref{figure:exp:fp_equi} shows the number of images required for sda-based approach to achieve at least the same TPR as the conventional way as well as the speedup gained in each case. For example, when fingerprint is created from $20$ textured images using conventional way, the same TPR can be achieved using $48$ images in sda-based approach. In this way, the fingerprint extraction is  approx. $3.85$ times faster for sda-based approach. Overall, using $2-3$ times more images for sda-based method, up to $4$ times speedup can be achieved with no loss in TPR when the images are textured.




% ------------------------------------------
\subsection{Performance comparison of video fingerprints}
\label{sec:exp:nstab}
In the above subsection, we have verified the two important concepts shown in the theoretical analysis. Here, we investigate a more practical use case of the proposed sda-based technique which is its usage for extracting a fingerprint from videos. Specifically, we investigate how performance changes when at least one of the query or known media is a video which can be pristine (unmodified) or from a social media. We first evaluate the performance of the video fingerprints on mixed media and analyze two important aspects of it on mixed media. We then focus on its performance on social media. 

% As mentioned in the Section~\ref{sec:background}, a video fingerprint can be extracted from i-frames or all-frames. Although, fingerprint from i-frames is faster to extract, the letter one creates a more reliable fingerprint, hence, likely to achieve higher performance. %In this subsection, we first investigate (i) the TPR for the mixed media case in NYUAD-MMD. We then analyze (ii) the number of frames in an sda-frame, (iii) whether order of frames have an impact, %(iv) the number of frames that is required for conventional method perform a similar performance as sda-based method, 
% and finally, we evaluated (v) and (vi) the performance on YouTube and %WhatsApp. %The experiments in this subsection were done using NYUAD-MMD except (v) and (vi) for which we have used VISION dataset.



\paragraph{{\color{blue}Train on video, test on images }}

Since videos are often long enough, extracting fingerprint from i-frames or all-frames may not cause significant difference in terms of TPR when two video fingerprints are correlated. However, in challenging cases such as matching a video fingerprint to a single image, the difference is likely to be very significant.
In \cite{taspinar2019source}, we investigated the TPR of the mixed-media NYUAD-mmd which contains images and videos from a number of cameras. The videos in the dataset are typically around $40$ seconds, so each video has approx. $1200$ frames. To analyze how the proposed sda-based approach performs compared to i-frames and all-frames, we have done ``Train on videos and test on images" experiment for these three cases. For each video, we created a fingerprint from $40$ i-frames, $40$ sda-frames, and all $1200$ frames of the $40$ second videos. This way we can evaluate whether or not sda-based approach can be useful. Notice that, here, sda-depth is equal to $30$ as we have $40$ sda-frame for each video. 
We then resized the images with bilinear scaling using the resizing factors we have learnt from the ``Train on images, test on videos" experiment and compare the resized images with the video fingerprints (For more details, please see~\cite{taspinar2019source}). 

\begin{table}[!ht]
\centering
\caption{TPR comparison of i-, sda-, all-frames for ``train on videos, test on images"}
\vspace{-0.3em}

\begin{tabular}{ |c|c|c|c|c| } 
    \hline
    type           & $\#match$ & $\#comparison$  & $ TPR $  & $\overline{PCE}$ \\  \hline
    i-frame        &   15070   & 23571    & 63.93\%      &  379  \\  \hline
    sda-frame      &   18849   & 23571    & 79.97\%      &  844  \\  \hline
    all-frame      &   19598   & 23571    & 83.14\%      &  879  \\  \hline
\end{tabular}
\label{table:vF2iN}
\vspace{-0.3em}
\end{table}



Table~\ref{table:vF2iN} compares the average PCE and TPR when fingerprint is obtained using these three approaches. When the fingerprints are obtained using only i-frames, $63.07\%$ of the images can be correctly attributed to their sources, and $82.85\%$ when all-frames are used. The proposed sda-based approach achieve slightly less that all-frames with TPR of $79.97\%$. %As seen, sda-frame achieves $4.89\%$ less than all-frames and $14.89\%$ more than i-frames which shows it can be used as a middle way between i-frames only and all-frames approaches. 


\begin{table}[!ht]
\centering
\caption{Time for video fingerprint extraction in second}
\vspace{-0.3em}
\begin{tabular}{|c|c|c|c|}
\hline
type           &  averaging & I/O + denoising  & total   \\ \hline
i-frame        & 0          & 50             & 50        \\ \hline
sda-frame      & 13         & 50             & 63        \\ \hline
all-frame      & 0          & 1407           & 1407      \\ \hline
\end{tabular}
\label{tbl:vF_extraction}
\vspace{-1em}
\end{table}

To understand how much time improvement can be achieved using sda-frames, we estimated fingerprint extraction time for a 40-second FullHD video captured @30 FPS. Table~\ref{tbl:vF_extraction} compares the average times for these approaches that it takes 50, 63, 1407 seconds for i-frames, sda-frames and all-frames, respectively. These results show that due to the superiority of sda-based fingerprint extraction over i-frame based, sda-based approach can easily replace commonly used i-frame based approach. Moreover, its accuracy is very close to all-frames based approach with a speedup of $22$ times. 

Notice that, the choice of sda-depth (i.e., $30$) is for comparison purpose. In the following experiment, we will investigate what is a good value for the sda-depth that can give an optimal performance in terms of time and speed.
% The results show that choosing only i-frames due to its low time-complexity is not the most effective solution in terms of performance for difficult cases such as mixed media. On the other hand, 


% Instead of using only i-frames, sda-based approach may significantly 

% These results show that the proposed approach can be a middle solution for fingerprint extraction from videos. %This technique compromises from performance to achieve a significant speed up.
% Furthermore, as mentioned in Section~\ref{sec:approach:sda_picture}, when the video is long enough (i.e. few minutes), more frames can be used in sda-frame which is expected to improve the performance.



{\color{blue}
\paragraph{Number of frames in sda-frame}}

To understand the schema, it is crucial to examine how the performance changes as $g$ (number of frames to be averaged for an sda-frame) changes. Given a video of $m$ frames (in our case approx. $1200$ frames), we divided them into groups of $g = 1, 5, 10, 30, 50, 200, 1200$. Therefore, $d = 1200, 240, 120, 40, 24, 6, 1$ sda-frames were created, respectively. When $g = 1$, the technique becomes same as using all frames whereas when $p = 1200$, all frames are used to create a single sda-frame. 

Each of these fingerprints are then compared with the noise all images from the same cameras in the above experiment.

Figure~\ref{figure:experiment:num_image_sda} shows the ROC curves for each sda-depth (i.e. $g$) as well as I-frames-only and all-frames (i.e., conventional approach). The results show that the conventional fingerprint extraction method results in the highest performance, whereas I-frame-only scheme performs significantly poorer compared to others. The proposed sda-based method performs close to conventional method that for all depths.

\begin{figure} [!ht]
\centering
{\includegraphics[width=\linewidth, trim={0.9cm 8.1cm 0.9cm 8cm}, clip]{images/sda_depth_roc.pdf}}
\caption{The ROC curves for varying sda-depths}
\label{figure:experiment:num_image_sda}
\end{figure}


Table~\ref{tbl:sda_depth} shows more details about the results as well as TPR when PCE threshold is set to $60$, average PCE, Area Under Curve (AUC), and average time it takes to create a fingerprint. As seen, the results indicate that the TPR and AUC of sda-based method are very close to conventional method, however, up to $50$ times speedup can be achieved using the sda-based method.


\begin{table}[!ht]
\centering
\caption{Sda-depths}
\label{tbl:sda_depth}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
            	 &i-    & all- 	& 5 	& 10   & 30   & 50   & 200  & 1200 \\\hline
TPR($\%$)	     &64.0  & 83.1 	& 82.3	& 81.3 & 80.0 & 79.8 & 80.1 & 79.8 \\\hline
$\overline{PCE}$ &379   & 879  	& 864	& 852  & 845  & 852  & 876	& 925  \\\hline
auc              & 85.3 & 94.6  & 94.1  & 93.6 & 92.9 & 92.7 & 93.1 & 93.5 \\ \hline
\textbf{time(s)} & 50   & 1407	&  276	& 142  & 62   & 48   &	32	& 27   \\ \hline
speedup         &28.1 & 1.0 & 5.1 & 9.9 & 22.7 & 29.3 & 44.0 & 52.1\\ \hline
\end{tabular}
\end{table}

On the other hand, using I-frames-only approach performs poorly compared to all other methods. Moreover, it does not achieve any speedup compared to sda-based method when sda-depth is greater than $50$. 


% Table~\ref{table:auc:num_image} shows the Area Under Curve (AUC) for Figure~\ref{figure:experiment:num_image_sda}. 


% \begin{table}[!ht]
% \centering
% \caption{AUC for proposed and conventional methods}
% \label{table:auc:num_image}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
%     $p$   & i-   & 1     & 5      & 10    & 30     & 50    & 200   & 1200  \\ \hline
%     % auc      & 0.946 & 0.9195 & 0.912 & 0.929  & 0.91 & 0.913 & 0.879 \\ \hline
%     auc & 85.3 & 94.6 & 94.1 & 93.6 & 92.9 & 92.7 & 93.1 & 93.5 \\ \hline
% \end{tabular}
% \end{table}



\paragraph{{\color{blue}Order of frames}}

Since a video is an ordered set of frames, each frame has significant similarity with previous and next frames. This section analyzes if the order of video has any impact on the proposed approach. In other words, our goal is to evaluate whether the TPR will change if the video frames are shuffled before sda-frames are created. For this purpose, we compared the TPR of when the images in sda-frames are ordered and they are shuffled in the same experimental setting above for the sda-depths we used above. Clearly, for sda-depth of $1$ and $1200$, there will be no difference because the same sda-frame(s) will be denoised and average. For example, when sda-depth is $1200$, the same sda-frame (the average of the $1200$ frames) will be produced for both ordered and shuffled case. 

\begin{table}[!ht]
\centering
\caption{Effect of order of frames on TPR($\%$)}
\label{table:exp:order}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
           & $1$    & $5$   & $10$  & $30$  & $50$  & $200$ & $1200$ \\ \hline
ordered    & 83.14 	& 82.25	& 81.30 & 79.97 & 79.85 & 80.05 & 79.77  \\ \hline
shuffled   & 83.14  & 82.35 & 81.32 & 80.09 & 79.82 & 80.15 & 79.77  \\ \hline
\end{tabular}

\end{table}

As seen in Fig.~\ref{table:exp:order}, the order of frames doesn't have a significant impact on TPR (i.e., approx. $0.05$ higher TPR on average). Overall, neither is has significant difference in terms of TPR. However, random access to frames is not as efficient as ordered access. Since p- and b- frames requires previous i-frames to be read first which makes the shuffled one will be significantly slower. For example, when the sda-depth is $30$, a fingerprint from the same video (as in Table~\ref{tbl:vF_extraction}) takes $299$ seconds with random access instead of $63$ seconds. If all the frames are extracted first, approx. 7 GB temporary storage is required for an uncompressed format which also will increase the I/O time. Overall, the ordered version is favorable as the very small performance improvement of shuffling comes at an expense of significant increase on either storage usage or time requirement. 


% \paragraph{{\color{red}(iv) The number of frames to achieve similar TPR}}
% Finally, it is known that the quality of fingerprint is not linearly improving as the number of frames increases. After a certain number of frames, the improvement in fingerprint quality gets smaller. In other words, it is possible to say that the TPR or PCE achieved using all $k$ frames (in our case $1200$), can be achieved using $k-l$ frames. Therefore, if $k-l$ frames are used instead of $k$, $\frac{l}{k}$ times speed up can be achieved. In this experiment, our goal is to find an approximate value of $l$ that achieves similar TPR and PCE as sda-frames. Specifically, we estimated TPR of fingerprints obtained using the first $100, 200, 300, \dots 1200$ frames as well as sda-frame from $1200$ frames whose depth is $1, 5, 10, 30, 50, 200,$ and $1200$ which is already available from Table~\ref{table:exp:order}.
% Table A shows ...

\paragraph{{\color{blue}Train and test on YouTube videos}}
This experiment aims to explore the performance achieved when two video fingerprints are correlated. Here, similar to the above experiment, we used the three fingerprints of each YouTube video. We correlate each video fingerprint with the others of the same type taken by the same camera. In other words, the fingerprints obtained from i-frames are correlated only the ones extracted using i-frames. The same is valid for sda- and all-frames. This way, a total of $3124$ correlation has been done for each type. 

Table~\ref{tbl:exp:ns:2yt} show that the fingerprints from i-frames results in significantly worse performance compared to sda- and all-frames. Moreover, the fingerprint extracted from all-frames takes 50x more times compared sda-frames while the performance is $x\%$ higher. These results differs slightly from the previous results. One reason the videos that are labeled ``still" and ``outdoor" tend to give lower PCE values for fingerprint from sda-frames compared to all-frames.
It is still show that sda-frames are always superior compared to i-frames in both time and speed.

\begin{table}[!ht]
\centering
\caption{TPR for train and test YouTube videos experiment}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & i-      & sda-50   & sda-200  & sda-600  & all-   \\ \hline
TPR & 29.29   & 59.54    & 54.58    & 50.74    & 69.62 \\ \hline
\end{tabular}
\label{tbl:exp:ns:2yt}
\end{table}


\paragraph{{\color{blue}Train on Facebook images, test on YouTube videos}}
From the previous experiments, we know that the sda-based fingerprint extraction can help achieve a significant speedup for both videos and images with a very small loss in performance which can be overcome by increasing the number of still images used for fingerprint extraction if available. (See experiment x for images, and y for videos). In this part, our goal is to show that the proposed method can be successfully applied to social media. Specifically, in this part, we will do ``Train on Facebook images, test on YouTube videos" experiment. The importance of this experiment is both media sharing services contains billions of visual media that the conventional fingerprint extraction approaches from these web pages has very high time complexity. Therefore, fingerprint extraction methods (along with search techniques) that speeds up the search is highly crucial.

In this experiment, for each camera in VISION dataset that has non-stabilized videos, we created fingerprints from $100$ Facebook images (i.e., the ones labeled FBH) using conventional fingerprint extraction methods. 
We then created fingerprints from all non-stabilized YouTube videos (i.e., the ones labeled flatYT, indoorYT, and outdoorYT) using only i-frames, sda-50, sda-200, sda-600, and all-frames. Here, we used the first $60$ seconds of YouTube videos to extract the above fingerprints. When we use sda- or all-frames, we approx. use $1800$ frames for each video whereas for the first $60$ seconds of the videos have $31.3$ i-frames on average. 

In this experiment, we correlated the image fingerprints with each video fingerprint of each type using the efficient search proposed in ~\cite{taspinar2019source} and a total of $343$ pair have been compared for each fingerprint type. 

Table~\ref{tbl:exp:ns:fb_yt} shows the TPR of these correlations. Similar to ``Train on videos, test on images" experiment, these results show that for fingerprints obtained from Facebook images matches with $81.34\%$ of the videos for sda-50 which is higher than both all-frames and i-frames. On the other hand, all-frames achieves slightly lower performance, fingerprints from i-frames yield approx. $30\%$ lower TPR for this setting. This results show that sda-based approach is a good replacement for usage of i-frames or all-frames for this case.

\begin{table}[!ht]
\centering
\caption{TPR of different fingerprint types when a fingerprint from Facebook images and another from  YouTube videos are correlated}
\label{tbl:exp:ns:fb_yt}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
    & i-      & sda-50   & sda-200  & sda-600  & all-   \\ \hline
TPR & 51.60   &  81.34   & 79.88    & 78.13    & 79.59  \\ \hline
\end{tabular}
\end{table}


% ------------------------------------------
\paragraph{{\color{blue}Stabilized videos}}
% \label{sec:exp:stab}

A recent work [cite] has shown that a fingerprint obtained from a long stabilized video can successfully be matched with other videos from the same camera. However, as above, thousands of frames must be denoised for this which may not be practical in some settings. A potential alternative for this problem is the usage of SDA-frames which may lead to a significant speed up. To evaluate this, we captured long stabilized videos from $5$ cameras, a total of $37$ videos which adds up to $260$ minutes. As shown in \cite{taspinar2016source, iuliani2017hybrid}, the first frame of the videos are typically not geometrically transformed. But as \cite{mandelli2018facing} pointed out, they may not always be available or some cameras may transform them as well, hence, we ignored those frames.

For this experiment, we extracted fingerprints from the frames of $20, 40, \dots 240$ seconds using conventional method as well as sda-based method for sda-depth of $30, 50,$ and $200$ as these are reasonable choices from the previous experiments. 
We correlated each fingerprint with other fingerprints of different videos from the same camera that are created using the same number of frames. For example, sda-30 fingerprints of $20$ second videos are correlated with the same type fingerprints from the same camera. 

Figure~\ref{figure:exp:stab_res} shows the TPR for three cameras (i.e., Huawei Honor, Samsung S8, and iPhone 6plus) and the total average of all the five cameras. 

% The results show that as the videos get longer, the TPR increases which supports the idea proposed in [the recent study/cite].   

% \begin{table}[!ht]
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
%       & 20 sec & 40 sec & 60 sec & 80 sec & 10 sec \\ \hline
% all    & 0.5321 & 0.8705 & 0.9659 & 0.9918 & 0.9981 \\ \hline
% sda-50 & 0.0346 & 0.2033 & 0.4239 & 0.5938 & 0.7172 \\ \hline
% \end{tabular}
% \end{table}

\begin{figure} [!ht]
\centering
{\includegraphics[trim={1.2cm 8cm 1.4cm 8.3cm}, clip, keepaspectratio=true,width=\linewidth]{images/total_stab3.pdf}}
% {\includegraphics[trim={2.75cm 9.3cm 2.75cm 9.3cm}, clip, keepaspectratio=true,width=\linewidth]{images/stab_res.pdf}}
\caption{TPR for stabilized videos for varying sda-depths}
\label{figure:exp:stab_res}
\end{figure}

The results show that as videos get longer, fingerprints obtained using conventional or sda-based approach get more reliable. Moreover, the effect of increased sda-depth is more significant for this case in comparison to non-stabilized videos. %This is because sda-based approach performs poorly for iPhone cameras whereas for others, the performance is not almost as good as conventional approach. Figure X shows TPR of 

While for some cameras conventional and sda-based approaches perform similarly (Huawei and Samsung cameras), for others (i.e., iPhone cameras) there is a significant difference between the two. For example, for Samsung S8 $sda-200$ fingerprint from $120$ seconds video, perform similarly as $180$ seconds conventional fingerprint. Therefore, for this particular case, $sda-200$ can speedup $66$ times \big(i.e. $\frac{180}{120}\times \frac{1407}{32}$\big)(see Table~\ref{tbl:sda_depth} for times). On the other hand for iPhone 6 plus, $60$ seconds video with conventional and $160$ seconds $sda-50$ have similar TPR. Therefore, $11x$ \big(i.e., $\frac{60}{160}\times \frac{1407}{48}$\big) speedup can be achieved in this case. Overall, a speedup between these numbers (i.e. $11$ and $60$) can be achieved without any loss in TPR if a long video is available.


Overall, this subsection shows that the proposed sda-based fingerprint extraction outperforms  the commonly used I-frame-only technique in all the cases for videos. These include for mixed media, stabilized videos, and social media. On the other hand, the sda-based method achieves comparable results as all-frames-used fingerprint extraction with up to 50 times speedup. We also show the impact of sda-depth on the performance that can be achieved in various cases. Finally, we show that sda-based method order of frames doesn't have an impact on performance, yet shuffling the frames cause either a significant slow down or high I/O cost. Therefore, ordered access to videos is preferable to random access.


\subsection{Analysis on image fingerprints}
\label{sec:exp:img}

This subsection 
To verify the theoretical analysis and understand the properties of the sda-based fingerprint extraction method, we have done some experimental analysis on images. The experiments help clarify three main issues related to images that potentially have impact on the performance: (i) the effect of texture, (ii) the depth of an sda-frame (i.e., the number of images an sda-frame)  (iii) the effect of compression. Moreover, we investigated (iv) the equivalence of conventional fingerprint extraction and proposed approach. In these experiments, we used VISION dataset \cite{shullani2017vision} as it is a comprehensive set containing flatfield and textured images as well as the compressed social media versions of those (i.e., compressed in WhatsApp or Facebook). 


\paragraph{{\color{blue}Effect of sda-depth on image fingerprint}}

Another crucial issue is to understand the effect of the number of images in each sda-frame on performance and time. Suppose there are $k$ textured images from a camera and we want to create a fingerprint using the proposed technique. For this, we can create $g$ groups of $d$ images (where $k=d \times g$). So, we create $g$ sda-frames resulting in $g$ denoising operations rather than $k$. For example, in the above experiment $d=k$ (i.e., sda) or $d=1$ (i.e., conv.) was chosen. Since we already know that flatfield images doesn't have much impact on correlation, we only use textured images for training set. 

In this experiment, for each camera in VISION dataset, we create fingerprints using $50$ textured images. We set the sda-depth to $1, 2, 5, 10, 25$ and $50$. Therefore, we create $50, 25, 10, 5, 2,$ and $1$ sda-frames, respectively. The rest of the images were used as test images. We then correlated each fingerprint with the noise of those query images in the block-wise manner as explained above. 

% Fig.X shows Y...
\begin{table}[!ht]
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
    & sda-1    & sda-2    & sda-5    & sda-10  & sda-25   & sda-50   \\ \hline
PCE & 652.8 & 514.6 & 390.0 & 332.2  & 285.0  & 252.4 \\ \hline
TPR & 0.80  & 0.78  & 0.75  & 0.72   & 0.69   & 0.67   \\ \hline
\end{tabular}
\caption{SDA-depth vs TPR and PCE, change with figure}
\label{table:sda_depth_perf}
\end{table}

Table~\ref{table:sda_depth_perf} shows that as the sda-depth increases, the average PCE decreases. This characteristic is consistent with the right columns in Fig.~\ref{fig:exp:texture:pce} and ~\ref{fig:exp:texture:tpr}. For textured images, the more images we combine to create an sda-frame, the lower PCE and TPR will be. As seen, when the depth is one (i.e., sda-1 which is same as conventional approach), the average PCE of $512\times512$ blocks is $663$ which gets lower when we combine more images. %Although the difference in of the two approaches is not very high in this setting, it might be higher when compression is higher.

\paragraph{{\color{blue}Social media images}}
% \textbf{THIS IS MORE LIKE SOCIAL MEDIA}
Another factor that might impact performance of sda-based method is the compression of the images used for reference fingerprint. To understand this batter, we used the images of VISION dataset. Fortunately, each image in the vision dataset has three compressed versions: WhatsApp(WA), Facebook high-resolution (FBH), and Facebook low-resolution (FBL). While the average size of original natural images are 2.88 MB, the average size of WA, FBH, and FBL are 327 KB, 337 KB, and 122 KB, respectively. Note that the resolution of FBH is typically higher than WA which indicates that the compression of FBH is higher than WA. So WA images has the lowest compression and FBL has the highest.

In this experiment, for each type of data (i.e., FBH, FBL, and WA), we used the $50$ textured images as training set and compared the fingerprints with rest of the images of a camera. We have done the same experiment as (sda-depth) and obtained\textbf{ ...}

\begin{table}[!ht]
\centering
\begin{tabular}{|c|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{WA} & \multicolumn{2}{c|}{FBH} & \multicolumn{2}{c|}{FBL} \\\hline 
       & PCE     & TPR     & PCE       & TPR    & PCE      & TPR  \\ \hline
sda-1  & 945.1   & 0.92    & 902.6     & 0.88   & 190.9    & 0.49 \\ \hline
sda-2  & 624.6   & 0.89    & 622.5     & 0.81   & 123.3    & 0.38 \\ \hline
sda-5  & 383.4   & 0.80    & 398.6     & 0.69   & 70.0     & 0.27 \\ \hline
sda-10 & 297.6   & 0.74    & 312.1     & 0.61   & 51.3     & 0.23 \\ \hline
sda-25 & 241.9   & 0.69    & 246.3     & 0.53   & 41.2     & 0.20 \\ \hline
sda-50 & 215.8   & 0.66    & 212.4     & 0.49   & 37.5     & 0.18 \\ \hline
\end{tabular}
\caption{compression}
\label{table:exp:img:compress}
\end{table}

As seen in the Table~\ref{table:exp:img:compress}, the higher the compression, the lower the PCE and TPR, which is already known in the field. However, based on these results, we can say that compression does not seem to affect  sda-depths. For example, the ratio of the average PCE for sda-10 and sda-25 is $\frac{297.6}{241.9}=1.23$ for WA, $\frac{312.1}{246.3}=1.27$ for FBH, and $\frac{51.3}{41.2}=1.25$ for FBL which shows compression does not have impact on sda-depth. 

An interesting behaviour to note that even though the average PCE for FBH is greater than WA, the TPR is lower. Based on the results, when the average PCE is low (i.e. below a few hundred), WA images tend to have higher average PCE, whereas when it is high, FBH tends to give higher average PCE than WA. Thus, total averages becomes approximately equal but the TPR of WA is significantly higher. However, we couldn't find the reason for this characteristic.

Note that, because the resolutions of images are lower in this experiment (due to social media resizing), we didn't employ block-wise correlation; instead we did the correlations on full resolutions.
% We also compressed the textured images by changing the quality factor of each image. Assuming the quality factor of original images is $100$, we compressed the images with quality factor $80, 60, 40,$ and $20$. This way, we created $5$ samples of each.

% \paragraph{(iv) Fingerprint equivalence}
% Finally, we evaluated the number of images required for both techniques that achieves similar PCE and TPR. For example, if $m$ still images are used in conventional approach, here we find the number of images that achieves similar performance using sda-based approach. 
% To evaluate this, we used VISION dataset that $19$ camera fingerprint is obtained from $2$ to $20$ images using conventional approach and $49$ fingerprints from $2$ to $50$ images using sda-based approach. We then found the lowest number of images for sda-based method that achieves at least the same PCE and TPR as conventional approach. 

% Furthermore, we again have employed block-wise comparison and a total of $244,127$ comparison has been made. 

% \begin{figure} [!ht]

% \subfloat[Equivalence of sda and conv]{\includegraphics[keepaspectratio=true, width=85mm]{images/im_fp_eq.pdf}\label{figure:exp:fp_equi:perf}}

% \subfloat[Speed up achieved by sda]{\includegraphics[keepaspectratio=true, width=88mm]{images/im_fp_eq_speedup2.pdf}\label{figure:exp:fp_equi:time}}
% \caption{Fingerprint Equivalence}
% \label{figure:exp:fp_equi}
% \end{figure}



% % \begin{figure} [!ht]
% % \centering
% % % trim={2.35cm 19.7cm 4.25cm 2.39cm},clip,
% % \subfloat [The effect of texture in terms of PCE] {\includegraphics[width=82mm] {images/texture_pce2}\label{fig:exp:texture:pce}}

% % \subfloat [The effect of texture in terms of TPR] {\includegraphics[width=82mm]{images/texture_tpr2}\label{fig:exp:texture:tpr}}
% % \caption{The effect of image content}
% % \end{figure}


% Figure~\ref{figure:exp:fp_equi:perf} shows the number of images required for sda-frame to achieve at least the same (i) TPR (ii) average PCE as the conventional fingerprint extraction. On the other hand, Figure~\ref{figure:exp:fp_equi:time} shows the speed up achieved by sda-frame approach compared to the conventional way. For example, to obtain same TPR of a fingerprint obtained using $10$ images using conventional way, $21$ images are needed using sda-based method. In this case $3.75x$ speedup can be achieved compared to conventional approach. On the other hand, to achieve approx. same PCE value $22$ images are needed which results in $3.6x$ speedup. 

% Notice that all images used in fingerprints are textured as it is the worst case scenario for sda-based approach based on theoretical analysis (and experiment (i)). When, more flatfield images exists in the sda-frames, the improvement will be higher for sda-based approach (see Table~\ref{table:time:flat}). 






==> todo.tex <==
+1) imFP vs vidFP
    imFP --> full sensor
    when imFP is not full sensor, it is important to make sure how it is created. (scale? crop? scale and crop). We will use relative scaling factor.
    
+2) vidFP vs vidFP
+3) vidFP vs imNS
+4) i-, all, and mean frame.
    math for mean frame
5) when do they fail, why? 
+6) time comparison
7) 


related work
how fingerprint is extracted
how it is used
how people proposed
single resolution vs. multiple resolution
what has been done for video research

in background, talk about sensor, video/image capture pipeline
different cameras, different methods

use random to create 40 avg frame compare 
try surf to choose best 1200 frames



1) PRNU
2) 
3) Scaling and cropping paper, cite our paper, too. Talk about NCC for a little bit. + equation.

4) Jump to video --> from previous work and the new ones
    4a) Sensor in terms of video and imagesz
5) 
